Euclid preparation: 6x2 pt analysis of Euclid's spectroscopic and photometric data sets

We present cosmological parameter forecasts for the Euclid 6x2pt statistics, which include the galaxy clustering and weak lensing main probes together with previously neglected cross-covariance and cross-correlation signals between imaging/photometric and spectroscopic data. The aim is understanding the impact of such terms on the Euclid performance. We produce 6x2pt cosmological forecasts, considering two different techniques: the so-called harmonic and hybrid approaches, respectively. In the first, we treat all the different Euclid probes in the same way, i.e. we consider only angular 2pt-statistics for spectroscopic and photometric clustering, as well as for weak lensing, analysing all their possible cross-covariances and cross-correlations in the spherical harmonic domain. In the second, we do not account for negligible cross-covariances between the 3D and 2D data, but consider the combination of their cross-correlation with the auto-correlation signals. We find that both cross-covariances and cross-correlation signals, have a negligible impact on the cosmological parameter constraints and, therefore, on the Euclid performance. In the case of the hybrid approach, we attribute this result to the effect of the cross-correlation between weak lensing and photometric data, which is dominant with respect to other cross-correlation signals. In the case of the 2D harmonic approach, we attribute this result to two main theoretical limitations of the 2D projected statistics implemented in this work according to the analysis of official Euclid forecasts: the high shot noise and the limited redshift range of the spectroscopic sample, together with the loss of radial information from subleading terms such as redshift-space distortions and lensing magnification. Our analysis suggests that 2D and 3D Euclid data can be safely treated as independent, with a great saving in computational resources.

==> input/1-Observables.tex <==
\section{Observables}
\label{sec:ch4_cls}
In this forecast the cosmological model adopted is a flat $\wzwaCDM$ cosmology. The dark energy equation of state is described by the CPL parameterisation
%
\begin{equation}
w_{\rm DE}(z) = \wz + \wa \frac{z}{1+z}
\end{equation}
%
and the Hubble factor $H(z)$ is given by
%
\begin{align}
\resizebox{0.45\textwidth}{!}{$
\frac{H^2(z)}{H^2_0} = 
\Omm (1+z)^3 + (1-\Omm)(1+z)^{3(1+\wz+\wa)}\exp\left(-3\wa\frac{z}{1+z}\right)\, .
$}
\end{align}
%
The cosmological parameters involved in the analysis are summarised in table \tabref{tab:ch4_cosmo_pars_fiducials}, were the values in the reference cosmology are reported.
%
\begin{table*}
\centering
\begin{tabular}{CCCCCCCCC}
\toprule
\text{Parameter} & \Omb & \Omm & \wz & \wa & \h & \ns & \sige & \mnu[\mathrm{eV}] \\
\midrule
\text{Fiducial value} & 0.05 & 0.32 & -1 & 0 & 0.67 & 0.96 & 0.816 & 0.06 \\
\bottomrule
\end{tabular}
\caption{Values of the cosmological parameters considered the forecast in the reference cosmology. All the parameters are let free to vary except for the sum of the neutrino masses, which has been fixed to its reference value $\mnu = \SI{0.06}{eV}$.}
\label{tab:ch4_cosmo_pars_fiducials}
\end{table*}
%
The probes considered in this forecast are: the photometric galaxy clustering ($\GCph$), the spectroscopic galaxy clustering ($\GCsp$), and the weak lensing ($\WL$). For the $\WL$ and $\GCph$ probes, the observable employed is the tomographic angular power spectrum $C_{ij}(\ell)$. For the $\GCsp$ probe, both the harmonic power spectrum and the Fourier power spectrum have been considered as observables. The Fourier power spectrum approach is the same followed in~\citetalias{Blanchard:2019oqi} and briefly described in \secref{sec:ch4_gcsp_pk}. However, in this work the corresponding Fisher matrix is not directly computed; instead it is taken as an external input from the IST:F public online repository~\cite{ISTFFishers}.

The angular power spectrum $C(\ell)$ is essentially the harmonic transform of the two-point tomographic angular correlation function. Each cosmological probe $A$ in a given redshift bin $i$ can be associated to a field $f^{A}_i(\versor{n})$ defined on the sky, which can be expanded in spherical harmonics
%
\begin{equation}\label{eq:ch4_spherical_harmonics_expansion}
f^A_i(\versor{n}) = 
\sum_{\ell = 0}^{\infty} \sum_{m = -\ell}^{\ell}
a_{\ell m}^{Ai} Y_{\ell m} (\versor{n})\, ,
\end{equation}
%
The $a^{Ai}_{\ell m}$ coefficients are the projection of $f^A_i$ on the spherical harmonics orthonormal basis
%
\begin{equation}\label{eq:ch4_alm_def}
a_{\ell m}^{Ai} = 
\int d\Omega \, Y_{\ell m}^{*}(\versor{n}) f^A_i(\versor{n})
\end{equation}
%
The tomographic angular correlation between probe $A$, at the redshift bin $i$, and $B$, at the redshift bin $j$, is then defined as the following implicit relation
%
\begin{equation}\label{eq:ch4_cl_implicit_def}
\left \langle 
a_{\ell m}^{Ai} 
\left( a_{\ell' m'}^{Bj} \right)^*
\right \rangle = \cl{AB}{ij}{\ell} \delta_{\ell\ell^{\prime}} \delta_{m m^{\prime}}\, .
\end{equation}
%
where the angular brackets here denote the theoretical expectation value. In the Limber approximation the expression of the angular power spectra can be parameterised as
%
\begin{equation}\label{eq:ch4_limber_cls}
\cl{AB}{ij}{\ell} \simeq \frac{c}{H_0} \int_{z_\mathrm{min}}^{z_\mathrm{max}} \mathrm{d} z \frac{W_{i}^{A}(z) W_{j}^{B}(z)}{E(z) \chi^{2}(z)} P_{\delta\delta}\left[k=\frac{\ell+1/2}{\chi(z)},z\right]\, ,
\end{equation}
%
where $\chi(z)$ is the comoving distance, $W_{i}^{A}$ is the weight (or window) function for the probe $A$ in the  $i$-bin  (details are given in the next subsections), and $P_{\delta\delta}$ is the total matter power spectrum introduced in \eqref{eq:ch1_pmm_definition}. In this forecast, it has been taken as an external input, loading the publicly available power spectra computed in~\citetalias{Blanchard:2019oqi}. These power spectra have been computed using the \CAMB Boltzmann code with a revised version of the HALOFIT~\cite{Takahashi2012} recipe to take into account non-linearities. Massive neutrinos have been included among the Boltzmann code configuration parameters, using $\mnu = \SI{0.06}{eV}$ as reference value.

The power spectra are publicly available at~\cite{ISTFPowerSpectra}.

The functional form of the weight function $W_{i}^{A}$ depends on the probe $A$. The fundamental ingredient for the computation of $W_i^A$ is the redshift distribution per unit solid angle, $\de N^A(z)/(\de z \de\Omega)$, associated to the probe. This can be either modelled analytically, as in the case of $\WL$ or $\GCph$, or can be obtained via simulations, as for $\GCsp$.

The normalised redshift density of the probe $A$ in the $i$-bin can be computed from the redshift distribution as
%
\begin{equation}\label{eq:ch4_norm_density_def}
n^A_{i}(z)=\frac{\int_{z_{i}^{-}}^{z_{i}^{+}} \de z_{\rm{p}} \, \frac{\de N^A}{\de z \de\Omega}(z) p_A\left(z_{\rm{p}} | z\right)}{\int_{z_{\min }}^{z_{\max }} \de z \int_{z_{i}^{-}}^{z_{i}^{+}} \de z_{\rm{p}} \, \frac{\de N^A}{\de z \de\Omega}(z) p_A\left(z_{\rm{p}} | z\right)}\, .
\end{equation}
%
The function $p_A(z_{\rm p}|z)$ is the probability that a galaxy with true redshift $z$ will be measured with a redshift $z_{\rm p}$. This probability incorporates the redshift measurement errors, and it is modelled differently depending whether the redshift measurement is photometric or spectroscopic. The parameterisation chosen is the same of~\citetalias{Blanchard:2019oqi}
%

\begin{align}
p_{A}(z_{\rm{p}} | z) = &
\frac{1-f_{\rm out}}{\sqrt{2 \pi}\sigma_{\rm{b}}(1+z)} 
\exp \left\{-\frac{1}{2}\left[\frac{z-c_{\rm{b}} z_{\rm{p}}-z_{\rm{b}}}{\sigma_{\rm{b}}(1+z)}\right]^{2}\right\} + \\ \nonumber
&\frac{f_{\rm out}}{\sqrt{2 \pi} \sigma_{\rm{o}}(1+z)}
\exp \left\{-\frac{1}{2}\left[\frac{z-c_{\rm{o}} z_{\rm{p}}-z_{0}}{\sigma_{\rm{o}}(1+z)}\right]^{2}\right\}\, 
\end{align}

This model allows us to include both a multiplicative and additive bias in the redshift determination of a fraction $1-f_{\rm out}$ of sources with well measured redshifts, and a fraction $f_{\rm out}$ of catastrophic outliers, i.e. systems with severely incorrect estimate of the redshift. The values of the parameters for the probability functions are summarised in \tabref{tab:ch4_prob_convolve_params}. The uncertainty $\sigma_{\rm b}$ on the correctly measured (not catastrophic) redshifts has been chosen from the \Euclid design requirements~\cite{euclidredbook} described in \chpref{ch2:euclid_mission}. In particular $\sigma_{\rm b} = 0.05$ for $\GCph$ and $\sigma_{\rm b} = 0.001$ for $\GCsp$.

%------- WEIGHT FUNCTIONS PLOT -------%
\begin{figure*}
\centering
\includegraphics{Figures/weight_functions_plot.pdf}
\caption{Plot of the weight functions for the probes considered in the forecast. Note that for $\WL$ at high redshift bins the weight function \eqref{eq:ch4_weak_lensing_full_weight} (solid line) becomes negative, due to the contribution of intrinsic alignment. The shear weight function \eqref{eq:ch4_shear_weight} (dashed line) remains instead always positive as it should be.}
\label{fig:ch4_weight_functions_plot}
\end{figure*}

%------- PROBABILITY DISTR PARAMS -------%
\begin{table*}
\centering
\begin{tabular}{L*{7}{C}}
\toprule
\text{probe} & c_{\mathrm{b}} & z_{\mathrm{b}} & \sigma_{\mathrm{b}} & c_{\mathrm{o}} & z_{\mathrm{o}} & \sigma_{\mathrm{o}} & f_{\text {out }} \\
\midrule
\GCph & 1.0 & 0.0 & 0.050 & 1.0 & 0.1 & 0.05 & 0.1 \\
\GCsp & 1.0 & 0.0 & 0.001 & \text{--} & \text{--} & \text{--} & \text{--} \\
\bottomrule
\end{tabular}
\caption{Values of the parameters adopted for the probability distributions defined in \eqref{eq:ch4_prob_z_distr} and \eqref{eq:ch4_spectro_prob_z_distr}. For $\GCsp$ the outlier parameters are not reported since they are irrelevant, being the outliers fraction $f_{\rm out} = 0$.}
\label{tab:ch4_prob_convolve_params}
\end{table*}

\subsection{Photometric galaxy clustering}
\label{sec:ch4_gcph}
In the case of galaxy clustering the starting point to write down the weight function is the galaxy density contrast $\delta^{\rm g}(\mathbf{x}, z)$, where $\mathbf{x} = \chi(z) \versor{n}$ is the comoving distance vector. This is also referred to as the 3D density constrast, since it is a function of both the direction and the distance. As galaxies are tracers of the dark matter distribution, $\delta^{\rm g}$ is expressed in terms of the matter density contrast $\delta$ through the galaxy bias $b$. In Fourier space the galaxy bias can be implicitly defined by the following relation
%
\begin{equation}\label{eq:ch4_bias_definition}
\delta^{\rm g}(\mathbf{k}, z) = b(z) \delta(\mathbf{k}, z)\, ,
\end{equation}
%
with $\mathbf{k}$ being the wavevector and $k$ its module. In general the galaxy bias depends also on the scale $k$, but in this work this $k$-dependence has been neglected, following the treatment of~\citetalias{Blanchard:2019oqi}.

The field to be expanded in spherical harmonics for galaxy clustering is $\Delta^{A}_i(\versor{n})$, the galaxy density contrast \emph{projected} along the observation direction $\versor{n}$
%
\begin{equation}\label{eq:ch4_projected_density_contrast}
\Delta^{A}_i(\versor{n})=
\int_{z_{\rm min}}^{z_{\rm max}} \mathrm{d}z \, W^A_i(z) 
\int \frac{\mathrm{d}^{3} k}{(2 \pi)^{3}} e^{i \mathbf{k} \cdot \versor{n} \chi(z)} \delta^{\rm g}_{i}(\mathbf{k}, z) \, .
\end{equation}
%
Here the index $A$ stands for $\GCph$ or $\GCsp$, and $W^A_i(z)$ is the galaxy clustering weight function
%
\begin{equation}\label{eq:ch4_galaxy_weight}
W^A_i(z) = b^A(z) \frac{H(z)}{c} n^{A}_{i}(z)\, ,
\end{equation}
%
where $n^{A}_{i}(z)$ is defined by \eqref{eq:ch4_norm_density_def}. The true redshift distribution of the photometric sample is modelled as in the \Euclid redbook~\cite{euclidredbook}
%
\begin{equation}\label{eq:ch4_photo_true_nz}
\frac{\de N^{\mathrm{ph}}}{\de z \de\Omega}(z) = N^{\mathrm{ph}}_0 \left(\frac{z}{z_{0}}\right)^{2} \exp \left[-\left(\frac{z}{z_{0}}\right)^{3 / 2}\right]\, ,
\end{equation}
%
where $z_0 = 0.9/\sqrt{2}$ and the normalisation factor $N^{\mathrm{ph}}_0$ is chosen such that the surface density of galaxies is equal to $30$ galaxies per $\si{arcmin^2}$, corresponding to an expected total number of galaxies of about $\num{1.6e9}$. This redshift distribution is then convolved with the photometric probability distribution $p_{\rm ph}(z_{\rm p}|z)$ defined in \eqref{eq:ch4_prob_z_distr}.

The redshift evolution of the galaxy bias $b^A(z)$ is modelled as in~\citetalias{Blanchard:2019oqi}: for $\GCph$ a piece-wise constant function is employed such that 
%
\begin{equation}
b^{\mathrm{ph}}(z) = b^{\mathrm{ph}}_i = \sqrt{1 + \bar{z}_i}, \qquad z_i^- < z < z_i^+\, ,
\end{equation}
%
where $\bar{z}_i = (z_i^- + z_i^+)/2$ is the mean redshift of the bin $i$. As in~\citetalias{Blanchard:2019oqi}, this forecast employs 10 tomographic bins chosen to be equally populated, i.e. with equal number of galaxies per bin, according to the distribution \eqref{eq:ch4_photo_true_nz}. The bin edges and the photometric galaxy bias values are summarised in \tabref{tab:ch4_photo_tomo_bins}. The $\GCph$ weight function is explicitly given by \eqref{eq:ch4_galaxy_weight} in which $A = \mathrm{ph}$
%
\begin{equation}
W^{\mathrm{ph}}_i(z) = b^{\mathrm{ph}}(z) \frac{H(z)}{c} n^{\mathrm{ph}}_{i}(z)\, .
\end{equation}
%
A plot of this function for all the photometric redshift bins is shown in the upper panel of \figref{fig:ch4_weight_functions_plot}.

% Tomographic Bins GCph
%-----------------------------------------%
\begin{table*}
\centering
\begin{tabular}{L*{10}{C}}
\toprule
z_i^- & 0.001 & 0.418 & 0.560 & 0.678 & 0.789 & 0.900 & 1.019 & 1.155 & 1.324 & 1.576 \\
z_i^+ & 0.418 & 0.560 & 0.678 & 0.789 & 0.900 & 1.019 & 1.155 & 1.324 & 1.576 & 2.500 \\
\midrule
b^{\rm ph}_i & 1.100 & 1.220 & 1.272 & 1.317 & 1.358 & 1.400 & 1.445 & 1.497 & 1.565 & 1.743 \\
\bottomrule
\end{tabular}
\caption{Tomographic bin edges for photometric ($\GCph$) galaxy clustering, along with the values of the bias.}
\label{tab:ch4_photo_tomo_bins}
\end{table*}
%-----------------------------------------%

\subsection{Spectroscopic galaxy clustering: 2D approach in the harmonic domain}
\label{sec:ch4_gcsp_cl}
For the spectroscopic sample the true redshift distribution is the one obtained from the analysis of the \Euclid SPV2~\cite{GranettSPV2}. The range of the expected distribution of $\Halpha$-emitting galaxies is determined by the sensitivity range of NISP detectors. In particular, for a galaxy to be observed by NISP its redshift must fall in the range $z \in [0.9, 1.8]$ (see \chpref{ch2:euclid_mission}). The total number of galaxies in the sample is about $\num{2e7}$, which is smaller by a factor $\sim 80$ than the total number photometric galaxies. In the present work, for numerical reasons\footnote{This operation is aimed at mitigating the sharpness of the boundaries of the spectroscopic bins, to prevent potential numerical instabilities in the computation of the redshift integrals.} it has been decided to convolve the spectroscopic redshift distribution with the probability $p_{\mathrm{sp}}(z_{\rm p}|z)$. For this probability is again assumed the functional form \eqref{eq:ch4_prob_z_distr}, but using parameters different from the case of photometric clustering
%
\begin{equation}\label{eq:ch4_spectro_prob_z_distr}
p_{\mathrm{sp}}\left(z_{\rm{p}} | z\right) = \frac{1}{\sqrt{2 \pi} \sigma_{\rm{b}}(1+z)} \exp \left\{-\frac{1}{2}\left[\frac{z-c_{\rm{b}} z_{\rm{p}}-z_{\rm{b}}}{\sigma_{\rm{b}}(1+z)}\right]^{2}\right\} \, .
\end{equation}
%
In particular, the redshift uncertainty $\sigma_{\rm b}$ is set to $\num{0.001}$ as specified in the scientific requirements in~\cite{euclidredbook} for \Euclid, and the fraction of outliers $f_{\rm out}$ is set to zero. The other parameters in \eqref{eq:ch4_spectro_prob_z_distr} are instead assumed to be the same as for $\GCph$, as summarised in \tabref{tab:ch4_prob_convolve_params}. 

The spectroscopic galaxy bias $b^{\mathrm{sp}}(z)$ also is taken to be a piece-wise constant function, and the values $b^{\mathrm{sp}}_i$ in the bins are summarised in \tabref{tab:ch4_spectro_tomo_bins} along with the bin edges. Both the bias values and the bins are the same that have been used in~\citetalias{Blanchard:2019oqi}, but in this work also a finer binning has been considered, in particular 12, 24 and 40 equally spaced bins in the range $0.9 < z < 1.8$. The values of the bias for finer binning are obtained by linear interpolation of the values listed in \tabref{tab:ch4_spectro_tomo_bins}.

The $\GCsp$ weight function is explicitly given by \eqref{eq:ch4_galaxy_weight} in which $A = \mathrm{sp}$
%
\begin{equation}
W^{\mathrm{sp}}_i(z) = b^{\mathrm{sp}}(z) \frac{H(z)}{c} n^{\mathrm{sp}}_{i}(z)\, .
\end{equation}
%
A plot of this function for the case of 4 spectroscopic redshift bins is shown in the middle panel of \figref{fig:ch4_weight_functions_plot}.

\begin{table}
\centering
\begin{tabular}{*{5}{C}}
\toprule
z_{i}^{-} & 0.90 & 1.10 & 1.30 & 1.50 \\
z_{i}^{+} & 1.10 & 1.30 & 1.50 & 1.80 \\
\midrule
b^{\rm sp}_i & 1.46 & 1.61 & 1.75 & 1.90 \\
\bottomrule
\end{tabular}
\caption{Tomographic binning and bias values for spectroscopic $\GCsp$ galaxy clustering.}
\label{tab:ch4_spectro_tomo_bins}
\end{table}

\subsection{Spectroscopic galaxy clustering: Fourier domain}
\label{sec:ch4_gcsp_pk}
In \citetalias{Blanchard:2019oqi} the spectroscopic galaxy clustering is treated by using the Fourier galaxy power spectrum $P_{\rm gg}(k, \mu ; z)$, where k is the modulus of the wave mode in Fourier space, and $\mu=\cos \theta=\boldsymbol{k} \cdot \hat{\mathbf{r}} / k$ is the cosine of the angle $\theta$ between the wave-vector $\boldsymbol{k}$ and the line-of-sight direction $\hat{\mathbf{r}}$. This section gives an overview of the Fisher matrix computation in the case of the 3D $\GCsp$. For further details refer to Sec.~3.2 in \citetalias{Blanchard:2019oqi}.

The main advantage of the Fourier power spectrum approach is that it significantly increases the constraining power of $\GCsp$ as a single probe with respect to the harmonic approach. This is because it allows us to include in a natural way a number of physical effects that carry cosmological information, e.g. the so-called {\it redshift space distortions} (RSD), which are instead neglected when treating $\GCsp$ in the harmonic domain. The full non-linear model for the observed power spectrum of the $\Halpha$ galaxies is given by the following equation:
%
\begin{equation}\label{eq:ch4_gcsp_pk_full_model}
\resizebox{0.45\textwidth}{!}{$
P_{\mathrm{obs}}\left(k_{\mathrm{ref}}, \mu_{\mathrm{ref}} ; z\right)=\frac{1}{q_{\perp}^{2} q_{\|}}\left\{\frac{\left[b \sigma_{8}(z)+f \sigma_{8}(z) \mu^{2}\right]^{2}}{1+\left[f(z) k \mu \sigma_{\mathrm{p}}(z)\right]^{2}}\right\} \frac{P_{\mathrm{dw}}(k, \mu ; z)}{\sigma_{8}^{2}(z)} F_{z}(k, \mu ; z)+P_{\mathrm{s}}(z)
$}
\end{equation}
%
The main physical effects included in this formula are:
%
\begin{itemize}
\item Anisotropies due to RSD: the peculiar velocity contributions to the observed redshifts induce anisotropies in the observed galaxy power spectrum.
This effect is encapsulated in the factor enclosed in curly braces in \eqref{eq:ch4_gcsp_pk_full_model}, where the denominator accounts for the so-called finger-of-God (FoG) effect by mean of the non-linear parameter $\sigma_{\rm p}(z)$.
\item Redshift uncertainty: despite being much more precise than the photometric redshift measurements, the spectroscopic redshifts are still affected by an uncertainty. This smears out the galaxy field along the line of sight, causing a partial suppression of the correlation between galaxy positions. This is included in the multiplicative term $F_{z}(k, \mu ; z)=\mathrm{e}^{-k^{2} \mu^{2} \sigma_{r}^{2}(z)}$.
\item Residual shot noise: this effect is modelled by the additive term $P_{\rm s}(z)$, and it accounts for the non-Poissonian component of the shot noise.
\item Alcock Paczynski (AP) projection effects: in order to convert redshifts into distances for the measurement of the galaxy power spectrum it is necessary to assume a reference cosmology. Choosing a reference cosmology which is not the true one results in a re-scaling of the components of the wave-vector $\boldsymbol{k}$ in the directions perpendicular and parallel to the line-of-sight. This is known as the Alcock Paczynski effect, which in \eqref{eq:ch4_gcsp_pk_full_model} is given by the multiplicative factor $1/(q_{\perp}^2 q_{\parallel})$, being $q_{\perp}$ and $q_{\parallel}$ the scaling factors of the transverse and radial components of the wave-vector respectively. The subscript ``ref'' for $k$ and $\mu$ in the left hand side of the equation means that $k$ and $\mu$ are considered in the reference cosmology.
\item Non-linear damping of BAO: another non-linearity effect that is taken into account is the damping of the BAO wiggles in the power spectrum, due to the late-time non-linearities. This is accounted for by using the so-called ``de-wiggled'' power spectrum $P_{\mathrm{dw}}(k, \mu ; z)$, which encapsulates an exponential damping factor of the BAO feature.
\end{itemize}
%
The Fisher matrix coming from the galaxy Fourier power spectrum $P_{\rm obs}$ is computed by summing up the contributions of the considered redshift bins. The Fisher matrix element for a bin centred at $z_i$ is
%
\begin{equation}
\resizebox{0.45\textwidth}{!}{$
F_{\alpha \beta}^{\mathrm{bin}}\left(z_{i}\right)=\frac{1}{8 \pi^{2}} \int_{-1}^{1} \mathrm{~d} \mu \int_{k_{\mathrm{min}}}^{k_{\max }} k^{2} \mathrm{~d} k\left[\frac{\partial \ln P_{\mathrm{obs}}\left(k, \mu ; z_{i}\right)}{\partial \alpha} \frac{\partial \ln P_{\mathrm{obs}}\left(k, \mu ; z_{i}\right)}{\partial \beta}\right] V_{\mathrm{eff}}\left(z_{i} ; k, \mu\right)
\, ,
$}
\end{equation}
%
where $V_{\mathrm{eff}}$ is the effective volume of the survey, defined as
%
\begin{equation}
V_{\mathrm{eff}}(k, \mu ; z)=V_{\mathrm{s}}(z)\left[\frac{n(z) P_{\mathrm{obs}}(k, \mu ; z)}{n(z) P_{\mathrm{obs}}(k, \mu ; z)+1}\right]^{2}\, ,
\end{equation}
%
and $n(z)$ is the number density of $\Halpha$ galaxies in each redshift bin
%
\begin{equation}
n(z)=\frac{\de N^{\rm sp}(z)}{\de \Omega \de z} \frac{A_{\rm survey}}{V_{\mathrm{s}}(z)} \Delta z\, .
\end{equation}
%
Finally the Fisher matrix is calculated by summing over the redshift bins:
%
\begin{equation}
F_{\alpha \beta}=\sum_{i=1}^{N_{z_{\text {bin }}}} F_{\alpha \beta}^{\text {bin }}(z_{i})\, .
\end{equation}





\subsection{Weak lensing}
\label{sec:ch4_wl}
As it is well known, the gravitational field of large-scale cosmic structure deflects the path of light rays emitted by distant galaxies, distorting the images of
the galaxies seen by the observers~\cite{Kilbinger2015,Kitching2017,Lemos2017}. At the linear level these distortions can be decomposed locally into convergence $\kappa$ and a (complex) shear $\gamma$, which are respectively related to the magnification and shape distortion of the image. In this work we will only consider the shear signal $\gamma$, treated in the harmonic domain with the Limber approximation \eqref{eq:ch4_limber_cls}. The corresponding weight function for cosmic shear is the following~\citetalias{Blanchard:2019oqi}
%
\begin{equation}\label{eq:ch4_shear_weight}
W_i^\gamma(z) = 
\frac{3}{2}\left(\frac{H_{0}}{c}\right)^{2} \Omm(1+z) \chi(z) \int_{z}^{z_{\rm max}} \de z'\, n^{\rm ph}_{i}(z')\left[1 - \frac{\chi(z)}{\chi(z')}\right]\, .
\end{equation}
%
Physically speaking, the integral  manifests that weak lensing is a cumulative effect, influenced by all the matter along the line of sight up to the considered redshift $z$.

The forecast also includes the \emph{intrinsic alignment} (IA), which is the main systematic effect altering weak lensing measurements~\cite{Joachimi2015,Kiessling2015,Kirk2015}. This is a physical phenomenon due to alignments of nearby galaxies caused by tidal interactions which occur during galaxy formation and evolution. It produces spurious correlations which affect the two-point correlation functions. The correlations caused by IA are indistinguishable to the ones produced by cosmic shear. 
Therefore, it is necessary to parameterise the IA effect on the lensing angular power spectrum. A possible way to do this is by using the extended non-linear alignment model~\cite{EuclidISTF2020,Bridle2007} which consists in the following modification of the cosmic shear weight function
%
\begin{equation}\label{eq:ch4_weak_lensing_full_weight}
W_{i}^{\rm wl}(z) = W_{i}^{\gamma}(z) - \mathcal{A}_{\mathrm{IA}} C_{\mathrm{IA}} \Omm \frac{H(z)\mathcal{F}_{\rm IA}(z)}{D(z)c} n^{\rm ph}_{i}(z)\, .
\end{equation}
%
In the above equation $D(z)$ is the growth factor introduced in \eqref{eq:ch1_transfer_growth_phi_def}, which can be directly computed from the linear power spectrum \eqref{eq:ch1_linear_pmm_expression}. The function $\mathcal{F}_{\rm IA}$ is defined as 
%
\begin{equation}\label{eq:ch4_FIA_def}
\mathcal{F}_{\rm IA}(z) \equiv (1+z)^{\etaIA}
\left[\frac{\langle L\rangle(z)}{L_{\star}(z)}\right]^{\betaIA}\, ,
\end{equation}
%
with $\langle L\rangle(z)$ and $L_{\star}(z)$ are the mean and characteristic luminosity functions respectively. The intrinsic alignment parameters $\aIA, \etaIA, \betaIA$ are treated as nuisance parameters in the analysis. The reference values for the IA parameters are the same adopted in~\citetalias{Blanchard:2019oqi}
%
\begin{equation}\label{eq:ch4_IA_parameters_values}
\left\{\aIA, \etaIA, \betaIA\right\}=\{1.72,-0.41,2.17\}
\end{equation}
%
The parameter $\CIA = 0.0134$ is instead fixed, since it is completely degenerate with $\aIA$. The scaled luminosity function $\langle L\rangle(z)/L_{\star}(z)$ is obtained via interpolation of its sampled values available at~\cite{ISTFPowerSpectra}.

==> input/2-Fisher.tex <==
\section{Fisher information matrix}
\label{sec:ch4_fisher}
The Fisher information matrix is defined as the expectation value of the hessian matrix of the log-likelihood:
%
\begin{equation}
F_{\alpha \beta} = -\left\langle\frac{\partial^{2} \ln L}{\partial \theta_\alpha \partial \theta_\beta}\right\rangle\, ,
\end{equation}
%
where $\alpha$ and $\beta$ are the parameter indices. The expected covariance matrix is the inverse of the Fisher matrix:
%
\begin{equation}
\mathcal{C}_{\alpha \beta}=\left(F^{-1}\right)_{\alpha \beta}\, .
\end{equation}
%
The diagonal elements of the covariance matrix are the squares of the marginalised $1\sigma$ uncertainties on the parameters, where $\sigma$ is the Gaussian standard deviation:
%
\begin{equation}
\sigma_{\alpha}=\sqrt{\mathcal{C}_{\alpha \alpha}}\, .
\end{equation}
%
The performances are quantified using the \emph{Figure-of-Merit} ($\FoM$) mentioned in \secref{sec:ch2_scientific_objectives}, which has been defined as in~\citetalias{Blanchard:2019oqi} 
%
\begin{equation}\label{eq:ch4_fom_def}
\FoM \equiv 
\sqrt{\operatorname{det}\left( \tilde{F}_{\wz\wa} \right)}
= \left[\sigma_{\wz}^2 \sigma_{\wa}^2 - \mathcal{C}^2_{\wz\wa}\right]^{-1/2}\, .
\end{equation}
%
The notation $\tilde{F}_{\wz\wa}$ denotes the Fisher information matrix relative to the dark energy equation of state parameters $\wz$ and $\wa$, marginalised over all the other free parameters. 
Note that the Cauchy-Schwarz inequality $\mathcal{C}_{\wz\wa} \leq \sigma_{\wz} \sigma_{\wa}$ guarantees that the argument of the square root is always greater than or equal to zero.
The value of the $\FoM$ can be boosted by small errors on $\wz$ and $\wa$ and/or by their cross-covariance $\mathcal{C}_{\wz\wa}$. The $\FoM$ is inversely proportional to the area of the $\onesigma$ marginalised contour ellipse in the $\wz\text{-}\wa$ plane. Tighter constraints on $\wz$ and $\wa$ lead to smaller ellipses, which in turn means higher FoMs.

\subsection{Fisher matrix from angular power spectra}
\label{sec:ch4_fisher_fullcl}
Under the assumption that the $a^{A}_{\ell m}$ of the observed fields follow a gaussian distribution, it can be shown that the corresponding Fisher matrix can be computed analytically. In this case the covariance matrix for the harmonic power spectra is
%
\begin{equation}\label{eq:ch4_4thorder_cov}
\operatorname{Cov} \left [ 
\cl{AB}{ij}{\ell}, \cl{CD}{km}{\ell'}
\right ] = \frac{\delta^{\rm K}_{\ell\ell'}}{2\ell+1}
\left  [
\sgl{AC}{ik}{\ell} \sgl{BD}{jm}{\ell'} +
\sgl{AD}{im}{\ell} \sgl{BC}{jk}{\ell'}
\right ]\, ,
\end{equation}
%
with $\delta^{\rm K}_{\ell\ell'}$ the Kronecker delta symbol, and
%
\begin{equation}
\sgl{AB}{ij}{\ell} = 
\frac{1}{\sqrt{f_{\rm sky} \Delta \ell}} \left ( \cl{AB}{ij}{\ell} + N_{ij}^{AB}(\ell)\right )\, ,
\end{equation}
%
The quantity $N^{AB}_{ij}(\ell)$ is the Poisson shot noise described later in \secref{sec:ch4_shot_noise}, $f_{\rm sky}$ is the sky fraction covered by the survey, and $\Delta \ell$ is the spacing between the multipoles in which the $C(\ell)$ are sampled.

In order to compute the Fisher matrix elements it is necessary to define a \emph{data-vector}, which contains the independent values of the $C(\ell)$'s to be include in the computation. In practice, since the tomographic angular power spectra are matrices, they need to be \emph{vectorised}\footnote{In this context the term ``vectorised'' refers to matrix vectorisation, which is defined in \secref{sec:apxA_linalg_tools}.} accordingly to their symmetry properties. For example the $\GCph$ auto-correlation $\cl{\phph}{ij}{\ell}$ at fixed  multipole $\ell$ is a $10\times 10$ symmetric matrix with $10(10+1)/2=55$ independent components. At fixed $\ell$ the data vector can be written in general as
%
\begin{equation}\label{eq:ch4_datavector_generic}
\mathbf{C}(\ell) = \left \lbrace
\mathbf{C}_1(\ell), \mathbf{C}_2(\ell), \dots, \mathbf{C}_\mathcal{N}(\ell)\right \rbrace\, ,
\end{equation}
%
where $\mathcal{N}$ is the number of the different types of $\mathbf{C}(\ell)$ according to the different probes considered in the analysis. When considering 3 probes at most -- $\WL$, $\GCph$, and $\GCsp$ -- the maximum number of angular power spectra that can be computed is $\mathcal{N}_{\rm max} = 6$. This is because there are $3$ possible auto-correlations and $3$ possible cross-correlations:
%
\begin{itemize}
\item auto-correlations: $\bcl{\wlwl}{\ell}$, $\bcl{\phph}{\ell}$, $\bcl{\phph}{\ell}$;
\item cross-correlations: $\bcl{\wlph}{\ell}$, $\bcl{\wlsp}{\ell}$, $\bcl{\phsp}{\ell}$.
\end{itemize}
%
The angular power spectra are evaluated in a finite number $N_{\ell}$ of multipoles, therefore the full data-vector $\mathcal{D}$ also includes all the values of the power spectra evaluated at all multipoles
%
\begin{equation}
\boldsymbol{\mathcal{D}} = 
\left \lbrace 
\bcl{}{\ell_1}, \bcl{}{\ell_2}, \dots,
\bcl{}{\ell_{N_\ell}} 
\right \rbrace\, .
\end{equation}
%
The covariance matrix associated to this data-vector is block diagonal, since the Kronecker delta of \eqref{eq:ch4_4thorder_cov} assures that different multipoles are uncorrelated
%
\begin{strip}
\begin{center}
\begin{equation}\label{eq:ch4_block_diag_multipole_covariance}
\resizebox{0.90\textwidth}{!}{$
\cov{\boldsymbol{\mathcal{D}}}{\boldsymbol{\mathcal{D}}} =
\begin{pmatrix}
\cov{\bcl{}{\ell_1}}{\bcl{}{\ell_1}} & 0 & \dots & 0 \\
0 & \cov{\bcl{}{\ell_2}}{\bcl{}{\ell_2}} & \dots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
0 & 0 & \dots & \cov{\bcl{}{\ell_{{N_\ell}}}}{\bcl{}{\ell_{N_\ell}}}
\end{pmatrix}\, .
$}
\end{equation}
\end{center}
\end{strip}
%
The generic diagonal block, $\cov{\bcl{}{\ell}}{\bcl{}{\ell}}$, accounts for all the correlations between the different kinds of $C(\ell)$'s included in the data-vector, and it is itself a block matrix
%
\begin{strip}
\begin{center}
\begin{equation}\label{eq:ch4_cov_matrix_generic_form}
\resizebox{0.90\textwidth}{!}{$
\cov{\mathbf{C}(\ell)}{\mathbf{C}(\ell)}
= \begin{pmatrix}
\cov{\mathbf{C}_1(\ell)}{\mathbf{C}_1(\ell)} & \cov{\mathbf{C}_1(\ell)}{\mathbf{C}_2(\ell)} &
\cdots & \cov{\mathbf{C}_1(\ell)}{\mathbf{C}_\mathcal{N}(\ell)} \\
\cov{\mathbf{C}_2(\ell)}{\mathbf{C}_1(\ell)} & \cov{\mathbf{C}_2(\ell)}{\mathbf{C}_2(\ell)} &
\cdots & \cov{\mathbf{C}_2(\ell)}{\mathbf{C}_\mathcal{N}(\ell)} \\
\vdots & \vdots & \ddots & \vdots \\
\cov{\mathbf{C}_\mathcal{N}(\ell)}{\mathbf{C}_1(\ell)} & \cov{\mathbf{C}_\mathcal{N}(\ell)}{\mathbf{C}_2(\ell)} &
\cdots & \cov{\mathbf{C}_\mathcal{N}(\ell)}{\mathbf{C}_\mathcal{N}(\ell)}
\end{pmatrix}\, ,
$}
\end{equation}
\end{center}
\end{strip}

%
where the single blocks $\cov{\mathbf{C}_i(\ell)}{\mathbf{C}_j(\ell)}$ are computed according to \eqref{eq:ch4_4thorder_cov}. 
With these definitions, the Fisher matrix element $F_{\alpha\beta}$ can be calculated as
%
\begin{equation}\label{eq:ch4_fisher_most_compact_form}
F_{\alpha\beta} = 
\pdv{\boldsymbol{\mathcal{D}}}{\theta_\alpha}
\invcov{\boldsymbol{\mathcal{D}}}{\boldsymbol{\mathcal{D}}}
\pdv{\boldsymbol{\mathcal{D}}}{\theta_\beta}
= \sum_{\ell = \ell_{1}}^{\ell_{N_{\ell}}}
F_{\alpha\beta}(\ell) \, ,
\end{equation}
%
where the second equality follows from the block diagonal form of the covariance, and the fisher matrix element\footnote{In this work the derivatives of the angular power spectra have been computed using the SteM numerical fitting procedure~\cite{Camera2017SKASystematics}.} at fixed $\ell$ is given by
%
\begin{equation}\label{eq:ch4_fisher_vec_4th_order_generic_fixed_ell}
F_{\alpha\beta}(\ell) = 
\pdv{\mathbf{C}(\ell)}{\theta_\alpha}^T
\cov{\mathbf{C}(\ell)}{\mathbf{C}(\ell)}^{-1}
\pdv{\mathbf{C}(\ell)}{\theta_\beta}\, .
\end{equation}


%
For later convenience, here are reported the adopted conventions for naming the Fisher matrices that have been computed in this work:
%
\begin{enumerate}
\item the name of a Fisher matrix is representative of the data vector, and it is composed by different labels, which identify the $C(\ell)$'s contained in the data-vector itself.
\item Within the name of a Fisher matrix, the auto-correlation $C^{\rm AA}(\ell)$ of the probe $\rm A$ is labeled simply as $\rm A$, while the cross-correlation $C^{\rm AB}(\ell)$ between the two probes $\rm A$ and $\rm B$ is denoted as $\xc{\mathrm{A}}{\mathrm{B}}$.
\item Square brackets are used to delimit the data-vector extent.
\item The pairwise cross-covariances between the $C(\ell)$'s included in a given data-vector are always taken into account in the computation of the corresponding Fisher matrix.
\item The sum of two Fisher matrices $[F_1]$ and $[F_2]$ is simply denoted by $[F_1] + [F_2]$. This simple sum corresponds to combine $[F_1]$ and $[F_2]$ without taking into account the cross-covariances between their data-vectors, i.e. it is an \emph{independent sum}.
\end{enumerate}
%
The simplest case of a Fisher matrix is when only the auto-correlation of a single probe $A$ is considered in the data-vector. 
For example, when say $A = \GCph$, the only observable that can be constructed is the auto-correlation of $A$ with itself. In this case the data-vector is simply
%
\begin{equation}
\mathbf{C}(\ell) = \left \lbrace \bcl{\phph}{\ell} \right \rbrace\, .
\end{equation}
%
Assuming $10$ tomographic bins for $\GCph$, the vector $\bcl{\phph}{\ell}$ will have $10(10+1)/2=55$ elements. Consequently the covariance matrix is made by a single $55\times 55$ block
%
\begin{equation}
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}}\, ,
\end{equation}
%
which takes into account the auto-covariance of $\GCph$ only. In this case, the Fisher matrix element from \eqref{eq:ch4_fisher_vec_4th_order_generic_fixed_ell} becomes
%
\begin{equation}
F^{[\GCph]}_{\alpha\beta}(\ell) = 
\left(\pdv{\bcl{\phph}{\ell}}{\theta_\alpha}\right)^T
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}}^{-1}
\pdv{\bcl{\phph}{\ell}}{\theta_\beta}\, ,
\end{equation}
%
or, in comma notation
%
\begin{equation}
F^{[\GCph]}_{\alpha\beta}(\ell) = 
\left[\bcl{\phph}{\ell}_{,\alpha}\right]^T
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}}^{-1}
\bcl{\phph}{\ell}_{,\beta}\, .
\end{equation}
%
When considering two or more probes, multiple combinations can be constructed, depending if \emph{cross-covariances} and \emph{cross-correlations} are included or not in the computation. In this work with the word ``cross-covariance'' are indicated the off-diagonal blocks of the covariance matrix \eqref{eq:ch4_cov_matrix_generic_form}, i.e. the blocks $\cov{\mathbf{C}_a(\ell)}{\mathbf{C}_b(\ell)}$ with $a \neq b$. The term ``cross-correlation'' (signal) is instead used to denote the data-vector entry corresponding to the correlation between two probes, which is therefore something carrying cosmological information.

In the following, the three possible combinations that can be constructed using two probes, $\rm A$ and $B$, are described in detail.

\subsubsection{Fisher matrix from two-probe combinations}
There are three possible angular power spectra that can be constructed from two probes $\rm A$ and $\rm B$:
%
\begin{itemize}
\item auto power spectrum of $\rm A$, $C^{\rm AA}(\ell)$;
\item auto power spectrum of $\rm B$, $C^{\rm BB}(\ell)$;
\item cross power spectrum between $\rm A$ and $\rm B$, $C^{\rm AB}(\ell)$.
\end{itemize}
%
As a concrete example, consider $\mathrm{A}=\GCph$ and $\mathrm{B}=\GCsp$.

\paragraph{Combining $\GCph$ and $\GCsp$ as independent probes}
When assuming $\GCph$ and $\GCsp$ to be independent, the resulting Fisher matrix will be given by the sum of the Fishers of the two single probes. According to the conventions explained above, the resulting Fisher is denoted as $[\GCph] + [\GCsp]$. This case is equivalent to build a data-vector including the two auto-correlations
%
\begin{equation}\label{eq:ch4_datavector_ph+sp}
\mathbf{C}(\ell) = 
\left\lbrace \bcl{\phph}{\ell}, \bcl{\spsp}{\ell} \right\rbrace \, .
\end{equation}
%
and setting to zero the off-diagonal blocks of the associated covariance matrix
%
\begin{equation}\label{eq:ch4_cov_ph+sp_indep}
\cov{\mathbf{C}(\ell)}{\mathbf{C}(\ell)} = 
\begin{pmatrix}
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}} & 0 \\[1ex]
0 & \cov{\bcl{\spsp}{\ell}}{\bcl{\spsp}{\ell}} 
\end{pmatrix}\, .
\end{equation}
%
This is equivalent to neglecting the cross-covariance between the auto-correlations of the two single probes, which is given by the block
%
\[
\cov{\bcl{\phph}{\ell}}{\bcl{\spsp}{\ell}}\, .
\]
%
Since the matrix in \eqref{eq:ch4_cov_ph+sp_indep} is block diagonal, its inverse will be of the same form~\cite{GuptaNagar}:
%
\begin{align}
\begin{pmatrix}
A & 0 \\[1ex]
0 & B
\end{pmatrix}^{-1} 
= 
\begin{pmatrix}
A^{-1} & 0 \\[1ex]
0 & B^{-1} 
\end{pmatrix}\, .
\end{align}
%
Therefore the matrix product entering the Fisher matrix element will be given by:
%
\begin{strip}
\begin{center}
\begin{equation}
\resizebox{0.90\textwidth}{!}{$
%\begin{split}
\begin{pmatrix}
\bcl{\phph}{\ell}_{,\alpha} & 
\bcl{\spsp}{\ell}_{,\alpha}
\end{pmatrix}
\begin{pmatrix}
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}}^{-1} & 0 \\[1ex]
0 & \cov{\bcl{\spsp}{\ell}}{\bcl{\spsp}{\ell}}^{-1} 
\end{pmatrix}
\begin{pmatrix}
\bcl{\phph}{\ell}_{,\beta} \\[1ex] 
\bcl{\spsp}{\ell}_{,\beta}
\end{pmatrix}\, .
%\end{split}
$}
\end{equation}
\end{center}
\end{strip}

%
And the resulting Fisher matrix element is
%
\begin{equation}
\begin{split}
F^{\GCph+\GCsp}_{\alpha\beta}(\ell) &=
\left[\bcl{\phph}{\ell}_{,\alpha}\right]^T
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}}^{-1}
\bcl{\phph}{\ell}_{,\beta} \\[1ex]
&+\left[\bcl{\spsp}{\ell}_{,\alpha}\right]^T
\cov{\bcl{\spsp}{\ell}}{\bcl{\spsp}{\ell}}^{-1}
\bcl{\spsp}{\ell}_{,\beta} \\[1ex]
&= F^{\GCph}_{\alpha\beta}(\ell) + F^{\GCsp}_{\alpha\beta}(\ell)\, .
\end{split}
\end{equation}
%
which is the simple sum of the fisher elements associated to the single probes.
%
\paragraph{Combining $\GCph$ and $\GCsp$ with cross-covariance}
The Fisher matrix in this case is denoted as $[\GCph+\GCsp]$. The data-vector is the same as the previous one \eqref{eq:ch4_data-vector_ph+sp}, but the off-diagonal blocks of the covariance matrix are taken into account
%
\begin{equation}\label{eq:ch4_cov_ph+sp_with_cov}
\resizebox{0.45\textwidth}{!}{$
\cov{\mathbf{C}(\ell)}{\mathbf{C}(\ell)} = 
\begin{pmatrix}
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}} &
\cov{\bcl{\phph}{\ell}}{\bcl{\spsp}{\ell}}\\[1ex]
\cov{\bcl{\spsp}{\ell}}{\bcl{\phph}{\ell}} & \cov{\bcl{\spsp}{\ell}}{\bcl{\spsp}{\ell}} 
\end{pmatrix}\, .
$}
\end{equation}
%
This matrix is not block-diagonal, hence, when inverting it, the blocks will mix with each other. There exist some formulas based on the Schur complement~\cite{GuptaNagar} for the inverse of a $2\times 2$ block matrix, but writing it down does not help to enlighten what happens in this case. From an intuitive point of view, the cross-covariance between two observables should worsen the constraints with respect to combining the two probes as independent. This can be understood with the following argument. If two observables exhibit a non-zero cross-covariance, there will be a mutual correlation between the two. In particular, a change in one of the two -- for example induced by a variation of the cosmological parameters -- will statistically induce a corresponding variation in the other. This in turn means that the two observables will share an amount of cosmological information, and therefore the total information coming from their combination will be \emph{less} than the direct sum of the two pieces of information carried individually by the two of them. More specifically, combining two correlated observables as if they were independent will end up in a double-counting of the same information, leading to an artificial improvement of the constraining power of their combination.
%
\paragraph{Combining $\GCph$, $\GCsp$ and their cross-correlation}
Here both the covariance and the cross-correlation between $\GCph$ and $\GCsp$ are taken into account. The resulting Fisher matrix is denoted as $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, and the data-vector includes accordingly the maximal set of the available $C(\ell)$'s
%
\begin{equation}\label{eq:ch4_datavector_ph+sp+xc}
\mathbf{C}(\ell) =
\left\lbrace 
\bcl{\phph}{\ell}, 
\bcl{\phsp}{\ell},
\bcl{\spsp}{\ell}
\right\rbrace\, ,
\end{equation}
%
and the covariance is the full $3\times 3$ block matrix associated to this data-vector
%
\begin{strip}
\begin{center}
\begin{equation}
\label{eq:ch4_cov_ph+sp+xc}
\resizebox{0.90\textwidth}{!}{$
\cov{\mathbf{C}(\ell)}{\mathbf{C}(\ell)} = 
\begin{pmatrix}
\cov{\bcl{\phph}{\ell}}{\bcl{\phph}{\ell}} &
\cov{\bcl{\phph}{\ell}}{\bcl{\phsp}{\ell}} &
\cov{\bcl{\phph}{\ell}}{\bcl{\spsp}{\ell}} \\[1ex]
\cov{\bcl{\phsp}{\ell}}{\bcl{\phph}{\ell}} &
\cov{\bcl{\phsp}{\ell}}{\bcl{\phsp}{\ell}} &
\cov{\bcl{\phsp}{\ell}}{\bcl{\spsp}{\ell}} \\[1ex]
\cov{\bcl{\spsp}{\ell}}{\bcl{\phph}{\ell}} &
\cov{\bcl{\spsp}{\ell}}{\bcl{\phsp}{\ell}} &
\cov{\bcl{\spsp}{\ell}}{\bcl{\spsp}{\ell}}
\end{pmatrix}\, .
$
}
\end{equation}
\end{center}
\end{strip}
%
In this case the new information coming from the cross-correlation is added to the data-vector, and this contribution is expected to tighten the resulting constraints with respect to the uncorrelated sum. In particular, the cross-correlation is itself a function of the cosmological parameters, meaning that its value will be sensitive to a variation of the parameters themselves. In this sense it is said that adding the \emph{cross-correlation signal} is expected to provide more cosmological information, therefore improving the combined constraints.
On the other hand, also all the cross-covariances between the $C(\ell)$'s are being considered in this case, and this will tend to worsen the constraints, as explained in the previous paragraph. So there are two concurring effects, and in principle it is not obvious which of them is dominant. The forecasts performed in my PhD Thesis show that the tightest constraints are actually obtained when both the cross-covariance and cross-correlation are included.
%

\subsection{Poisson shot noise}
\label{sec:ch4_shot_noise}
The Poisson shot noise~\cite{Baldauf2013} has been implemented in a similar way to what has been done in \citetalias{Blanchard:2019oqi}. It is assumed that only the auto-correlation $C(\ell)$'s are affected by a shot noise, which is independent of the multipole and is a tomographic diagonal matrix
%
\begin{equation}\label{eq:ch4_shotnoise_kronecker}
N^{AB}_{ij}(\ell) = \delta^{\rm K}_{AB} \delta^{\rm K}_{ij} N^{A}_{i}\, .
\end{equation}
%
So the definition of the noise is reduced to define the quantity $N^{A}_{i}$, which represents the shot noise associated to the probe $A$ at tomographic bin $i$. For photometric and spectroscopic galaxy clustering in the harmonic domain this is simply given by
%
\begin{align}\label{eq:ch4_gc_shot_noise}
N^{\rm ph}_{i} &\equiv \frac{1}{\int_{z_i^-}^{z_i^+} \de z\, \frac{\de N^{\rm ph}}{\de z \de \Omega}}\, ,
&
N^{\rm sp}_{i} &\equiv \frac{1}{\int_{z_i^-}^{z_i^+} \de z\, \frac{\de N^{\rm sp}}{\de z \de \Omega}}
\, .
\end{align}
%
For weak lensing the definition is instead given by the $\GCph$ shot noise multiplied by the variance $\sigma^2_\epsilon$ of the intrinsic galaxy ellipticity
%
\begin{equation}\label{eq:ch4_wl_shot_noise}
N^{\rm wl}_{i} \equiv \frac{\sigma^2_\epsilon}{\int_{z_i^-}^{z_i^+} \de z\, \frac{\de N^{\rm ph}}{\de z \de \Omega}}\, .
\end{equation}
%
The value assumed for $\sigma_\epsilon$ is $0.3$ as in \citetalias{Blanchard:2019oqi}.

As the Kronecker delta $\delta^{\rm K}_{AB}$ of \eqref{eq:ch4_shotnoise_kronecker} states, no shot noise has been considered for the cross-correlation $C(\ell)$'s. It is in fact commonly assumed for the noises of different tracers to be uncorrelated~\citetalias{Blanchard:2019oqi}. This approximation is expected to work well for the cross-correlation between weak lensing and galaxy clustering, since these are different tracers of the same underlying dark matter distribution.

In the cross-correlation of $\GCph$ with $\GCsp$ the tracers are the galaxies for both the probes, so in principle a shot noise on the cross power spectra (cross-noise) should be present. In this work we checked the $\delta^{\rm K}_{\rm ph sp}$ approximation of \eqref{eq:ch4_shotnoise_kronecker} with the following approach. Given that the Poisson shot noise affecting the two-point function comes from the count of galaxy \emph{self-pairs} -- see introduction of \cite{Baldauf2013} -- the cross-noise will be due to those galaxies which are in both the photometric and in the spectroscopic sample. The scenario with the highest noise is therefore the one in which the spectroscopic sample is a \emph{proper subset} of the photometric one. So, assuming this worst case scenario, a \emph{subtraction} of the spectroscopic galaxy distribution from the photometric one has been performed. After the subtraction there will be no more overlap between the two samples, and their cross-noise becomes zero by construction. It has been checked that the constraints do not change appreciably after the subtraction, with the FoM and the marginalised uncertainties of the free parameters being negligibly affected.

The shot noise affects in a direct way the diagonal covariance blocks corresponding to the auto-correlation power spectra, as it enters in all the factors of \eqref{eq:ch4_4thorder_cov}. This is what happens for example in the case of the auto-covariance of $\GCsp$
%
\begin{align}\label{eq:ch4_spsp_diag_cov_block}
\cov{\cl{\spsp}{ij}{\ell}}{\cl{\spsp}{km}{\ell}} 
\propto
&\left[\cl{\spsp}{ik}{\ell}) + N^{\spsp}_{ik}(\ell) \right] 
 \left[\cl{\spsp}{jm}{\ell}) + N^{\spsp}_{jm}(\ell)) \right] + \\
\notag
&\left[\cl{\spsp}{im}{\ell}) + N^{\spsp}_{im}(\ell) \right]
 \left[\cl{\spsp}{jk}{\ell}) + N^{\spsp}_{jk}(\ell)) \right]
\, .
\end{align}
%
However, the fact that the auto-correlation power spectra are contaminated by the shot noise indirectly alters also the other blocks of the covariance matrix. For example the diagonal block corresponding to the auto-covariance of $\bcl{\phsp}{\ell}$ reads
%
\begin{equation}\label{eq:ch4_phsp_diag_cov_block}
\resizebox{0.5\textwidth}{!}{$
\cov{\cl{\phsp}{ij}{\ell}}{\cl{\phsp}{km}{\ell}} 
\propto
\left[\cl{\phph}{ik}{\ell}) + N^{\phph}_{ik}(\ell) \right] \left [ \cl{\spsp}{jm}{\ell}) + N^{\spsp}_{jm}(\ell)) \right] +
\cl{\phsp}{im}{\ell} \cl{\phsp}{jk}{\ell}
$}\, ,
\end{equation}
%
and therefore also the terms coming from the inclusion of the $\xc{\GCph}{\GCsp}$ are affected by the shot noise of both $\GCph$ and $\GCsp$. Moreover, since the number of galaxies in the spectroscopic sample is $\sim 80$ times smaller than the galaxies in the photometric one, from \eqref{eq:ch4_gc_shot_noise} it is clear that the $\GCsp$ shot noise will be larger than the one associated to $\GCph$. In order to quantify the impact of the $\GCsp$ noise the forecast has been performed also in an unrealistic alternative scenario, where this noise is artificially reduced as if the number of spectroscopic galaxies were equal to the number of the photometric ones. This is done in practice by introducing an alternative reduced shot noise for $\GCsp$, defined as follows
%
\begin{equation}\label{eq:ch4_reduced_gcsp_noise}
\tilde{N}^{\rm sp}_{i}
\equiv \frac{N_{\rm sp}^{\rm tot}}{N_{\rm ph}^{\rm tot}}\cdot N^{\rm sp}_{i}\, ,
\end{equation}
%
where $N_{\rm sp}^{\rm tot}$ ($N_{\rm ph}^{\rm tot}$) is the total number of spectroscopic (photometric) galaxies, computed by integrating the galaxy distribution over its redshift range. As it is discussed in \secref{sec:ch4_results} it turns out that the results in the harmonic approach dramatically change using this reduced noise.

\subsection{Fisher matrix in the hybrid 2D-3D approach}
\label{sec:ch4_fisher_2dx3d}
As it has been already pointed out, in this work the observables adopted to compute the Fisher matrix are the angular power spectra. These are computed by mean of a projection on the sky of the galaxy density contrast. From a mathematical point of view, in the Limber approximation this translates into the computation of an integral in the radial direction. For weak lensing, this approach is the most natural one, since the deformation of the images of the source galaxies is a consequence of the cumulative effect of all the matter encountered by the light rays along the line of sight.

Treating also galaxy clustering with this approach allows us to compute cross-covariances and cross-correlation between the main probes in a straightforward way. The main disadvantage of treating the clustering signal in the harmonic domain is that the projection on the celestial sphere consists in a integral along the line of sight. Therefore this projection results in a partial loss of the information from the galaxy density distribution along the radial direction. This in turn ends up in a smaller constraining power from the projected galaxy clustering probe. For photometric clustering, $\GCph$, this loss is limited, since the redshift resolution is already hampered by the large photometric errors, and therefore one does not lose too much information when projecting transversely to the line of sight. Moreover, the constraining power of $\GCph$ is boosted by the large number of galaxies in the sample, and this is the main strength of the $\GCph$ probe.

In the spectroscopic sample there are instead fewer galaxies, and their redshifts are known with much better precision, which is the main strength of the spectroscopic clustering probe. Therefore the 2D projection results in a larger loss of constraining power from $\GCsp$. The tomographic technique can be employed in order to partially recover the radial information about the distances of the galaxies.

The most natural approach to treat $\GCsp$ is the one adopted in~\citetalias{Blanchard:2019oqi}, which has been briefly described in \secref{sec:ch4_gcsp_pk}, and here it is referred as ``3D'' or $P_k$. In this method the 3D galaxy power spectrum is used as the observable, which allows us to naturally exploit the high redshift resolution of the spectroscopic sample, thus significantly increasing the constraining power of $\GCsp$ alone. Nonetheless, in this case it is difficult to compute cross-correlations and cross-covariances between $\WL, \GCph$, and $\GCsp$. 

In this forecast we therefore considered two approaches to combine $\GCsp$ with $\WL$ and $\GCph$. The first is to treat all probes with the angular power spectra, as described in the previous section. In the second approach, which is the topic of this section, the Fisher matrix for the spectroscopic auto-correlation is not computed from the angular power spectra. The contribution of $\GCsp$ is considered by adding \emph{a posteriori} the Fisher matrix computed in the 3D approach of~\citetalias{Blanchard:2019oqi}, referred here as $\GCsp(P_k)$. This matrix has not been recomputed from scratch by implementing the recipe reported in \secref{sec:ch4_gcsp_pk}, instead the official results of~\citetalias{Blanchard:2019oqi} have been taken as external inputs. The advantage of this method is that it allows us to include the information coming from the cross-correlations between $\GCsp$ and the other probes in the angular domain, preserving at the same time the higher constraining power of the 3D approach for $\GCsp$. The main drawback is that it is an approximation. In fact, when adding the Fisher matrix of $\GCsp(P_k)$ a posteriori, the cross-covariances between the $\GCsp$ auto-correlation and the other observables are neglected.

In order to be more concrete, here it is reported the case of the combination of $\GCph$ with $\GCsp$. The starting point is to include only the harmonic $\GCph$ auto-correlation and the harmonic $\GCph\times\GCsp$ cross-correlation in the data-vector
%
\begin{equation}
\mathbf{C}(\ell) = \left \lbrace
\bcl{\phph}{\ell}, \bcl{\phsp}{\ell}
\right \rbrace \, .
\end{equation}
%
Consequently, the covariance matrix is built considering only the upper left sector of \eqref{eq:ch4_cov_ph+sp+xc}. The Fisher matrix element is computed with the usual formula \eqref{eq:ch4_fisher_most_compact_form}, and we refer to the resulting matrix with the notation $[\GCph+\xc{\GCph}{\GCsp}]$. Finally, the Fisher matrix of $\GCsp(P_k)$ is simply added via a sum
%
\begin{fullpageequation}
\resizebox{0.80\textwidth}{!}{$
F_{\alpha\beta}[\GCph+\xc{\GCph}{\GCsp}\, + \, \GCsp(P_k)] = 
F_{\alpha\beta}[\GCph+\xc{\GCph}{\GCsp}] + F_{\alpha\beta}[\GCsp(P_k)]\, .
$}
\end{fullpageequation}
%
This procedure is equivalent to neglecting the covariance terms between the $\GCsp$ auto-correlation and the other observables, and performing the computation by using a covariance matrix that can be symbolically written as
%
\begin{equation}
\begin{pmatrix}
\cov{\phph}{\phph} & \cov{\phph}{\phsp} & 0 \\
\cov{\phsp}{\phph} & \cov{\phsp}{\phsp} & 0 \\
0 & 0 & \cov{\spsp}{\spsp} \\
\end{pmatrix} \, .
\end{equation}
%
The upper left $2\times 2$ sector contains the covariances between the elements of the $\cl{\phph}{}{\ell}$ and $\cl{\phsp}{}{\ell}$ matrices, organised in block-diagonal form for all multipoles as in \eqref{eq:ch4_block_diag_multipole_covariance}. Analogously, the lower right corner block represents the auto-covariance of the spectroscopic galaxy Fourier power spectrum for all wave-numbers and redshifts considered. The zeroes correspond to the elements containing the unknown covariances between the 2D and 3D power spectra, which are therefore neglected.


==> input/3-Results.tex <==
% Forecast settings table
%-----------------------------------------%
\begin{table*}[]
\centering
\begin{tabular}{llll}
\toprule
\multicolumn{4}{c}{Forecast settings in the harmonic approach} \\
\midrule
\multirow{6}{*}{Multipoles settings} & \multirow{3}{*}{Optimistic} & $\GCph$ & $10 \leq \ell \leq 3000$ \\
 & & $\GCsp$ & $10 \leq \ell \leq 3000$ \\
 & & $\WL$ & $10 \leq \ell \leq 5000$ \\[1ex]
 & \multirow{3}{*}{Pessimistic} & $\GCph$ & $10 \leq \ell \leq 750$ \\
 & & $\GCsp$ & $10 \leq \ell \leq 750$ \\
 & & $\WL$ & $10 \leq \ell \leq 1500$ \\
 \midrule
\multirow{4}{*}{General settings} & \multirow{2}{*}{Baseline} & $\GCph$ & all the $10$ bins of \tabref{tab:ch4_photo_tomo_bins} \\
 & & $\GCsp$ & reduced shot noise \eqref{eq:ch4_reduced_gcsp_noise} \\[1ex]
 & \multirow{2}{*}{Alternative} & $\GCph$ & only $4$ bins of \tabref{tab:ch4_photo_tomo_bins} with $z_i^-, z_i^+ \in [0.9, 1.8]$\\
 & & $\GCsp$ & reduced shot noise \eqref{eq:ch4_reduced_gcsp_noise}\\
\bottomrule
\end{tabular}
\caption{Summary of the setting scenarios considered in the forecast. For $\WL$ the general settings are not reported since no distinction other than the multipole range has been made. The scenario in which the $\GCsp$ shot noise is reduced \emph{is not intended to be realistic}, and has been studied only to probe the theoretical limitations of the harmonic approach.}
\label{tab:ch4_scenarios_settings}
\end{table*}
%-----------------------------------------%
\section{Results}
\label{sec:ch4_results}
In this section the results of the forecast are presented. As a convention, the reported marginalised $\onesigma$ uncertainties are always fractional, i.e. divided by the values of the parameters in the reference cosmology in \tabref{tab:ch4_cosmo_pars_fiducials}. The only exception are the contour plots, which are drawn using the original values of the uncertainties computed via \eqref{eq:ch4_marg_sigma_def}. In order to quantitatively assess the impact of cross-covariances and cross-correlations on the forecasts, the corresponding percentage variations of the parameter constraints are plotted with vertical bars. This is done both for the FoM and the relative $\onesigma$ uncertainty, using the following formula
%
\begin{equation}\label{ch4:perc_diff_definition}
\delta X\,[\%] \equiv 100 \cdot \frac{X_{b} - X_{a}}{X_{a}}\, ,
\end{equation}
%
where $X$ generically denotes the FoM or the relative uncertainty $\sigma_{\theta}/\theta_{\rm fid}$. The subscript $a$ denotes the Fisher matrix whose constraints are used as reference, while $b$ is the Fisher matrix under examination, also referred as the \emph{minuend} in the following.

This section is organised as follows. \secref{sec:ch4_results_settings} reports the different scenarios and settings with which the forecast has been performed. 
In \secref{sec:ch4_results_phxsp} the results from the combination of $\GCph$ and $\GCsp$ are presented. Also a comparison is made between $\GCph$ and $\GCsp$ when treated in the harmonic domain.
In \secref{sec:ch4_results_wlxsp} the results are reported for the combination of $\WL$ and $\GCsp$, also comparing the impact on the constraints from $\xc{\WL}{\GCsp}$ against $\xc{\WL}{\GCph}$.
Finally in \secref{sec:ch4_results_6x2pt} the constraints coming from the combination of the full set of \Euclid main probes are shown, focusing on the importance of cross-covariances and cross-correlations between $\GCsp$ and $\WL, \GCph$. In this last section the results of the so-called \Euclid $\sixtwoptShort$ statistics are reported; with this term it is meant the combination of the all possible two-point functions that can be constructed from $\WL, \GCph$, and $\GCsp$. Using the naming convention for the Fisher matrices introduced in \secref{sec:ch4_fisher}, the \emph{harmonic} $\sixtwoptShort$ statistics results are explicitly denoted by
%
\begin{fullpageequation}\label{eq:ch4_6x2pt_harmonic_def}
\resizebox{0.9\textwidth}{!}{$
[(\text{harmonic})\, \sixtwoptShort] \equiv [\sixtwoptLong]\, .
$}
\end{fullpageequation}
%
Here the word ``harmonic'' indicates that all the observables are treated using the angular power spectrum formalism. The corresponding notation of the $\sixtwoptShort$ statistics results in the hybrid approach is
%
\begin{fullpageequation}\label{eq:ch4_6x2pt_hybrid_def}
\resizebox{0.9\textwidth}{!}{$
[(\text{hybrid})\, \sixtwoptShort] \equiv [\WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]\, .
$}
\end{fullpageequation}
%
Therefore, in the hybrid $\sixtwoptShort$ approach everything is treated using $C(\ell)$'s except for the spectroscopic auto-correlation, whose Fisher matrix is added a posteriori and computed via the full, anisotropic, and redshift-dependent galaxy power spectrum as described in \secref{sec:ch4_gcsp_pk}.

\subsection{\large{Settings description}}
\label{sec:ch4_results_settings}
The scenarios considered in this forecast are summarised in \tabref{tab:ch4_scenarios_settings}. Regarding the multipole range, two scenarios have been studied: one \emph{optimistic} and one \emph{pessimistic}. In the optimistic scenario the multipole range for $\GCph$ and $\GCsp$ (in the harmonic domain) is set to $\ell \in [10, 3000]$, while it is $\ell \in [10, 5000]$ for $\WL$. In the pessimistic scenario instead the multipole range is $\ell \in [10, 750]$ for $\GCph$, $\GCsp$ (in the harmonic domain), and $\ell \in [10, 1500]$ for $\WL$. 

For galaxy clustering one more assumption has been made, in order to better understand the differences between $\GCph$ and $\GCsp$ when both are treated in the harmonic domain. For $\GCsp$ the alternative reduced shot noise described in \secref{sec:ch4_shot_noise} has been employed, in order to assess its impact on the results. However it is important to stress that this scenario in which the $\GCsp$ shot noise has been reduced \emph{is not meant to be realistic}. It has been considered only to understand the reason for the different constraining power of the $\GCsp$ and $\GCph$ probes. 
%to probe the theoretical limitations of the $C(\ell)$ formalism when applied to $\GCsp$. 
For the same reason, in the case of photometric clustering the analysis has been performed using also an alternative tomographic binning, where only the $4$ photometric bins entirely comprised in the redshift range $z \in [0.9, 1.8]$ are considered. This has been done in order to make both $\GCph$ and $\xc{\WL}{\GCph}$ comparable with $\GCsp$ and $\xc{\WL}{\GCsp}$ respectively. In fact, apart from the shape of the galaxy distribution and the values of the galaxy bias, in the harmonic domain the two main differences between $\GCph$ and $\GCsp$ are the shot noise and the redshift range of the galaxy catalogue. As said in \secref{sec:ch4_shot_noise}, the shot noise of $\GCsp$ is much larger than the $\GCph$ one, since the spectroscopic sample has 80 times fewer galaxies than the photometric one. Moreover, the redshift range covered by the photometric galaxy distribution is $[0.001, 2.5]$, while for the spectroscopic galaxy distribution it is limited to $z \in [0.9, 1.8]$ due to the wavelength range in which NISP is sensitive.

\subsection{\large{Combining photometric and spectroscopic clustering}}
\label{sec:ch4_results_phxsp}

% TABLE GCphxGCsp: FoM
%-----------------------------------------%
\begin{table*}[t]
\centering
\begin{resultstable}{CL*{3}{C}}
\multicolumn{5}{c}{$\GCph\times\GCsp$ FoM results} \\
\midrule
\GCsp\, \text{bins} & \text{Fisher matrix} & \FoM & \Delta\FoM & \Delta\FoM(\%)\\
\midrule
\text{--} & [\GCph] & 63.12 & \text{--} & \text{--} \\
 \midrule
\multirow{4}{*}{4}
& [\GCph] + [\GCsp(P_k)]                   & 230.27 & \text{--} & \text{--} \\
& [\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)] & 234.54 & \text{--} & \text{--} \\
& [\GCph] + [\GCsp]                        & 65.69  & \text{--} & \text{--} \\
& [\GCph+\GCsp]                            & 63.95  & -1.75 & \negative{-2.66\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}]          & 69.63  & +3.94 & \positive{+6.00\%} \\
\midrule
\multirow{4}{*}{12}
& [\GCph] + [\GCsp] & 72.02 & \text{--} & \text{--}\\
& [\GCph+\GCsp] & 70.48 & -1.55 & \negative{-2.15\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 79.87 & +7.85 & \positive{+10.90\%} \\
\midrule
\multirow{4}{*}{24}
& [\GCph] + [\GCsp] & 85.02 & \text{--} & \text{--}\\
& [\GCph+\GCsp] & 83.88 & -1.13 & \negative{-1.33\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 108.35 & +23.34 & \positive{+27.45\%}\\
\midrule
\multirow{4}{*}{40}
& [\GCph] + [\GCsp] & 111.22 & \text{--} & \text{--} \\
& [\GCph+\GCsp] & 110.39 & -0.83 & \negative{-0.75\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 153.71 & +42.48 & \positive{+38.20\%} \\
\end{resultstable}
\caption{Table reporting the $\FoM$ for $\GCph$, $\GCsp$ and their cross-correlation.
The $\Delta\FoM$ column contains the variation of the figure of merit with respect to the independent sum $[\GCph] + [\GCsp]$ for the given number of bins. The $\Delta\FoM (\%)$ column is calculated by taking $\Delta\FoM$ as a percentage of the FoM of $[\GCph] + [\GCsp]$.}
\label{tab:ch4_results_phsp_fom}
\end{table*}
%-----------------------------------------%

In this section we report the results for the combination of $\GCph$ and $\GCsp$. As said above, in this case the Fisher matrix in the harmonic approach is denoted as $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, while in the hybrid one as $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$. In the following we discuss the impact on the constraints given by the inclusion of the $\GCph$-$\GCsp$ cross-covariance and the $\xc{\GCph}{\GCsp}$ cross-correlation. In this section, we take as reference values for the percentages the constraints coming from the independent combination of $\GCph$ and $\GCsp$, that is $[\GCph]+[\GCsp]$ in the harmonic approach and $[\GCph]+[\GCsp(P_k)]$ in the hybrid one. The results for this combination are reported in the optimistic scenario only for brevity.

% PERC. DIFF. PLOT GCphxGCsp: FULL CL
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=0.80\textwidth]{Figures/optimistic/perc_diff_errors/GCphGCsp_cov_and_xc_impact.pdf}
\caption{Impact, on $\onesigma$ parameter errors and $\FoM$, of cross-covariance and cross-correlation in the harmonic approach for the combination of $\GCph$ and $\GCsp$. The left panel shows the impact of the cross-covariance, quantified with the percentage differences between $[\GCph+\GCsp]$ and $[\GCph] + [\GCsp]$. In the right panel the impact of the cross-correlation is reported, quantified by percentage differences of $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$ with respect to $[\GCph]+[\GCsp]$.}
\label{fig:ch4_phsp_fullcl_percdiff_plot}
\end{figure*}

\subsubsection{Impact of the $\bGCph$-$\bGCsp$ cross-covariance on parameter constraints}
According to the notation convention defined in \secref{sec:ch4_fisher_fullcl}, in the case of the cross-covariance alone, the Fisher matrix $[\GCph+\GCsp]$ is computed in the harmonic domain by taking into account only the cross-covariance between $\GCph$ and $\GCsp$. The notation $[\GCph] + [\GCsp]$ represents instead the simple sum of the Fisher matrices of the two probes, which does not take the cross-covariance into account. From \tabref{tab:ch4_results_phsp_fom} it can be seen that in any case the cross-covariance slightly worsens the FoM, as expected. 
Anyway the contribution is always smaller than $3\%$, in particular it is $-2.66\%$ with $4$ bins and $-0.75\%$ with $40$ bins used for $\GCsp$. This decreasing trend can be understood as follows: the finer the tomographic binning of $\GCsp$ the smaller the support of the integrand of the off-diagonal terms $\bcl{\phsp}{\ell}$. Intuitively, the value of the integral over each of the $4$ thick bins is diluted into more thinner bins when a finer binning is used. Hence the off-diagonal block $\cov{\bcl{\phph}{\ell}}{\bcl{\spsp}{\ell}}$ and its transposed counterpart become larger and sparser as the number of bins is increased, and therefore the cross-covariance contribution becomes smaller. Physically this could be understood considering that for 40 bins the loss of information due to the projection transversely to the line of sight is less severe than for 4 bins only.

The same trend is observed also for the marginalised uncertainties on the cosmological parameters, as it can be seen by \figref{fig:ch4_phsp_fullcl_percdiff_plot}, where the percentage difference between the uncertainties, as defined in \eqref{ch4:perc_diff_definition}, are drawn as vertical bars. In particular, the impact of the cross-covariance is shown in the left panel as the comparison between $[\GCph+\GCsp]$ and $[\GCph]+[\GCsp]$, taking this last as reference. The parameters mostly affected by the covariance are $\Omb$ and $\h$, whose constraints in the 4 bin setting worsen by $4\%$ and $6\%$ respectively. However, as soon as the binning is refined, the effect gets smaller, becoming about $0.9\%$ for $\Omb$ and $2.5\%$ for $h$. The uncertainties on $\Omm$, $\ns$, and $\sige$ are instead affected by less than $2\%$ for all the binning settings. This outcome is confirmed also by \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}, which reports the relative marginalised uncertainties and the FoM as horizontal bars. The $[\GCph+\GCsp]$ bars (in blue) always have practically the same length as the $[\GCph] + [\GCsp]$ bars (in cyan), and they look more and more similar as the number of $\GCsp$ bins increases. 

In conclusion the cross-covariance between $\GCph$ and $\GCsp$ can be considered negligible, as it does not change the uncertainties on the cosmological parameters by more than $6\%$ and the FoM by more than $3\%$.

% GCphxGCsp: hybrid XC impact
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.60\textwidth]{Figures/optimistic/perc_diff_errors/phsp_hybrid_xc_impact.pdf}
\caption{Impact, on FoM and marginalised $\onesigma$ errors, of the $\xc{\GCph}{\GCsp}$ in the hybrid approach, for the optimistic scenario. The reference here are the constraints coming from $[\GCph]+[\GCsp(P_k)]$, while the minuend for the percentage difference is $[\GCph+\xc{\GCph}{\GCsp}]+[\GCsp(P_k)]$. Note that in the hybrid approach only $4$ tomographic bins were used to compute the $\xc{\GCph}{\GCsp}$ angular power spectra, for consistency with the Fourier power spectrum analysis.}
\label{fig:ch4_phsp_hybrid_xc_impact}
\end{figure*}
%-----------------------------------------%

\subsubsection{\large{Impact of the $\bxc{\bGCph}{\bGCsp}$ signal on parameter constraints}}

\paragraph{Harmonic approach}

In the harmonic approach the contribution to the FoM coming from the $\xc{\GCph}{\GCsp}$ cross-correlation is always positive, as reported in \tabref{tab:ch4_results_phsp_fom}, and it is about $6\%$ $(38\%)$ with $4$ $(40)$ bins for $\GCsp$. This gain is visible also in \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}, where the FoM and the marginalised uncertainties from the  $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$ Fisher matrix are represented with green bars. The improvements on the errors for $\wz, \wa$, and consequently on the FoM, are particularly visible for finer binnings, coherently with the results reported in the table. 

The marginalised uncertainties on the cosmological parameters also improve when including the $\mathrm{XC}$ signal, but the gain is more modest than the one on the FoM, as it is shown in the right panel of \figref{fig:ch4_phsp_fullcl_percdiff_plot}. In fact, the biggest improvements are for $\wz$ and $\wa$, whose uncertainties get smaller at most by $23\%$ and $25\%$, respectively. Instead, the uncertainty on the baryon density parameter, $\Omb$, slightly increases by about $1\%$ with 4 bins and becomes smaller by $18\%$ with 40 bins. The small worsening on this parameter in the case of 4 bins has been attributed to the contribution of the cross-covariances between the $C(\ell)$'s included in the data-vector of the Fisher matrix $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, which are not taken into account in the simple sum $[\GCph] + [\GCsp]$. It is possible that with 4 bins the gain coming from the inclusion of the $\rm XC$ signal is compensated by the covariance contribution, producing a net (small) worsening. However, as soon as the number of $\GCsp$ bins increases, the positive contribution of the cross-correlation signal starts to dominate, and the constraints on $\Omb$ to improve too.
The uncertainties on the other parameters also improve, in particular $\Omm$ and $\sige$ gain at most $12\%$ when $40$ bins are used, as well as $\h$ and $\ns$ which improve by $7\%$ at maximum.

% GCphxGCsp, hybrid vs harmonic: % diff barplot
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\textwidth]{Figures/optimistic/perc_diff_errors/phsp_hybrid_vs_harmonic.pdf}
\caption{Percentage difference between FoM and marginalised $\onesigma$ errors of the hybrid and harmonic approaches, for the combination of $\GCph$ and $\GCsp$ in the baseline optimistic scenario. The percentage differences are normalised to the results of the harmonic approach.}
\label{fig:ch4_phsp_hybrid_vs_harmonic}
\end{figure*}
%-----------------------------------------%

\paragraph{Hybrid approach}
In the hybrid approach instead, the $\xc{\GCph}{\GCsp}$ has quite a small impact on the constraints: the marginalised uncertainties and FoM from the  $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$ Fisher matrix are very similar to the ones from $[\GCph] + [\GCsp(P_k)]$, as it is qualitatively shown by the contour plots in \figref{fig:ch4_contour_w0wa_phsp_fullcl_vs_2dx3d} and from the barplots in \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}. A more detailed analysis is reported in \figref{fig:ch4_phsp_hybrid_xc_impact}, where the percentage variations on the constraints resulting from adding the $\xc{\GCph}{\GCsp}$ are shown. The variation on the FoM is comprised between $+1.5\%$ and $+2\%$, so there is a very small improvement when including $\xc{\GCph}{\GCsp}$ in the hybrid approach. This is also the case for the marginalised uncertainties which improve less than $1\%$. 
Therefore, it can be concluded that, in the hybrid approach, the inclusion of the $\xc{\GCph}{\GCsp}$ cross-correlation in the combination of $\GCph$ and $\GCsp$ has a negligible impact on the results.

\subsubsection{Hybrid approach vs harmonic approach}
As \figref{fig:ch4_phsp_hybrid_vs_harmonic} shows, the hybrid approach performs better than the harmonic one in constraining almost all the cosmological parameters, even if the constraining power of the harmonic approach significantly improves with increasing the number of $\GCsp$ tomographic bins. The harmonic approach has a FoM of $69$ ($153$) for $4$ ($40$) spectroscopic bins, while the hybrid one provides a FoM of $234$, which is $236\%$ ($52\%$) larger than in the former case. Thus the hybrid approach is better even when $40$ spectroscopic bins are used for the harmonic one. In particular, this is true for the reduced Hubble constant $h$. In this case the hybrid approach performs remarkably better, with a gain on the marginalised uncertainty which is always between $75\%$ and $100\%$, depending only slightly on the number of $\GCsp$ bins used for the harmonic approach. This is expected, since the hybrid approach takes advantage of the 3D power spectrum as an observable, in which radial BAO and RSD are included. The constraints on the other parameters appear instead quite sensitive to the $\GCsp$ binning. The differences on the $\wz$ and $\wa$ uncertainties significantly decrease from more than $50\%$ with $4$ bins to about $20\%$ with $40$ bins, as it could be expected from the FoM differences between the hybrid approach and the harmonic one. For $\Omm$, and $\sige$ the hybrid approach is still better than the harmonic one, even if the difference between the two approaches decreases significantly with the number of bins too.

The only exceptions are given by the baryon density, $\Omb$, and the spectral index, $\ns$. In particular, the $\Omb$ uncertainty from the hybrid approach is more than $25\%$ smaller than from the harmonic one with $4$ spectroscopic bins, but the situation gets reversed with $40$ bins. In the latter case the harmonic approach provides $\sim 10\%$ better constraints on $\Omb$ than the hybrid one. The $\ns$ uncertainty in the harmonic approach with $4$ bins is about $20\%$ larger than in the hybrid one. Instead, when $40$ bins are used for the harmonic approach, the $\ns$ uncertainty given by the hybrid approach is a few percents larger than the one given by the former.

To conclude, for the combination of $\GCph$ and $\GCsp$, the hybrid approach always provides better constraints than the harmonic one. Increasing the number of bins of the harmonic approach improves its performances. Using $40$ bins allows us to reach the performances of the hybrid approach for some parameters -- $\ns$ and $\Omb$ -- but a large gap still remains for the other constraints, especially for $h$ and the FoM.

% FoM Gain PLOT GCphxGCsp
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.80\textwidth]{Figures/optimistic/fom_gain/phsp_fom_gain.pdf}
\caption{Percentage gain on the FoM relative to photometric clustering alone ($[\GCph]$). In the left panel the computation has been done using the standard $\GCsp$ shot noise \eqref{eq:ch4_gc_shot_noise}, while in the right panel the reduced version \eqref{eq:ch4_reduced_gcsp_noise} has been used.}
\label{fig:ch4_phsp_fom_gain}
\end{figure*}
%-----------------------------------------%

\subsubsection{Comparing photometric and spectroscopic clustering in the harmonic domain}
As anticipated in \secref{sec:ch4_results_settings} two alternative configurations have been considered both for $\GCph$ and $\GCsp$. The baseline configuration for $\GCph$ consists in using all the $10$ redshift bins reported in \tabref{tab:ch4_photo_tomo_bins}, while in the alternative configuration only the $4$ bins strictly contained in the range $[0.9, 1.8]$ are considered. For spectroscopic clustering instead the baseline settings correspond to use the shot noise as calculated from the second equation of \eqref{eq:ch4_gc_shot_noise}, while the alternative consists in using the artificially reduced version \eqref{eq:ch4_reduced_gcsp_noise} of the noise. In fact, from further investigation it turned out that a great limitation of the harmonic approach is due to the shot noise associated to the $\GCsp$ auto-correlation $C(\ell)$'s. This is in fact much higher than the one associated to $\GCph$, since the expected number of $\Halpha$-emitting galaxies in the \Euclid catalogue ($\sim \num{2e7}$) is smaller than the expected number of galaxies in the photometric sample ($\sim \num{1.6e9}$). Therefore, in order to quantify the impact of the spectroscopic shot noise, the forecast has been performed also in the artificially reduced shot noise setting, as explained in \secref{sec:ch4_shot_noise}. 
The results are shown in \figref{fig:ch4_phsp_fom_gain}: in the left panel the standard $\GCsp$ shot noise computed from \eqref{eq:ch4_gc_shot_noise} is employed, while in the right one the reduced noise \eqref{eq:ch4_reduced_gcsp_noise} is used. From the panels it is manifest that lowering the shot noise systematically boosts the results of the harmonic approach by about one order of magnitude, making its performance comparable or even better than in the hybrid case. In particular, as it can be expected, the observable which most improves its performance thanks to the noise reduction is the harmonic $\GCsp$ auto-correlation. Instead, the $\xc{\GCph}{\GCsp}$ is not affected as the shot noise does not enter its definition, as can be observed from \eqref{eq:ch4_shotnoise_kronecker}. 
% GCph vs GCsp in various settings
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.70\textwidth]{Figures/optimistic/gcph_vs_gcsp.pdf}
\caption{Comparison between the constraints coming from $[\GCph]$ and $[\GCsp]$ in the harmonic approach, in the different configurations described in \secref{sec:ch4_results_settings}. The scale on the vertical axis is logarithmic to make visible both the relative marginalised uncertainties and the FoM in the same plot.}
\label{fig:ch4_gcph_vs_gcsp_harmonic}
\end{figure*}
%-----------------------------------------%

Instead, when considering the behaviour of the $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$ Fisher matrix, as compared to the corresponding one in the harmonic domain, its performance remains stable against the change of the shot noise level, since the possible change of the latter would enter only $\GCsp(P_k)$, which is a fixed external input. Therefore, while in the harmonic case the survey performance increases with the noise reduction and the increasing of the number of spectroscopic bins, in the hybrid case the performance stay unchanged since both the noise level and the bin number are fixed to the values of the external input.

It is important to stress that the condition of reduced shot noise for $\GCsp$ \emph{is not realistic}, since it is realised only if the number of galaxies in the spectroscopic sample equals the number of the photometric one, which is not the case. This check has been done in order to better understand the limitations of $\GCsp$ in the harmonic approach.

The results of considering the same shot noise level and redshift range for $\GCsp$ and $\GCph$ are reported in \figref{fig:ch4_gcph_vs_gcsp_harmonic}. The height of the bars labeled with the cosmological parameters is equal to the relative marginalised uncertainty for that particular parameter. Regarding the FoM the height is instead given by the value of the FoM itself. From the plot it is evident that the constraints coming from $\GCph$ restricted to the $4$ bins in the spectroscopic range (blue bars) are very close to the ones of $\GCsp$ when the shot noise is reduced (yellow bars). Thus in these special conditions the two probes are essentially equivalent. This is expected, since the functional form of the weight for galaxy clustering is always the same, with the photometric function $W_i^{\rm ph}$ differing from the spectroscopic one $W_i^{\rm sp}$ only for the shape of the galaxy distribution and the values of the galaxy bias.

\figref{fig:ch4_gcph_vs_gcsp_harmonic} shows also the two probes in the baseline configuration, in which the $10$ bins listed in \tabref{tab:ch4_photo_tomo_bins} are used for $\GCph$ (red bars) and the more realistic shot noise \eqref{eq:ch4_gc_shot_noise} is used for $\GCsp$ (green bars). On the one hand, the usage of all bins for $\GCph$ makes a big difference, improving the FoM by a factor of $\sim 30$ and reducing the uncertainties of about one order of magnitude on average. On the other hand, the realistic shot noise of $\GCsp$ significantly affects its performances, reducing the FoM by a factor of $\sim 10$ and making the uncertainties larger.

The conclusion is therefore that the shot noise and the redshift range of the galaxy sample are what makes the difference between $\GCph$ and $\GCsp$ in terms of constraining power, when both are treated in the harmonic domain. When $\GCph$ is restricted to the same range of $\GCsp$ and the shot noise of the latter is reduced to the same level of the former, their constraints become comparable with each other.

%------CONTOUR GCphxGCsp-----------------%
\begin{figure*}[h!]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.75\textwidth]{Figures/optimistic/contours/phsp/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf} \\
\includegraphics[width=0.75\textwidth]{Figures/optimistic/contours/phsp/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the combination of $\GCph$ and $\GCsp$.}
\label{fig:ch4_contour_w0wa_phsp_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%

% ERROR BARPLOT GCphxGCsp
%-----------------------------------------%
\begin{figure*}[h!]
\centering
\includegraphics[width=0.80\textwidth]{Figures/optimistic/error_plots/phsp/fullcl_vs_2dx3d/phsp_fullcl_vs_2dx3d.pdf}
\caption{Comparison between harmonic and hybrid harmonic-Fourier approaches for the case of $\GCph\times\GCsp$.}
\label{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

%

% WLxGCsp
%-----------------------------------------%
\subsection{\large{Combining weak lensing and spectroscopic clustering}}
\label{sec:ch4_results_wlxsp}
In this section we report the results from the combination of $\WL$ and $\GCsp$. The Fisher matrix in the harmonic approach is $[\WL+\GCsp+\xc{\WL}{\GCsp}]$, while in the hybrid one it is $[\WL+\xc{\WL}{\GCsp}] + [\GCsp(P_k)]$. we quantify the impact on parameter constraints of the $\WL$-$\GCsp$ cross-covariance and the $\xc{\GCph}{\GCsp}$ cross-correlation using percentage differences. we take as reference values for the percentages the constraints coming from the Fisher matrix corresponding to independent combination of $\WL$ and $\GCsp$, that is $[\WL]+[\GCsp]$ in the harmonic approach and $[\WL]+[\GCsp(P_k)]$ in the hybrid one. For brevity, the results of this combination are reported in the optimistic scenario only.

% TABLE FoM WLxGCsp
%-----------------------------------------%
\begin{table*}[t]
\centering
\begin{resultstable}{CL*{3}{C}}
\multicolumn{5}{c}{$\WL\times\GCsp$ FoM results} \\
\midrule
\GCsp \, \text{bins} & \text{Fisher matrix} & \FoM & \Delta \FoM & \Delta \FoM (\%)\\
\midrule
\multirow{3}{*}{4} 
& [\WL] + [\GCsp(P_k)]                 & 158.13 & \text{--} & \text{--} \\
& [\WL+\xc{\WL}{\GCsp}] + [\GCsp(P_k)] & 182.74 & \text{--} & \text{--} \\
& [\WL] + [\GCsp]                      & 74.72  & \text{--} & \text{--} \\
& [\WL+\GCsp]                          & 74.37  & -0.35 & \negative{-0.47\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}]          & 103.56 & +28.83 & \positive{+38.59\%}\\
\midrule
\multirow{3}{*}{12} 
& [\WL] + [\GCsp] & 92.90 & \text{--} & \text{--}\\
& [\WL+\GCsp] & 92.77 & -0.13 & \negative{-0.14\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 131.38 & +38.47 & \positive{+41.41\%}\\
\midrule
\multirow{3}{*}{24} 
& [\WL] + [\GCsp] & 111.41 & \text{--}& \text{--}\\
& [\WL+\GCsp] & 111.42 & +0.01 & \positive{+0.0021\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 155.18 & +43.76 & \positive{+39.28\%}\\
\midrule
\multirow{3}{*}{40} 
& [\WL] + [\GCsp] & 141.12 & \text{--} & \text{--}\\
& [\WL+\GCsp] & 141.17 & +0.06 & \positive{+0.042\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 188.45 & +47.34 & \positive{+33.55\%}\\
\end{resultstable}
\caption{Table reporting the $\FoM$ for $\WL$, $\GCsp$ and their cross-correlation
The $\Delta\FoM$ column contains the variation of the figure of merit with respect to the independent sum $[\WL] + [\GCsp]$ for the given number of bins. The $\Delta\FoM (\%)$ column is calculated by taking $\Delta\FoM$ as a percentage of the FoM of $[\WL] + [\GCsp]$.}
\label{tab:ch4_results_wlsp_fom}
\end{table*}
%-----------------------------------------%

% PERC.DIFF ERRORS PLOT WLxGCsp: FULL CL
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.90\textwidth]{Figures/optimistic/perc_diff_errors/WLGCsp_cov_and_xc_impact.pdf}
\caption{Impact, on $\onesigma$ parameter errors and $\FoM$, of cross-covariance and cross-correlation in the harmonic approach for the combination of $\WL$ and $\GCsp$. The left panel shows the impact of the cross-covariance, quantified with the percentage differences between $[\WL+\GCsp]$ and $[\WL] + [\GCsp]$. In the right panel the impact of the cross-correlation is reported, quantified by percentage differences of $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ with respect to $[\WL]+[\GCsp]$. Note that the percentages on the left panel have been multiplied by $10$ in order to make them visible with the same vertical scale of the right panel.}
\label{fig:ch4_wlsp_fullcl_percdiff_plot}
\end{figure*}
%-----------------------------------------%

\subsubsection{Impact of the $\bWL$-$\bGCsp$ cross-covariance on parameter constraints}
In \tabref{tab:ch4_results_wlsp_fom} are reported the FoM values resulting from the combinations of $\WL$ and $\GCsp$. In this case the cross-covariance is even more negligible than in the $\GCph$-$\GCsp$ case, always impacting by less than $0.5\%$ on the figure of merit. This effect gets smaller as the number of bins increases, starting from $-0.47\%$ with $4$ spectroscopic bins up to $+0.042\%$ with $40$ spectroscopic bins respectively. This last is unexpectedly positive, but the variation is so small that can be considered as a numerical fluctuation around zero.

The same conclusion can be drawn by looking at the effect of the covariance on the marginalised $\onesigma$ uncertainties on the cosmological parameters, shown in the left panel of \figref{fig:ch4_wlsp_fullcl_percdiff_plot}. The marginalised uncertainties affected the most by the cross-covariance are the ones on $h$ and $\Omb$, with variations of $0.7\%$ and $0.3\%$ respectively. The variations on all the other parameters are always well below $0.2\%$, and in all cases the absolute value of these variations decreases as the number of $\GCsp$ bins increases, confirming the same trend observed for the FoM.

The conclusion here is that, when combining $\WL$ and $\GCsp$ in the harmonic domain, their cross-covariance can be safely neglected. A similar result for another experiment other than \Euclid has been obtained in~\cite{Heymans2020}. Here the authors performed a joint data analysis combining weak lensing measurements from the Kilo-Degree Survey (KiDS-1000) and spectroscopic clustering from the Baryon Acoustic Oscillations Survey (BOSS) and 2-degree Field Lensing Survey (2dFLenS). The $\WL$ was treated using the harmonic power spectrum as observable, as it has been done in this work. Moreover, the cross-covariance matrix was computed in the harmonic domain, considering only the correlation between $\WL$ and the transverse component of $\GCsp$. The authors estimated the covariance matrix for the data through an analysis of over $\num{20 000}$ fast full-sky mock galaxy catalogues, finding that the off-diagonal (cross-covariance) terms were negligible with respect to the diagonal (auto-covariance) ones.

% WLxGCsp: hybrid XC impact
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\textwidth]{Figures/optimistic/perc_diff_errors/wlsp_hybrid_xc_impact.pdf}
\caption{Impact, on FoM and marginalised $\onesigma$ errors, of the $\xc{\WL}{\GCsp}$ in the hybrid approach, for the optimistic scenario. Note that in the hybrid approach only $4$ tomographic bins were used to compute the $\xc{\WL}{\GCsp}$ angular power spectra, for consistency with the Fourier power spectrum analysis.}
\label{fig:ch4_wlsp_hybrid_xc_impact}
\end{figure*}
%-----------------------------------------%

\subsubsection{Impact of the $\bxc{\bWL}{\bGCsp}$ signal on parameter constraints}
\paragraph{Harmonic approach}
When combining $\WL$ and $\GCsp$ only, the $\xc{\WL}{\GCsp}$ has a quite significant impact on the results of the harmonic approach, as \tabref{tab:ch4_results_wlsp_fom} shows. The percentage gain on the figure of merit is always larger than $+30\%$, and slightly depends on the number of spectroscopic bins used. This can be explained by observing that $\WL$ weight functions have a broad support, which becomes larger as the tomographic index increases, as \figref{fig:ch4_weight_functions_plot} shows. This suggests that increasing the radial resolution may not help in improving the constraints coming from the $\xc{\WL}{\GCsp}$. It is also worth noting that the FoM percentage gain does not strictly increase with the number of spectroscopic bins. In particular it is $+38\%$ at 4 bins and $+33\%$ with $40$ bins, with a maximum of about $+41\%$ at $12$ bins.
This not intuitive behaviour is due to the normalisation of the FoM percentage difference, which is the FoM of the $[\WL] + [\GCsp]$ Fisher matrix. This quantity depends on the number of spectroscopic bins, and it increases slightly faster than the variation induced by the cross-correlation in the FoM of the $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ Fisher matrix. This can be seen from \tabref{tab:ch4_results_wlsp_fom}: the difference $\Delta\FoM$ between the FoMs of the $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ and $[\WL] + [\GCsp]$ Fisher matrices grows slower with the number of bins than the FoM of $[\WL] + [\GCsp]$ alone.

The marginalised $\onesigma$ uncertainties decrease when the $\xc{\WL}{\GCsp}$ cross-correlation signal is included, especially the ones on $\wz, \wa, \sige$ and $\Omm$, as it can be seen from \figref{fig:ch4_wlsp_fullcl_percdiff_plot}. For these parameters the improvement is always larger than $12\%$ with $4$ $\GCsp$ bins, and it is about $20\%$ at most when $40$ bins are used. The gain on the $\Omb$ uncertainty is more modest, being comprised between $5\%$ and $10\%$. The uncertainties on the reduced Hubble constant $h$ and the scalar spectral index $\ns$ gain always less than $5\%$.

The improvement on the marginalised uncertainties $\xc{\WL}{\GCsp}$ cross-correlation seems to decrease when increasing the number of spectroscopic bins, as it happens for the FoM. Again, the reason of this behaviour is that the performances of the Fisher matrix taken as reference -- that is $[\WL] + [\GCsp]$ -- improve faster than the relative contribution of the cross-correlation. This is true for all parameters except for $h$, which is the parameter affected the least.

\paragraph{Hybrid approach}
The impact on the constraints of the $\xc{\WL}{\GCsp}$ cross-correlation in the hybrid approach is less significant than in the harmonic one, as shown in \figref{fig:ch4_wlsp_hybrid_xc_impact}.
The FoM of the $[\WL+\xc{\WL}{\GCsp}] + [\GCsp(P_k)]$ Fisher matrix is $183$, which is $\sim 15\%$ higher than the one of the independent combination $[\WL] + [\GCsp(P_k)]$, which is $158$. The improvements on the marginalised uncertainties are all comprised between $5\%$ and $7\%$, and there are no significant differences between the various parameters. The uncertainty on $\Omm$ is the most affected, gaining about $8\%$, while the least affected is the uncertainty on $\ns$, which is slightly lower than $5\%$.

% WLxGCsp, hybrid vs harmonic
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\textwidth]{Figures/optimistic/perc_diff_errors/wlsp_hybrid_vs_harmonic.pdf}
\caption{Percentage difference between FoM and marginalised $\onesigma$ errors of the hybrid and harmonic approaches, for the combination of $\WL$ and $\GCsp$ in the baseline optimistic scenario. The percentage differences are normalised to the results of the harmonic approach.}
\label{fig:ch4_wlsp_hybrid_vs_harmonic}
\end{figure*}
%-----------------------------------------%

% FoM Gain PLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/fom_gain/wlsp_fom_gain.pdf}
\caption{Percentage gain on the FoM relative to weak lensing clustering alone ($[\WL]$). In the left panel the computation has been done using the standard $\GCsp$ shot noise \eqref{eq:ch4_gc_shot_noise}, while in the right panel the reduced version \eqref{eq:ch4_reduced_gcsp_noise} has been used.}
\label{fig:ch4_wlsp_fom_gain}
\end{figure*}
%-----------------------------------------%


% XC(WL,GCph) vs XC(WL,GCsp) comparison plot
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=0.85\textwidth]{Figures/optimistic/xcwlph_vs_xcwlsp.pdf}
\caption{Impact, on FoM and marginalised $\onesigma$ uncertainties, of the $\xc{\WL}{\GCph}$ and $\xc{\WL}{\GCsp}$ cross-correlations in different configurations. The vertical bars represent the percentage differences on the uncertainties normalised to the independent sum of the two probes. For $\xc{\WL}{\GCph}$ the reference is $[\WL] + [\GCph]$, while for $\xc{\WL}{\GCsp}$ is $[\WL] + [\GCsp]$. Note that for the uncertainties the percentage variation is \emph{negative}, meaning that the contribution of the cross-correlations \emph{reduces} the errors.}
\label{fig:ch4_xcwlph_vs_xcwlsp}
\end{figure*}
%-----------------------------------------%

\subsubsection{Hybrid approach vs harmonic approach}
In contrast to what happens in the case of $\GCph$ and $\GCsp$, when combining $\WL$ and $\GCsp$ the harmonic approach can reach the FoM of the hybrid one. However, this only happens when $40$ $\GCsp$ bins are used to compute the harmonic Fisher matrix $[\WL+\GCsp+\xc{\WL}{\GCsp}]$. The value reached by the FoM is $188$, which is only $3\%$ higher than the on given by the hybrid approach. Moreover, \figref{fig:ch4_wlsp_hybrid_vs_harmonic} shows that the marginalised uncertainties in $\wz, \wa$ of the hybrid approach are smaller than their harmonic counterparts. Nonetheless, as said above, the FoM of the harmonic approach is slightly higher than the one of the hybrid approach. This is due to the correlation $\mathcal{C}_{\wz\wa}$ between the parameters, which enters the definition \eqref{eq:ch4_fom_def} of the FoM. This correlation is higher for the harmonic approach, and this compensates for the larger uncertainties, with a net result of slightly higher FoM. This effect can also be seen by zooming on the bottom panel of \figref{fig:ch4_contour_w0wa_wlsp_fullcl_vs_2dx3d}. The contour of the harmonic approach (cyan) in the $\wz$-$\wa$ plane is slightly narrower than the contour of the hybrid one (red), even if being more elongated, and this results in a smaller area of the contour ellipse -- which means an higher FoM -- of the former with respect to the latter.

Regarding the marginalised uncertainties, \figref{fig:ch4_wlsp_hybrid_vs_harmonic} shows that the hybrid approach always performs better than the harmonic one. The reduced Hubble constant $h$ is the parameter for which the difference is highest. In particular, the hybrid approach produces an uncertainty on $h$ which is $\sim 90\%$ ($75\%$) smaller than the one given by the harmonic approach with $4$ ($40$) spectroscopic bins. For the uncertainties on the other parameters the gap is smaller, and it reduces significantly as the number of spectroscopic bins increases. The most sensitive uncertainty is the one on $\Omb$, for which the gap between the two approaches decreases from more than $50\%$ to less than $10\%$ when $4$ and $40$ bins are used for the harmonic approach respectively. The uncertainty on $\ns$ is quite sensitive to the number of bins too, and the difference between the two approaches ranges from $40\%$ to $10\%$ when the number bins of the harmonic approach increases from $4$ to $40$. Finally, the differences on the marginalised uncertainties on $\Omm$ and $\sige$ are smaller, ranging from $20\%$ to less than $5\%$.

\subsubsection{Comparing $\bxc{\bWL}{\bGCsp}$ with $\bxc{\bWL}{\bGCph}$}
In~\citetalias{Blanchard:2019oqi} it has been shown that the $\xc{\WL}{\GCph}$ cross-correlation considerably improves the constraints on the cosmological parameters. In this work the same result is found: in the optimistic scenario the Fisher matrix $[\WL+\GCph+\xc{\WL}{\GCph}]$ yields a FoM which is a factor of $\sim 5$ higher than the one given by the $[\WL] + [\GCph]$ Fisher matrix. This means that the percentage gain induced by the cross-correlation signal is about $400\%$. The $\xc{\WL}{\GCsp}$ cross-correlation has a smaller impact on the constraints, as the $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ Fisher matrix produces a FoM at most $\sim 40\%$ higher than the one of the $[\WL] + [\GCsp]$ combination. This is what happens when both $\GCph$ and $\GCsp$ are treated in the baseline settings, i.e. when the standard shot noise \eqref{eq:ch4_gc_shot_noise} is used for $\GCsp$ and $10$ tomographic bins are used for $\GCph$. The effect of the shot noise on $\GCsp$ can be seen from \figref{fig:ch4_wlsp_fom_gain}, where it is reported the percentage gain on the FoM of various combinations with respect to $\WL$ alone. Left panel refers to the standard $\GCsp$ shot noise computed with the second equation of \eqref{eq:ch4_gc_shot_noise}, right panel refers to the alternative reduced noise of \eqref{eq:ch4_reduced_gcsp_noise}. When the noise is reduced the Fisher matrix of the harmonic approach with $4$ bins is already competitive with the one of the hybrid approach, yielding a gain of $\sim 300\%$ relative to $\WL$ alone. The observable gaining the most from the noise reduction is the $\GCsp$ auto-correlation, as the two curves of $[\WL+\GCsp]$ and $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ converges towards each other as the number of bins increases. 

A direct comparison between the gain coming from $\xc{\WL}{\GCph}$ and $\xc{\WL}{\GCsp}$ cross-correlations is shown in \figref{fig:ch4_xcwlph_vs_xcwlsp}, where the percentage variations on parameter constraints are represented with vertical bars. When $\GCsp$ and $\GCph$ have the same shot noise level and the same redshift range, the effect of the $\xc{\WL}{\GCsp}$ on the constraints becomes comparable with the one of $\xc{\WL}{\GCph}$.

Therefore, the conclusion is the same drawn for the direct comparison between the $\GCph$ and $\GCsp$ auto-correlations. The shot noise and the redshift range of the galaxy catalogue are what makes the differences between $\xc{\WL}{\GCph}$ and $\xc{\WL}{\GCsp}$ in terms of constraining power.

% CONTOUR PLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}[h!]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.75\textwidth]{Figures/optimistic/contours/wlsp/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf} \\
\includegraphics[width=0.75\textwidth]{Figures/optimistic/contours/wlsp/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the combination of $\WL$ and $\GCsp$.}
\label{fig:ch4_contour_w0wa_wlsp_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%

% ERROR BARPLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}[h!]
\centering
\includegraphics[width=0.80\textwidth]{Figures/optimistic/error_plots/wlsp/fullcl_vs_2dx3d/wlsp_fullcl_vs_2dx3d.pdf}
\caption{Comparison between harmonic and hybrid harmonic-Fourier approaches for the case of $\WL\times\GCsp$.}
\label{fig:ch4_wlsp_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

% 6x2pt
%-----------------------------------------%
\subsection{\large{Exploiting the \Euclid $\bsixtwoptShort$ statistics}}
\label{sec:ch4_results_6x2pt}
In this section we present the results of the combination of all the \Euclid main probes: $\WL, \GCph$, and $\GCsp$. The starting point is the (photometric) $\threetwoptShort$ statistics, defined as
%
\begin{equation}\label{eq:ch4_3x2pt_def}
\threetwoptShort \equiv [\threetwoptLong]\, .
\end{equation}
%
This combination has already been studied in~\citetalias{Blanchard:2019oqi}, finding that the $\xc{\WL}{\GCph}$ cross-correlation has a large impact on the constraints. The same result is found in this work too, as it has been already pointed out in \secref{sec:ch4_results_wlxsp} -- see the red bars of \figref{fig:ch4_xcwlph_vs_xcwlsp}. In terms of this combination, the $\sixtwoptShort$ statistics, defined in \eqref{eq:ch4_6x2pt_harmonic_def} and \eqref{eq:ch4_6x2pt_hybrid_def}, can be expressed as
%
\begin{comment}
\begin{equation}\label{eq:ch4_6x2pt_defs_from_3x2pt}
\begin{split}
[(\text{harmonic})\, \sixtwoptShort] &= [\threetwoptShort + \GCsp + \xc{\WL}{\GCsp} + \xc{\GCph}{\GCsp}]\\
[(\text{hybrid})\, \sixtwoptShort] &= [\threetwoptShort + \xc{\WL}{\GCsp} + \xc{\GCph}{\GCsp}] + [\GCsp(P_k)]
\end{split}
\end{equation}
\end{comment}

\begin{align*}
[(\text{harmonic})\, \sixtwoptShort] =&\; [\threetwoptShort + \GCsp + \xc{\WL}{\GCsp} + \\ 
&\;\xc{\GCph}{\GCsp}]
\end{align*}
\begin{align}\label{eq:ch4_6x2pt_defs_from_3x2pt}
[(\text{hybrid})\, \sixtwoptShort] =&\; [\threetwoptShort + \xc{\WL}{\GCsp} +\\\nonumber 
&\;\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]
\end{align}
%
In this section we report the \Euclid performance when $\GCsp$ and its cross-correlations with $\WL$, and $\GCph$ are combined with the $\threetwoptShort$ statistics. The discussion will be focused on two main points: 
\begin{itemize}
\item the importance of the cross-covariance between $\GCsp$ and the $\threetwoptShort$ statistics;
\item the contribution to the constraints of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations.
\end{itemize}
The cross-covariance between $\GCsp$ and $\threetwoptShort$ statistics is studied only in the harmonic approach, since in the hybrid approach it is neglected by definition. The effect of the cross-correlations is assessed for both the harmonic and the hybrid approaches, and in both the pessimistic and optimistic scenarios defined in \tabref{sec:ch4_results_settings}.

% Cov with GCsp impact 
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/cov_impact_6x2pt.pdf}
\caption{Impact, on FoM and marginalised 1-$\sigma$ uncertainties, of cross covariances between $\GCsp$ and $\threetwoptShort\, ([\WL+\GCph+\xc{\WL}{\GCph}])$, quantified with percentage differences on the constraints, in the optimistic (left) and pessimistic (right) scenarios. The reference for the percentage are the constraints of $[\threetwoptShort] + [\GCsp]$, where $\GCsp$ is considered as \emph{independent} from the rest.}
\label{fig:ch4_3x2pt_sp_cov_impact}
\end{figure*}
%-----------------------------------------%

\subsubsection{Impact of the $\bGCsp$ cross-covariances on parameter constraints}
The impact on the constraints of the cross-covariance between $\GCsp$ and $\threetwoptShort$ is shown in the two panels of \figref{fig:ch4_3x2pt_sp_cov_impact}, the left one representing the optimistic scenario and the right the pessimistic one. The plot compares the constraints from the $[\threetwoptShort+\GCsp]$ and $[\threetwoptShort]+[\GCsp]$ combinations: in the former the $\GCsp$-$\threetwoptShort$ cross-covariance is taken into account, while it is not in the latter. It can be seen that the impact of the cross-covariance is almost the same in the two scenarios and decreases as the number of $\GCsp$ bins increases, confirming the same trend observed in the two pairwise combinations $\GCph$-$\GCsp$ and $\WL$-$\GCsp$. The percentage variations on the constraints are always below $10\%$ ($5\%$) with $4$ ($40$) spectroscopic bins. It is also evident that the covariance almost always worsens the constraints, reducing the FoM and increasing the marginalised $\onesigma$ uncertainties with respect to considering $\GCsp$ and $\threetwoptShort$ as independent. The parameters whose uncertainties are affected the most by the $\GCsp$-$\threetwoptShort$ cross-covariance are $\Omb$ and $h$, with variations of $\sim 8\%$ with $4$ bins. When $40$ bins are used for $\GCsp$ the variation reduces to $\sim 2\%$ for both parameters.

On of the most evident differences between the optimistic and the pessimistic scenario is the impact on the FoM, which is slightly higher in the pessimistic than in the optimistic setting. However the percentage difference is always below $5\%$, the worst case being the pessimistic scenario with $4$ bins, where it is $\sim 4\%$. The percentage variation on the $\Omm$ uncertainty is at the sub-percent level in the optimistic scenario, while it is about at the percent level in the pessimistic scenario. The uncertainty on $\sige$ is always smaller than $1\%$ in the optimistic scenario, while it ranges from $4\%$ to $1\%$ in the pessimistic scenario.

% 6x2pt harmonic: XCs impact, ref. [3x2pt+GCsp] 
% (COVARIANT)
%-----------------------------------------%
% Versione nuova (plot singolo 2x3)
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/6x2pt_harmonic_xcs_impact_ref_[3x2pt+GCsp].pdf}
\caption{Impact of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations on FoM and marginalised $\onesigma$ uncertainties, with respect to the constraints given by the $[\threetwoptShort+\GCsp]$ Fisher matrix, in which the cross-covariance between $\threetwoptShort$ statistics and $\GCsp$ is taken into account. The top panels refer to the optimistic scenario, while the bottom panels refer to the pessimistic one. Note that the percentage differences related to $\xc{\WL}{\GCsp}$ have been multiplied by $100$ to make them visible when using a single scale on the $y$ axis.}
\label{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov}
\end{figure*}

\subsubsection{Impact of the $\rm \mathbf{XC}$ signals on parameter constraints}
Here we discuss the impact on the constraints of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations. The impact of the cross-correlations is quantified as percentage differences on the constraints with respect to the given reference, represented with vertical bars. \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_nocov} and \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov} show the results in the harmonic approach, and  \figref{fig:ch4_6x2pt_hybrid_xcs_impact} in the hybrid one. Each of these plots contains three columns. The left column reports the effect of the inclusion of the $\xc{\WL}{\GCsp}$ cross-correlation, the middle column reports the impact of the $\xc{\GCph}{\GCsp}$ cross-correlation, and the right column reports the impact of both.

\paragraph{Harmonic approach}
For the harmonic approach, two Fisher matrices have been used as reference for the percentage differences: $[\threetwoptShort] + [\GCsp]$, where the $\threetwoptShort$ statistics and $\GCsp$ are combined as independent, and $[\threetwoptShort+\GCsp]$, where the cross-covariance between the two is taken into account (see \secref{sec:ch4_fisher_fullcl}). As explained in the previous section, these two combinations do not produce the same constraints (see \figref{fig:ch4_3x2pt_sp_cov_impact}), as the independent combination yields slightly better constraints.

I consider the two different references above since, when the cross-correlations are added in the harmonic approach, the cross-covariance between $\GCsp$ and the $\threetwoptShort$ statistics is always accounted for. Thus, on the one hand, we focus on the improvement due to the inclusion of the $\rm XC$ signals alone, and this is done when the Fisher matrix $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ is compared to the reference $[\threetwoptShort+\GCsp]$, and the same for $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ and $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}]$ (see \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov}). In this case, the percentage differences are representative of the \emph{net effect} of the cross-correlation signals on the constraints, which is expected to be always positive.

On the other hand, when the Fisher matrices comprising the $\rm XC$'s information are compared to the independent combination $[\threetwoptShort] + [\GCsp]$, we focus on the \emph{total effect}, which not only contains the gain from the inclusion of the $\rm XC$ signals, but also the penalty from the cross-covariance between $\GCsp$ and the $\threetwoptShort$ statistics (see \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_nocov}). This comparison is useful in order to evaluate the overall impact of the cross angular power spectra.

\paragraph{Harmonic approach: adding $\bxc{\bWL}{\bGCsp}$}
The net effect of the $\xc{\WL}{\GCsp}$ inclusion is shown in the left panels of \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov}, where the Fisher matrix $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ is compared to the reference $[\threetwoptShort+\GCsp]$. The differences in this case have been amplified by a factor of $100$ to make them visible on the same vertical scale of the other plots. The variation on the constraints due to the addition of $\xc{\WL}{\GCsp}$ to $[\threetwoptShort+\GCsp]$ is always about $0.01\%$-$0.05\%$, with no significant differences between the optimistic and pessimistic scenarios. Therefore, it seems that this cross-correlation does not give any contribution to the constraints, i.e. it looks like the computation of the total $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ Fisher matrix is not useful to improve the \Euclid performance.
This might seem in contrast to what happens in the pairwise combination of $\WL$ and $\GCsp$, where the $\xc{\WL}{\GCsp}$ cross-correlation signal has a significant impact on the constraints. However, the latter case does not include by definition the $\xc{\WL}{\GCph}$ signal, since it refers only to $\WL$ combined with $\GCsp$. Instead, in the case now under discussion of $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$, the reference for the net effect here considered is $[\threetwoptShort+\GCsp]$, which contains the contribution of the $\xc{\WL}{\GCph}$ cross-correlation, proven to be dominant.

From the above reasoning, it is also possible to infer the reason why the constraints from the $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ Fisher matrix are worse by $6\%$ at most (see \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_nocov}) than the ones from the independent combination $[\threetwoptShort]+[\GCsp]$ taken now as reference: the impact of the cross-correlation signal is so small that its possible improvements are completely dominated by the cross-covariance between $\GCsp$ and the $\threetwoptShort$ statistics (see \figref{fig:ch4_3x2pt_sp_cov_impact}), which is present when adding the cross signal, but not kept into account in the reference. Therefore, the total effect of the inclusion of $\xc{\WL}{\GCsp}$ in the combination of $\GCsp$ with the $\threetwoptShort$ statistic is to worsen the parameter constraints. However, while it has been just shown that the $\xc{\WL}{\GCsp}$ signal can be safely neglected, the cross-covariance between $\GCsp$ and the $\threetwoptShort$ statistic needs to be taken with caution.  

\paragraph{Harmonic approach: adding $\bxc{\bGCph}{\bGCsp}$}
The middle panel of \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov} shows the \emph{positive} net effect of the $\xc{\GCph}{\GCsp}$ inclusion, which increases with the number of spectroscopic bins. This confirms the same behaviour observed in the pairwise combination of $\GCph$ and $\GCsp$. The gain on the FoM relative to the Fisher matrix $[\threetwoptShort+\GCsp]$ is about $1\%$ for $4$ bins, and increases up to $8$-$10\%$ for $40$ bins, with practically no differences between the optimistic and the pessimistic scenario. \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_nocov} shows that when the independent combination $[\threetwoptShort]+[\GCsp]$ is used as reference instead, the FoM variation due to the $\xc{\GCph}{\GCsp}$ inclusion is $-2\%$ ($+7\%$) for $4$ ($40$) $\GCsp$ bins. The small worsening at $4$ bins is due to the fact that the positive contribution of the cross-correlation is cancelled by the negative contribution of the $\GCsp$-$\threetwoptShort$ cross-covariance (see \figref{fig:ch4_3x2pt_sp_cov_impact}). In fact, this cross-covariance is taken into account in the Fisher matrix $[\threetwoptShort+\GCsp+\xc{\GCph}{\GCsp}]$, while it is not in the $[\threetwoptShort]+[\GCsp]$, which is used as the reference in this last case.

Analogously, the marginalised $\onesigma$ uncertainties on the cosmological parameters exhibit a similar behaviour, with no significant differences between the optimistic and the pessimistic scenarios. When using $4$ spectroscopic bins the inclusion of the $\xc{\GCph}{\GCsp}$ cross-correlation produces a small improvement when the Fisher matrix $[\threetwoptShort+\GCsp]$ is used as reference. For a small number of bins, this positive contribution is in general compensated by cross-covariance effects when the percentage differences are referred to the $[\threetwoptShort]+[\GCsp]$ Fisher matrix. When using $40$ spectroscopic bins the cross-correlation dominates and the cross-covariance effects become negligible, and the percentage differences become always positive, independently of the reference that is used. The parameters whose uncertainties decrease the most are $\Omb$ and $h$, gaining $15\%$ and $10\%$ respectively in the optimistic scenario, $10\%$ and $5\%$ in the pessimistic.

Therefore, the total effect of the inclusion of $\xc{\GCph}{\GCsp}$ in the combination of $\GCsp$ with the $\threetwoptShort$ statistic depends on the chosen binning set, and may be dominant with respect to $\GCsp$-$\threetwoptShort$ cross-covariance effects for a large number of bins.


% 6x2pt harmonic: XCs impact, ref. [3x2pt] + [GCsp]
% (NO CROSS-COVARIANCE)
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/6x2pt_harmonic_xcs_impact_ref_[3x2pt]_+_[GCsp].pdf}
\caption{Impact of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations on FoM and marginalised $\onesigma$ uncertainties, with respect to the constraints given by $[\threetwoptShort]+[\GCsp]$, $\threetwoptShort$ and $\GCsp$ are combined as independent. The top panels refer to the optimistic scenario, while the bottom panels refer to the pessimistic one.}
\label{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_nocov}
\end{figure*}
%-----------------------------------------%

\paragraph{Harmonic approach: the $\bsixtwoptShort$ statistics}
The harmonic $\sixtwoptShort$ statistics in \eqref{eq:ch4_6x2pt_harmonic_def} consists of the inclusion of the $\xc{\WL}{\GCsp}$ and $\xc{\GCph}{\GCsp}$ cross-correlations in the $[\threetwoptShort+\GCsp]$ data-vector. In the harmonic approach, the constraints produced by the $\sixtwoptShort$ analysis are equivalent to the ones given by including the $\xc{\GCph}{\GCsp}$ alone. The percentage differences between the constraints from the $\sixtwoptShort$ Fisher matrix and the $[\threetwoptShort+\GCsp]$ Fisher matrix are reported in the rightmost panels of \figref{fig:ch4_6x2pt_harmonic_xcs_impact_ref_3x2pt_gcsp_cov}. These are indistinguishable from the ones reported in the middle panels, which refer to the impact of the $\xc{\GCph}{\GCsp}$ cross-correlation only with respect to $[\threetwoptShort+\GCsp]$. This is expected, since in the above paragraphs it has been shown that $\xc{\WL}{\GCsp}$ provides a negligible contribution with respect to $\xc{\GCph}{\GCsp}$.

% 6x2pt hybrid: XCs impact, ref. [3x2pt] + [GCsp(Pk)]
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/6x2pt_hybrid_allxcs_impact.pdf}
\caption{Impact, on FoM and marginalised $\onesigma$ errors, of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations in the hybrid approach. The reference for the percentage differences is $[\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp(P_k)]$. In any case the cross-correlations are always considered to be \emph{covariant} with the $\threetwoptShort$ statistics observables. Note that the percentage differences in left panel have been multiplied by $10$, to make them visible to the naked eye.}
\label{fig:ch4_6x2pt_hybrid_xcs_impact}
\end{figure*}
%-----------------------------------------%

\paragraph{Hybrid approach}
The contribution of the $\xc{\WL}{\GCsp}$ and $\xc{\GCph}{\GCsp}$ signals in the hybrid approach is reported in \figref{fig:ch4_6x2pt_hybrid_xcs_impact}, quantified with percentage differences of the constraints plotted as vertical bars. In this case the reference used is always the independent combination $[\threetwoptShort]+[\GCsp(P_k)]$, since in the hybrid approach the cross-covariance between $\GCsp(P_k)$ and the $\threetwoptShort$ is neglected by definition. 
Only the $4$ bins case is presented for consistency with the power spectrum analysis done in \citetalias{Blanchard:2019oqi}, for which the authors employ the $4$ standard spectroscopic bins listed in \tabref{tab:ch4_spectro_tomo_bins}. Again, \figref{fig:ch4_6x2pt_hybrid_xcs_impact} is subdivided in three columns. The first column reports the impact of $\xc{\WL}{\GCsp}$, the middle column reports the impact of $\xc{\GCph}{\GCsp}$, and finally in the last column reports the impact of both.

\paragraph{Hybrid approach: adding $\bxc{\bWL}{\bGCsp}$}
In the hybrid approach the impact of the $\xc{\WL}{\GCsp}$ cross-correlation on the constraints from $[\threetwoptShort+\xc{\WL}{\GCsp}]+[\GCsp(P_k)]$, relative to $[\threetwoptShort]+[\GCsp(P_k)]$, is negligible, being always less than $0.05\%$, both in the optimistic and in the pessimistic scenarios. The contribution is so small that it has been amplified by a factor of $10$, in order to make it visible when using a single scale on the vertical axis. This result is analogous to what has been found with the harmonic approach, when we consider the comparison of $[\threetwoptShort+\GCsp+\xc{\WL}{\GCsp}]$ with respect to $[\threetwoptShort+\GCsp]$, to isolate the impact of $\xc{\WL}{\GCsp}$. This is expected, since there are no differences in the $\threetwoptShort$ between the two approaches, and, in particular, the $\xc{\WL}{\GCph}$ cross-correlation is computed in the same way in the two cases.

\paragraph{Hybrid approach: adding $\bxc{\bGCph}{\bGCsp}$}
In the hybrid approach the impact of the $\xc{\GCph}{\GCsp}$ cross-correlation on the constraints from $[\threetwoptShort+\xc{\GCph}{\GCsp}]+[\GCsp(P_k)]$, relative to $[\threetwoptShort]+[\GCsp(P_k)]$, is slightly smaller than in the harmonic one with $4$ spectroscopic bins. The middle panel of \figref{fig:ch4_6x2pt_hybrid_xcs_impact} shows that the absolute percentage differences on all constraints is always below $2\%$. The gain on the FoM is $\sim 1\%$ both in the optimistic and the pessimistic scenario. The parameters whose uncertainties are affected the most are $\Omb$ and $h$, with a gain of $1.5\%$ at most in the pessimistic scenario, and less than $0.5\%$ in the optimistic scenario.

\paragraph{Hybrid approach: the $\bsixtwoptShort$ statistics}
As it happens for the harmonic approach, the constraints given by the hybrid $\sixtwoptShort$ statistics are similar to the ones given by the inclusion of the $\xc{\GCph}{\GCsp}$ cross-correlation only. This is manifest in the right panel of \figref{fig:ch4_6x2pt_hybrid_xcs_impact}: the vertical bars representing the differences are indistinguishable from the ones in the middle panel. Nonetheless, in the hybrid approach the inclusion of the $\xc{\GCph}{\GCsp}$ cross-correlation has a negligible impact on the constraints, as discussed in the above paragraph. Therefore, the Fisher matrix of the hybrid $\sixtwoptShort$ statistics produces constraints that are almost equivalent to the $[\threetwoptShort]+[\GCsp(P_k)]$ Fisher matrix.

% Hybrid vs Harmonic 6x2pt
%-----------------------------------------%
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/hybrid_vs_harmonic.pdf}
\caption{Comparison between FoM and marginalised $\onesigma$ uncertainties of the hybrid $\sixtwoptShort$ and the harmonic $\sixtwoptShort$ statistics, quantified using percentage differences taking the latter as reference.}
\label{fig:ch4_6x2pt_hybrid_vs_harmonic}
\end{figure*}
%-----------------------------------------%

\subsubsection{The $\bsixtwoptShort$ statistics: hybrid approach vs harmonic approach}
For the $\sixtwoptShort$ statistics the hybrid approach performs better than the harmonic one, especially when a small number of spectroscopic bins is used for the latter. The comparison of the two approaches is reported in \figref{fig:ch4_6x2pt_hybrid_vs_harmonic}, where the percentage differences between their constraints are plotted as vertical bars. In this case, the reference adopted is the Fisher matrix of the harmonic approach, \eqref{eq:ch4_6x2pt_harmonic_def}. The hybrid approach produces a FoM which is $20\%$ ($40\%$) larger than the harmonic one in the optimistic (pessimistic) scenario, when $4$ spectroscopic bins are used for the latter. When using $40$ bins, the harmonic approach performs instead slightly better ($\sim 6\%$) than the hybrid one in the optimistic scenario, while it is equivalent to it in the pessimistic scenario. 

Regarding the marginalised $\onesigma$ uncertainties on the dark energy parameters, $\wz, \wa$, the hybrid approach always provides better constraints than the harmonic one, regardless the number of spectroscopic bins used for the latter. However, the harmonic approach with $40$ bins produces a slightly higher FoM than the hybrid one in the optimistic scenario.

%This is possible because the FoM is not only affected by the uncertainties on $\wz$ and $\wa$, but also by their covariance $\mathcal{C}_{\wz\wa}$ -- see \eqref{eq:ch4_fom_def}. The Fisher matrix of the harmonic approach with $40$ spectroscopic bins produces an higher covariance $\mathcal{C}_{\wz\wa}$, which compensates for the larger uncertainties and providing in the end a slightly higher FoM.

% 6x2pt FoM TABLE
%-----------------------------------------%
\begin{table*}[t]
\centering
\begin{resultstable}{*{1}{L}*{4}{C}}
\multicolumn{5}{c}{$\sixtwoptShort$ FoM results} \\
\GCsp\, \text{bins} & \text{Fisher matrix} & \FoM & \Delta \FoM & \Delta \FoM (\%) \\
\midrule
% ---------- OPTIMISTIC ----------- %
\multicolumn{5}{c}{Optimistic scenario} \\
\midrule
\multirow{3}{*}{4} 
& [\threetwoptShort] + [\GCsp(P_k)] & 1216.16  & \text{--} & \text{--} \\
& \sixtwoptShort \, \mathrm{hybrid} &  1227.69 &   11.53 &  \positive{+0.95\%} \\
& \sixtwoptShort \, \mathrm{harmonic} &  1018.43 & -197.73 & \negative{-16.26\%} \\
\midrule
\multirow{1}{*}{12} 
& \sixtwoptShort \, \mathrm{harmonic} &  1073.31 & -142.85 & \negative{-11.75\%} \\
\midrule
\multirow{1}{*}{24} 
& \sixtwoptShort \, \mathrm{harmonic} &  1151.13 &  -65.03 &  \negative{-5.35\%} \\
\midrule
\multirow{1}{*}{40} 
& \sixtwoptShort \, \mathrm{harmonic} &  1296.44 &   80.28 &  \positive{+6.60\%} \\
\midrule
% ---------- PESSIMISTIC ---------- %
\multicolumn{5}{c}{Pessimistic scenario} \\
\midrule
% Fisher FoM DeltaFoM DeltaFoM (%)
\multirow{3}{*}{4} 
& [\threetwoptShort] + [\GCsp(P_k)]    & 549.37 & \text{--} & \text{--} \\
& \sixtwoptShort \, \mathrm{hybrid} &  555.87 &    6.50 &  \positive{+1.18\%} \\
& \sixtwoptShort \, \mathrm{harmonic} &  379.85 & -169.52 & \negative{-30.86\%} \\
\midrule
\multirow{1}{*}{12} 
& \sixtwoptShort \, \mathrm{harmonic} &  434.00 & -115.37 & \negative{-21.00\%} \\
\midrule
\multirow{1}{*}{24} 
& \sixtwoptShort \, \mathrm{harmonic} &  486.40 &  -62.97 & \negative{-11.46\%} \\
\midrule
\multirow{1}{*}{40} 
& \sixtwoptShort \, \mathrm{harmonic} &  550.82 &    1.45 &  \positive{+0.26\%} \\
\end{resultstable}
\caption{Figure-of-Merit of the $\sixtwoptShort$ statistics in the harmonic and hybrid approaches and in the hybrid one. The $\Delta\FoM$ columns quantify the differences with respect to the $[\threetwoptShort]+[\GCsp(P_k)]$ combination, which is used as reference to assess the impact on the $\FoM$ of the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations. In fact this combination does not include the contributions of $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$, but only the one of $\xc{\WL}{\GCph}$ -- see \eqref{eq:ch4_3x2pt_def}. For the definitions of $\sixtwoptShort$ statistics in the two approaches see \eqref{eq:ch4_6x2pt_harmonic_def} and \eqref{eq:ch4_6x2pt_hybrid_def}.}
\label{tab:ch4_6x2pt_fom_table}
\end{table*}
%-----------------------------------------%

\figref{fig:ch4_6x2pt_hybrid_vs_harmonic} shows that the hybrid approach performs drastically better in constraining $h$, producing a $\onesigma$ uncertainty on it which is always more than $70\%$ smaller than the one in the harmonic approach. The hybrid approach gives better uncertainties than the harmonic one for $\ns$ and $\Omb$ too. For $\ns$ the uncertainty of the hybrid approach is always smaller than the one of the harmonic approach by $30$-$40\%$. For $\Omb$ the hybrid approach gives a $60\%$ smaller uncertainty than the harmonic approach with $4$ bins, while the difference is about $20\%$ with $40$ bins. Concerning the uncertainty on $\Omm$ the two approaches produce results that are always comparable within $5\%$. Finally, on $\sige$ the harmonic approach with $12$ bins performs slightly better than the hybrid one. In the optimistic scenario the uncertainties on $\sige$ are always comparable, while in the pessimistic case the harmonic approach produces a $10\%$ smaller uncertainty when using $40$ tomographic bins.

% ERROR BARPLOT: 6x2pt
%-----------------------------------------%
\begin{figure*}[!ht]
\centering
\begin{tabular}{c}
\includegraphics[width=\textwidth]{Figures/6x2pt/error_horiz_plot_6x2pt_scenario_optimistic.pdf} \\
\includegraphics[width=\textwidth]{Figures/6x2pt/error_horiz_plot_6x2pt_scenario_pessimistic.pdf}
\end{tabular}
\caption{Comparison between harmonic and hybrid approaches for the case of $\sixtwoptShort$ statistics. The top panels refer to the optimistic scenario, while the bottom panels refer to the pessimistic one.}
\label{fig:ch4_6x2pt_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

% CONTOUR PLOT 6x2pt
%-----------------------------------------%
\begin{figure*}[!ht]
\centering
\begin{tabular}{c}
\includegraphics[width=\textwidth]{Figures/optimistic/contours/6x2pt/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf}\\
\includegraphics[width=\textwidth]{Figures/optimistic/contours/6x2pt/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the case of the $\sixtwoptShort$ statistics.}
\label{fig:ch4_contour_w0wa_6x2pt_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%




==> input/4-Conclusions.tex <==
\section{Conclusions and outlook}
\label{sec:ch4_conclusions}

In this work we present the results of the first \Euclid forecast which includes all the pairwise correlations between the main probes: weak lensing ($\WL$), photometric galaxy clustering ($\GCph$), and spectroscopic galaxy clustering ($\GCsp$). we have studied these correlations from two points of view. First, as off-diagonal terms of the covariance matrix, the \emph{cross-covariances}, that account for the statistical correlation between two different probes. Second, as additional observables, the \emph{cross-correlation signals} which can be sensitive to cosmological parameters.

My work is a natural extension of the \Euclid IST forecast~\citetalias{Blanchard:2019oqi}, where the authors studied $\WL$ and $\GCph$ including their correlation in the 2D harmonic domain. The $\GCsp$ was instead studied in the 3D Fourier domain, and in first approximation was assumed to be independent from the other two probes. Here we extend the harmonic formalism also to $\GCsp$, with the aim of including the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ correlations in the analysis as well. 

I have performed the forecast in two scenarios: one \emph{optimistic} and one \emph{pessimistic}, differing only for the multipole ranges chosen for the harmonic power spectra. In the optimistic scenario, the multipole range was $10 \leq \ell \leq 3000$ for both $\GCph$ and the projected $\GCsp$ and $10 \leq \ell \leq 5000$ for $\WL$. In the pessimistic scenario the ranges were $10 \leq \ell \leq 750$ and $10 \leq \ell \leq 1500$, respectively. 

I have considered two different approaches to include the cross-correlations in the analysis: the \emph{harmonic} approach and the \emph{hybrid} approach.

In the harmonic approach all the observables -- the two-point correlation functions -- are treated in the harmonic domain, i.e. using the $C(\ell)$'s formalism. This approach allows us to naturally take into account all cross-covariances between the observables, computed via \eqref{eq:ch4_4thorder_cov}. Nonetheless, it has the disadvantage to significantly lower the constraining power of $\GCsp$, since the integral along the line of sight prevents to fully exploit the accurate radial information provided by the spectroscopic clustering. In order to recover such information, we tried to refine the tomographic binning of the projected $\GCsp$, from $4$ bins (the baseline setting) up to a maximum of $40$ bins. 

In the hybrid approach all the observables are studied in the harmonic domain -- including $\xc{\WL}{\GCsp}$ and $\xc{\GCph}{\GCsp}$ -- except for the $\GCsp$ auto-correlation function. we have considered it as an independent observable, adding the $\GCsp$ Fisher matrix that had been computed in IST:F~\citetalias{Blanchard:2019oqi}, using the 3D Fourier power spectrum as observable. The main advantage of this approach is that it fully exploits the potential of $\GCsp$, keeping the information from radial BAO and RSD available thanks to accurate spectroscopic redshift measurements. At the same time the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations are included in the analysis as harmonic two-point functions, i.e. $C(\ell)$'s. However, this approach comes with two main drawbacks. First, for consistency with the official 3D spectroscopic galaxy clustering setting, only $4$ tomographic bins can be employed for computing the $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations, thus limiting the gain of constraining power which comes from their inclusion in the analysis. Second, it is not obvious how to compute the cross-covariance terms between the 3D $\GCsp$ auto-correlation and the other 2D observables. Therefore, accordingly to the conclusions from the analysis in the harmonic domain (which correctly accounts for the projected part of such cross-covariances), in the hybrid approach they have been neglected, leaving their computation to future work.

% Results
Here we summarise the results of the analysis in the three cases considered: the combination of $\GCph$ and $\GCsp$, the combination of $\WL$ and $\GCsp$, and the so-called $\sixtwoptShort$, i.e. the full combination of $\WL, \GCph, \GCsp$ altogether. In the latter case -- which is the most interesting for the \Euclid data analysis -- we presented the results in both the optimistic and pessimistic scenarios. Instead, for the two pairwise combinations $\GCph$-$\GCsp$ and $\WL$-$\GCsp$, we reported the results for the optimistic scenario alone. 

\paragraph{Combination of $\bGCph$ and $\bGCsp$} 
In the harmonic approach, the full analysis, $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, i.e. including cross-covariance and cross-spectrum, provides a FoM of 69 in the baseline setting of 4 spectroscopic bins. In the combination of $\GCph$ and $\GCsp$, the cross-covariance between the two (as said above, computed only in the harmonic approach) can be considered practically negligible, as it does not change the uncertainties on the cosmological parameters by more than $6\%$ and the FoM by more than $3\%$, with respect to the reference combination in the harmonic domain, $[\GCph]+[\GCsp]$, of the two probes taken as independent. In the harmonic approach, the $\xc{\GCph}{\GCsp}$ cross-correlation signal starts to be significant only when using $40$ bins, yielding a maximum FoM of $153$, which is $38\%$ higher than for the $[\GCph]+[\GCsp]$ combination. Regarding the uncertainties on $\wz$ and $\wa$, the improvement given by the $\xc{\GCph}{\GCsp}$ cross-correlation is X and Y respectively in the baseline $4$ bins setting, while it is $23\%$ and $25\%$ when using $40$ bins. The gain on the uncertainties on the other parameters is less than $5\%$ with $4$ bins and ranges from $10\%$ to $20\%$ with $40$ bins.

In the hybrid approach, the full analysis, $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$, including cross-spectrum but, as said above, neglecting cross-covariance, gives instead a FoM of $234$, which is much higher than in the harmonic case. However, in the hybrid case the impact of the $\xc{\GCph}{\GCsp}$ signal is negligible, as combining the probes as independent, $[\GCph]+[\GCsp(P_k)]$, provides a FoM of $230$, which is only $1.7\%$ lower than for the full analysis. The gain on the marginalised uncertainties is even smaller, being always less than $1\%$. Therefore, it is possible to conclude that the $\xc{\GCph}{\GCsp}$ cross-correlation can be neglected in the combination of $\GCph$ with $\GCsp$.

\paragraph{Combination of $\bWL$ and $\bGCsp$} 
In the harmonic approach, the full analysis, $[\WL+\GCsp+\xc{\WL}{\GCsp}]$, i.e. including cross-covariance and cross-spectrum, provides a FoM of 103 in the baseline setting of 4 spectroscopic bins. In the combination of $\WL$ and $\GCsp$, the cross-covariance (computed only in the harmonic approach) is even more negligible than for the combination of $\GCph$ with $\GCsp$, impacting the constraints always by less than $1\%$ with respect to the reference independent combination, $[\WL] + [\GCsp]$, computed in the harmonic domain. In this domain, the $\xc{\WL}{\GCsp}$ cross-correlation signal improves the constraints almost independently of the number of tomographic bins used for $\GCsp$, when compared to $[\WL]+[\GCsp]$. The percentage gain on the FoM produced by the $\rm XC$ inclusion is $38\%$ and $33\%$ with $4$ and $40$ bins respectively. This counterintuitive trend has been explained in \secref{sec:ch4_results_wlxsp}: it is due to the fact that the performance of the harmonic $\GCsp$ auto-spectrum alone improves faster than for $\xc{\WL}{\GCsp}$ when refining the spectroscopic binning. The value of the FoM provided by the full combination, $[\WL+\GCsp+\xc{\WL}{\GCsp}]$, increases to $188$ with $40$ bins, i.e. by $\sim 45\%$ with respect to the baseline bin setting.
%\placeholder{Uncertainties caso armonico WLxGCsp}
The $\xc{\WL}{\GCsp}$ improvement on the marginalised uncertainties on $\wz$ and $\wa$ exhibits the same trend observed for the FoM, decreasing from $20\%$ to $13\%$ as the number of spectroscopic bins increases from $4$ to $40$. This happens also for the uncertainties on $\Omm$ and $\sige$, with improvements ranging from $18\%$ to $12\%$ for the former and from $16\%$ to $11\%$ for the latter. The decrease on the uncertainties on $\Omb$ and $\ns$ ranges instead from $5\%$ to $8\%$ for the former and from $5\%$ to $2\%$ on the latter. Finally, the uncertainty on $h$ is the only exception to this trend, as its decrease improves from $1\%$ to $4\%$.


In the hybrid approach, the full analysis, $[\WL+\xc{\WL}{\GCsp}] + [\GCsp(P_k)]$, including cross-spectrum but neglecting cross-covariance, provides a FoM of $183$, which is comparable to the harmonic case when 40 bins are used, but is $\sim 56\%$ larger in the case of 4 bins. In the hybrid approach, the impact of the $\xc{\WL}{\GCsp}$ signal is not negligible, since the FoM is $15\%$ larger than for the independent combination, $[\WL]+[\GCsp(P_k)]$, of the two probes.
The improvements on the marginalised uncertainties are all comprised between $4\%$ and $8\%$, with no significant differences between the parameters. The uncertainty on $\Omm$ is the one improving the most, about $8\%$, while the one gaining the least is the uncertainty on $\ns$, decreasing by slightly less than $5\%$.

\paragraph{Combination of $\bWL, \bGCph, \bGCsp$ and the $\bsixtwoptShort$ statistics}
In the harmonic approach, the full $\sixtwoptShort$ analysis, \eqref{eq:ch4_6x2pt_harmonic_def}, i.e. including all cross-covariances and cross-spectra, provides a FoM of 1018 in the baseline setting of 4 spectroscopic bins.
The overall impact of the cross-covariances (computed only in the harmonic approach) between the angular $\GCsp$ and the observables of the $\threetwoptShort$ statistics, with respect to the independent combination $[\threetwoptShort]+[\GCsp]$, is slightly higher than for the pairwise combinations $\GCph$-$\GCsp$ and $\WL$-$\GCsp$, reported above. This is presumably due to the cumulative effect of three independent off-diagonal covariance blocks. These account for the covariances between the $\GCsp$ auto-spectrum and the three observable power spectra of the $\threetwoptShort$ statistics, namely the auto-spectra of $\WL$, $\GCph$ and their cross-spectrum $\xc{\WL}{\GCph}$. However, the increase on parameter uncertainties is never larger than $8\%$, as \figref{fig:ch4_3x2pt_sp_cov_impact} shows.

Both in the harmonic and hybrid approaches, the cross-correlations with $\GCsp$ are always negligible. The $\xc{\WL}{\GCsp}$ is definitely negligible both in the optimistic and pessimistic scenarios. 
In the harmonic approach, it always improves parameter constraints by less than $0.05\%$, with respect to the independent combination, $[\threetwoptShort+\GCsp]$, computed in the same approach. This is because the contribution brought by the $\xc{\WL}{\GCsp}$ is dominated by the $\xc{\WL}{\GCph}$, which is already present in the Fisher used as reference. Moreover, still in the harmonic approach, the effect of the $\xc{\WL}{\GCsp}$ becomes completely invisible with respect to the results from the independent combination, $[\threetwoptShort]+[\GCsp]$, computed in the same approach. This is because the difference is dominated by the cross-covariance between $\GCsp$ and $\threetwoptShort$, which is accounted when adding the cross-correlation observable.

% WLxGCsp
In the hybrid approach the situation is similar: the $\xc{\WL}{\GCsp}$ cross-correlation improves both the FoM and the uncertainties by always less than $0.05\%$ with respect to the constraints produced by the $[\threetwoptShort]+[\GCsp(P_k)]$ combination.
 
The effect of the $\xc{\GCph}{\GCsp}$ is larger than the one of $\xc{\WL}{\GCsp}$, both in the optimistic and pessimistic scenarios and both in the harmonic and in the hybrid approach. For this reason the $\sixtwoptShort$  statistics is essentially equivalent to adding $\xc{\GCph}{\GCsp}$ only.
Nonetheless, the improvement on the constraints produced by the $\xc{\GCph}{\GCsp}$ cross-correlation is almost always smaller than $10\%$. In the harmonic approach, its improvement is always below $5\%$ when compared to $[\threetwoptShort+\GCsp]$, while
it is dominated by the covariance effect when compared to $[\threetwoptShort]+[\GCsp]$. The only exception is when using $40$ bins for $\GCsp$: in this case the $\FoM$ improves by about $10\%$, while the marginalised uncertainties on $\Omb$ and $\h$ decrease by $\sim 15\%$. The uncertainties on the other parameters decrease by always less than $5\%$ instead.

In the hybrid approach the $\xc{\GCph}{\GCsp}$ improvement is always below $2\%$, for both FoM and uncertainties with respect to $[\threetwoptShort]+[\GCsp(P_k)]$, as in this case only the baseline setting of $4$ spectroscopic bins can be used for consistency with the official 3D spectroscopic galaxy clustering approach.

Finally, looking at the absolute performance, the values of the FoM are reported in \tabref{tab:ch4_6x2pt_fom_table}, which is possible to summarise as:

\begin{enumerate}
    \item the $[\threetwoptShort]+[\GCsp(P_k)]$ is taken as reference, and it gives a FoM of $1216$ ($549$) in the optimistic (pessimistic) scenario;
    
    \item the harmonic $\sixtwoptShort$ statistics with $40$ bins gives a FoM of $1296$ ($550$) in the optimistic (pessimistic) scenario, which is only $6.6\%$ ($0.26\%$) better than 1. When using $4$ bins it gives a FoM of $1018$ ($380$) in the optimistic (pessimistic) scenario, which instead is $15\%$ ($31\%$) worse than 1. 
    
    \item The hybrid $\sixtwoptShort$ statistics is essentially equivalent to the $[\threetwoptShort]+[\GCsp(P_k)]$, with a FoM of $1228$ ($556$) in the optimistic (pessimistic) scenario, only $1.18\%$ ($0.95\%$) better than 1. 
\end{enumerate}


Therefore, $\xc{\GCph}{\GCsp}$ and $\xc{\WL}{\GCsp}$ cross-correlations are negligible when added to the combination of $\GCsp$ and the $\threetwoptShort$ statistics, both in the harmonic and hybrid approaches.\\

In conclusion, either the cross-covariances (here computed only in the harmonic approach) or the cross-correlations (computed both in the harmonic and hybrid approaches) between $\GCsp$ and the other main probes of \Euclid, represented by the so-called $\threetwoptShort$ statistics, have a negligible impact on the cosmological parameter constraints.

In the case of the hybrid approach, we attribute this result to the effect of the $\xc{\WL}{\GCph}$ cross-correlation which is dominant with respect to the other cross-correlations, and to the higher performance of the full anisotropic 3D $\GCsp$ probe with respect to the projected one.

In the case of the 2D harmonic domain, we attribute this result to two main theoretical limitations of the projected $\GCsp$ probe: the high shot noise and the limited redshift range of the sample. we have found that, under two conditions, $\GCsp$ in harmonic space becomes equivalent to $\GCph$ in terms of constraining power, as it can be seen from \figref{fig:ch4_gcph_vs_gcsp_harmonic}. The first condition is to reduce the shot noise of $\GCsp$ to the same level of $\GCph$. The second is to restrict the tomographic bins of $\GCph$ to the $4$ photometric bins comprised in the $\GCsp$ redshift range, i.e. $z \in [0.9, 1.8]$. Under these same conditions, $\xc{\WL}{\GCsp}$ and $\xc{\WL}{\GCph}$ become equivalent in terms of constraining power too, as we show in \figref{fig:ch4_xcwlph_vs_xcwlsp}. Nonetheless, these conditions are not realistic.


% Extensions
%Future extensions of this work would be to overcome some approximations that have been made.

%First, we have computed the $C(\ell)$'s making use of the Limber approximation. It has been shown in a recent work~\cite{Fang2020} that this may result in a biased analysis. Using the exact expression for computing the angular power spectra would help to prevent this issue. Second, we have computed the $C(\ell)$'s covariance with \eqref{eq:ch4_4thorder_cov} as in IST:F~\citetalias{Blanchard:2019oqi}, and this formula only accounts for the Gaussian contributions. Comparison with covariances estimated from $N$-body simulations showed that the inclusion of non-Gaussian effects may be necessary to reach a better agreement with simulations~\cite{Krause2017}. In particular, including the super-sample covariance effect may help to improve Fisher forecasts by making the signal-to-noise ratio more realistic~\cite{Lacasa2019}. Third, in what we have called the ``hybrid approach'' we have neglected the covariances between the Fourier $\GCsp$ auto-correlation and the other observables. The computations done here with $\GCsp$ in the harmonic space suggest that these terms may be negligible. Nonetheless, providing an analytical modelling of these terms when $\GCsp$ is studied in the 3D Fourier space would surely help to confirm this hypothesis.



==> input/OLD_3-Results.tex <==
\section{Results}
\label{sec:ch4_results}
In this section the results of the forecast are presented. As a convention, the marginalised uncertainties presented are always fractional, i.e. divided by the values of the parameters in the reference cosmology \tabref{tab:ch4_cosmo_pars_fiducials}. The only exception are the contour plots, which are drawn using the original values of the uncertainties obtained from the diagonal of the inverted Fisher matrices.

The section is organised as follows. In \secref{sec:ch4_results_settings} the scenarios in which the forecast has been performed are described. 
In \secref{sec:ch4_results_phxsp} the results from the combination of $\GCph$ and $\GCsp$ are presented, reporting the results in the harmonic and hybrid approaches considered for the Fisher matrix computation. A comparison is also made between $\GCph$ and $\GCsp$ when treated as single probes in the harmonic domain.
In \secref{sec:ch4_results_wlxsp} the results are reported for the combination of $\WL$ and $\GCsp$. The results are reported both for the harmonic and for the hybrid approach. In addition a comparison of the impact of the $\xc{\WL}{\GCsp}$ cross-correlation with the one of $\xc{\WL}{\GCph}$ is discussed.
Finally in \secref{sec:ch4_results_6x2pt} the constraints coming from the combination of the full set of \Euclid main probes are shown, focusing on the impact of the cross-correlations on the constraints, both in the harmonic and in the hybrid approaches.

\subsection{Settings description}
\label{sec:ch4_results_settings}
The scenarios considered in this forecast are summarised in \tabref{tab:ch4_scenarios_settings}. Regarding the multipoles range, the two configurations have been studied: one \emph{optimistic} and one \emph{pessimistic}. In the optimistic scenario the multipole range for $\GCph$ and $\GCsp$ is set to $\ell \in [10, 3000]$, while it is $\ell \in [10, 5000]$ for $\WL$. In the pessimistic scenario instead the multipole range is $\ell \in [10, 750]$ for $\GCph$, $\GCsp$, and $\ell \in [10, 1500]$ for $\WL$. 

For galaxy clustering another distinction has been made, in order to better understand the differences between between $\GCph$ and $\GCsp$ when both are treated in the harmonic domain. In particular for spectroscopic clustering the alternative reduced shot noise described in \secref{sec:ch4_shot_noise} has been employed, in order to assess the impact on the results of the shot noise itself. However it is important to stress that this scenario in which the $\GCsp$ shot noise is reduced \emph{is not meant to be realistic}. It has been studied only to probe the theoretical limitations of the harmonic approach when applied to $\GCsp$. For photometric clustering instead the analysis has been performed using also an alternative tomographic binning, retaining only the $4$ photometric bins entirely comprised in the redshift range $z \in [0.9, 1.8]$. This has been done in order to make both $\GCph$ and $\xc{\WL}{\GCph}$ comparable with $\GCsp$ and $\xc{\WL}{\GCsp}$ respectively. In fact, apart from the shape of the galaxy distribution and the values of the galaxy bias, the two main differences between $\GCph$ and $\GCsp$ when treated in the harmonic domain are the shot noise and the volume of the catalog. In particular, as said in \secref{sec:ch4_shot_noise}, the shot noise of $\GCsp$ is larger than the one of $\GCph$, because the spectroscopic sample has a factor of $\sim 80$ less galaxies than the photometric one. Moreover, the redshift range covered by the photometric galaxy distribution is assumed to be $[0.001, 2.5]$ for $\GCph$, while for $\GCsp$ the range is restricted to $z \in [0.9, 1.8]$ because of the wavelength range in which NISP is sensitive.


\subsection{Combining photometric and spectroscopic clustering}
\label{sec:ch4_results_phxsp}

% FULL CL TABLE phsp
\begin{table*}[]
\centering
\begin{resultstable}{CL*{3}{C}}
\multicolumn{5}{c}{$\GCph\times\GCsp$ FoM: full harmonic approach} \\
\midrule
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta\FoM & \Delta\FoM(\%)\\
\midrule
\text{--} & [\GCph] & 63.12 & \text{--} & \text{--} \\
 \midrule
\multirow{4}{*}{4}
& [\GCph] + [\GCsp] & 65.69 & \text{--} & \text{--} \\
& [\GCph+\GCsp] & 63.95 & -1.75 & \negative{-2.66\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 69.63 & +3.94 & \positive{+6.00\%} \\
\midrule
\multirow{4}{*}{12}
& [\GCph] + [\GCsp] & 72.02 & \text{--} & \text{--}\\
& [\GCph+\GCsp] & 70.48 & -1.55 & \negative{-2.15\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 79.87 & +7.85 & \positive{+10.90\%} \\
\midrule
\multirow{4}{*}{24}
& [\GCph] + [\GCsp] & 85.02 & \text{--} & \text{--}\\
& [\GCph+\GCsp] & 83.88 & -1.13 & \negative{-1.33\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 108.35 & +23.34 & \positive{+27.45\%}\\
\midrule
\multirow{4}{*}{40}
& [\GCph] + [\GCsp] & 111.22 & \text{--} & \text{--} \\
& [\GCph+\GCsp] & 110.39 & -0.83 & \negative{-0.75\%} \\
& [\GCph+\GCsp+\xc{\GCph}{\GCsp}] & 153.71 & +42.48 & \positive{+38.20\%} \\
\end{resultstable}
\caption{Table reporting the $\FoM$ for $\GCph$, $\GCsp$ and their cross-correlation, in the full $C(\ell)$ approach.
The $\Delta\FoM$ column contains the variation of the figure of merit with respect to the independent sum $[\GCph] + [\GCsp]$ for the given number of bins. The $\Delta\FoM (\%)$ column is calculated by taking $\Delta\FoM$ as a percentage of the FoM of $[\GCph] + [\GCsp]$.}
\label{tab:ch4_results_phsp_fullcl}
\end{table*}

The results in the full harmonic approach are shown in \tabref{tab:ch4_results_phsp_fullcl}, where the column $\Delta\FoM$ reports the percentage difference between the figure of merit of the current row and the one of the sum of the two probes as independent $[\GCph] + [\GCsp]$ for that number of bins. In this case the Fisher coming from the full harmonic ($C(\ell)$) approach is $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, while the hybrid one is $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$.

% PERC.DIFF PLOT GCphxGCsp: FULL CL
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/perc_diff_errors/GCphGCsp_cov_and_xc_impact.pdf}
\caption{Impact, on 1--$\sigma$ parameter errors and $\FoM$, of cross-covariance and cross-correlation in the full harmonic approach for the combination of $\GCph$ and $\GCsp$. The left panel shows the impact of the cross-covariance, quantified with the percentage differences between $[\GCph+\GCsp]$ and $[\GCph] + [\GCsp]$. In the right panel the impact of the cross-correlation is reported, quantified by percentage differences of $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$ with respect to $[\GCph]+[\GCsp]$.}
\label{fig:ch4_phsp_fullcl_percdiff_plot}
\end{figure*}
%-----------------------------------------%

\subsubsection{Cross-covariance impact}
According to the naming convention defined in \secref{sec:ch4_fisher_fullcl}, the Fisher $[\GCph+\GCsp]$ is computed by taking into account the cross-covariance between $\GCph$ and $\GCsp$. Instead $[\GCph] + [\GCsp]$ represents the simple sum of the Fisher matrices of the two probes, and therefore in this Fisher matrix the cross-covariance is neglected. From \tabref{tab:ch4_results_phsp_fullcl} it can be seen that in any case the cross-covariance slightly worsens the FoM, as expected. 
Anyway the contribution is always smaller than $3\%$, in particular it is $-2.66\%$ with $4$ bins and $-0.75\%$ with $40$ bins. This decreasing trend can be understood as follows: the finer the tomographic binning of $\GCsp$ the smaller the support of the integrand of the off-diagonal terms $\bcl{\phsp}{\ell}$. Intuitively, the value of the integral over the $4$ thick bins is diluted into more than one bin when a finer binning is used. Hence the off-diagonal block $\cov{\bcl{\phph}{\ell}}{\bcl{\spsp}{\ell}}$ and its transposed counterpart become larger and sparser as the number of bins is increased, and therefore the cross-covariance contribution becomes smaller. 

This is true also for the marginalised uncertainties on the cosmological parameters, as it can be seen by \figref{fig:ch4_phsp_fullcl_percdiff_plot}, where the percentage difference on the uncertainties are drawn as vertical bars. In particular the impact of the cross-covariance is shown in the left panel as the comparison between $[\GCph+\GCsp]$ and $[\GCph]+[\GCsp]$, taking this last as reference. The parameters mostly affected by the covariance are $\Omb$ and $\h$, whose constraints in the 4 bins case worsen by $4\%$ and $6\%$ respectively. However, as soon as the binning is refined the effect gets smaller, as it happens for the FoM, becoming about $0.9\%$ for $\Omb$ and $2.5\%$ for $h$. The uncertainties on $\Omm, \ns$, and $\sige$ are instead affected by less than $2\%$ for all binnings. This outcome is confirmed also by \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}, reporting the relative marginalised uncertainties and the FoM as horizontal bars for the most relevant combinations involving photometric and spectroscopic galaxy clustering. The $[\GCph+\GCsp]$ bars (in blue) always have practically the same length as the $[\GCph] + [\GCsp]$ bars (in cyan), and they look more and more similar as the number of $\GCsp$ bins is increased. 

In conclusion the cross-covariance between $\GCph$ and $\GCsp$ can be considered practically negligible, as it does not change the uncertainties on the cosmological parameters by more than $6\%$ and the FoM by more than $3\%$.

% ERROR BARPLOT GCphxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/error_plots/phsp/fullcl_vs_2dx3d/phsp_fullcl_vs_2dx3d.pdf}
\caption{Comparison between full harmonic and hybrid harmonic-Fourier approaches for the case of $\GCph\times\GCsp$.}
\label{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

\subsubsection{Cross-correlation signal}

\paragraph{Full harmonic approach}
In the full harmonic approach the contribution to the FoM coming from the $\xc{\GCph}{\GCsp}$ cross-correlation is always positive, as reported in \tabref{tab:ch4_results_phsp_fullcl}, and it is about $6\%$ $(38\%)$ with $4$ $(40)$ $\GCsp$ bins. This gain is visible also in \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot}, where the FoM and the marginalised uncertainties of $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$ are represented with green bars. The improvements on the errors on $\wz, \wa$, and consequently on the FoM, are particularly visible for finer binnings, coherently with the results reported in the table. 

The marginalised uncertainties on the cosmological parameters also improve when including the $\mathrm{XC}$ signal, but the gain is more modest than the one on the FoM, as it is shown in the right panel of \figref{fig:ch4_phsp_fullcl_percdiff_plot}. The biggest improvements are on $\wz$ and $\wa$, whose uncertainties get smaller at most by $23\%$ and $25\%$ respectively. The uncertainty on the baryon density parameter $\Omb$ instead slightly increases by about $1\%$ with 4 bins and becomes smaller by $18\%$ with 40 bins. The small worsening on this parameter in the 4 bins case has been attributed to the contribution of the cross-covariance between the $C(\ell)$'s included in the data-vector of the Fisher $[\GCph+\GCsp+\xc{\GCph}{\GCsp}]$, which is not included in the computation of $[\GCph] + [\GCsp]$. In particular it is possible that with 4 bins the gain coming from the inclusion of the $\rm XC$ signal is compensated by the covariance contribution, giving an overall small worsening. However, as soon as the number of $\GCsp$ bins increases the positive contribution of the cross-correlation signal starts to dominate, and the constraints $\Omb$ improve too.
The uncertainty on the other parameters also improve, in particular $\Omm$ and $\sige$ gain at most $12\%$ when $40$ bins are used, as well as $\h$ and $\ns$ which improve by $7\%$ at maximum.

\paragraph{Hybrid approach}
In the hybrid approach instead the $\xc{\GCph}{\GCsp}$ has a quite small impact on the constraints: the marginalised uncertainties and FoM of $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$ are very similar to the ones of $[\GCph] + [\GCsp(P_k)]$, as \figref{fig:ch4_phsp_fullcl_vs_2dx3d_error_barplot} shows. This is also confirmed by the contour plots \figref{fig:ch4_contour_w0wa_phsp_fullcl_vs_2dx3d}: the $[\GCph] + [\GCsp(P_k)]$ curves (in yellow) are practically undistinguishable by the $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$ ones (in red).

% FoM Gain PLOT GCphxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/fom_gain/phsp_fom_gain.pdf}
\caption{Percentage gain on the FoM relative to photometric clustering alone ($[\GCph]$). In the left panel the computation has been done using the regular $\GCsp$ shot noise \eqref{eq:ch4_gc_shot_noise}, while in the right panel the reduced version \eqref{eq:ch4_reduced_gcsp_noise} has been used.}
\label{fig:ch4_phsp_fom_gain}
\end{figure*}
%-----------------------------------------%

% GCphxGCsp: hybrid vs harmonic table
%-----------------------------------------%
%\input{Chapters/inputtables/optimistic/phsp_hybrid_vs_harmonic}
%-----------------------------------------%

% GCphxGCsp, hybrid vs harmonic: % diff barplot
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=0.75\textwidth]{Figures/optimistic/perc_diff_errors/phsp_hybrid_vs_harmonic.pdf}
\caption{Percentage difference between FoM and marginalised 1--$\sigma$ errors of the hybrid and harmonic approaches, for the combination of $\GCph$ and $\GCsp$ in the baseline optimistic scenario. The percentage differences are normalised to the results of the harmonic approach.}
\label{fig:ch4_phsp_hybrid_vs_harmonic}
\end{figure*}
%-----------------------------------------%

\subsubsection{Hybrid approach vs harmonic approach}
As the plot in \figref{fig:ch4_phsp_hybrid_vs_harmonic} shows, the hybrid approach performs better than the harmonic one in constraining all the cosmological parameters, even if the constraining power of the harmonic approach significantly improves with increasing the number of $\GCsp$ tomographic bins. The harmonic approach has a FoM of $69$ ($153$) for $4$ ($40$) bins, while the hybrid one $234$, which is $236\%$ ($52\%$) larger, therefore the hybrid is better even when $40$ bins are used for the harmonic. This is true for all the parameters, in particular for the reduced Hubble constant $h$. In this case the hybrid approach performs remarkably better, with a gain on the marginalised uncertainty which is always between $75\%$ and $100\%$, and depends only slightly on the number of $\GCsp$ bins used for the harmonic approach. This is expected, since the hybrid approach takes advantage of the Fourier power spectrum as an observable, in which BAO and RSD are included. The constraints on the other parameters appear instead quite sensitive to the $\GCsp$ binning. The differences on $\wz, \wa$ significantly decrease from more than $50\%$ with $4$ bins to about $20\%$ with $40$ bins, as it could be expected from what happens to the FoM. 

In the case of the baryon density $\Omb$ the uncertainty from hybrid approach is more than $25\%$ smaller than in the harmonic when using $4$ bins, while the situation is reversed when $40$ bins are employed for the harmonic. In this last case the harmonic provides $\sim 10\%$ better constraints on $\Omb$ than hybrid. This indicates that the radial information recovered with finer binning helps in constraining $\Omb$, while this is not the case for $h$. For the other parameters $\Omm$, $\ns$, and $\sige$ the difference between the two approaches decreases significantly with the number of bins too.

From further investigation it turned out that a great limitation of the harmonic approach is the shot noise associated to the $\GCsp$ auto-correlation $C(\ell)$'s. This is in fact higher than the one of $\GCph$, since the expected number of $\Halpha$-emitter galaxies in the \Euclid catalog ($\sim \num{2e7}$) is smaller than the expected number of galaxies coming from the photometric one ($\sim \num{1.6e9}$). In order to quantify the impact of the spectroscopic shot noise the results of the forecast have been computed using also the artificially reduced version of the noise, as explained in \secref{sec:ch4_shot_noise}. 
The results are shown in \figref{fig:ch4_phsp_fom_gain}: in the left panel the normal $\GCsp$ shot noise computed from \eqref{eq:ch4_gc_shot_noise} is employed, while in the right panel the same plot is done with the reduced noise \eqref{eq:ch4_reduced_gcsp_noise}. From the plots it is manifest that lowering the shot noise in this way systematically boosts the results of the full harmonic approach by about 1 order of magnitude, making its performances comparable or even better than the hybrid one. In particular, as it can be expected, the observable gaining the most from this noise reduction is the harmonic $\GCsp$ auto-correlation. The $\xc{\GCph}{\GCsp}$ is not much affected instead, since the performances of the hybrid Fisher $[\GCph+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)]$ remain quite unaltered, and this is also expected. First of all in the hybrid approach only $4$ tomographic bins can be used for $\GCsp$, and this limits the constraining power of the $\GCph\times\GCsp$ cross-correlation angular power spectra $C^{\phsp}(\ell)$. Secondly the cross power spectra are only indirectly \eqref{eq:ch4_phsp_diag_cov_block} affected by the shot noise in contrast to what happens for the auto-correlation $\GCsp$ $C(\ell)$ \eqref{eq:ch4_spsp_diag_cov_block}. Consequently the impact of the shot noise on the cross-correlation is expected to be smaller than the one on the auto-correlation.
It is important to stress that this condition of reduced shot noise for $\GCsp$ is not realistic, since it is realised only if the number of galaxies in the spectroscopic sample equals the number of the photometric one, which evidently is not the case. This check has been done in order to better understand the limits of the harmonic approach, and not with the aim to provide a forecast of the constraints from $\GCsp$ and its combinations in a plausible scenario.

Therefore the conclusion is that, under realistic conditions, for the combination of $\GCph$ and $\GCsp$ the hybrid approach always provides better constraints than the harmonic one. Increasing the number of bins of the harmonic approach improves the constraints, but only when using $40$ bins the results becomes comparable with the hybrid approach.

% GCph vs GCsp in various settings
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=0.70\textwidth]{Figures/optimistic/gcph_vs_gcsp.pdf}
\caption{Comparison between the constraints coming from $[\GCph]$ and $[\GCsp]$ in the different configurations described in \secref{sec:ch4_results_settings}. The scale on the vertical axis is logarithmic to allow both the relative marginalised uncertainties and the FoM to be visible in the same plot.}
\label{fig:ch4_gcph_vs_gcsp_harmonic}
\end{figure*}
%-----------------------------------------%

\subsubsection{Comparing photometric and spectroscopic clustering in the harmonic domain}
As anticipated in \secref{sec:ch4_results_settings} two alternative configurations have been considered both for $\GCph$ and $\GCsp$. The baseline configuration for $\GCph$ consists in using all the $10$ redshift bins reported in \tabref{tab:ch4_photo_tomo_bins}, while in the alternative configuration only the $4$ bins strictly contained in the range $[0.9, 1.8]$ are considered. For spectroscopic clustering instead the baseline settings correspond to use the shot noise as calculated from the second equation of \eqref{eq:ch4_gc_shot_noise}, while the alternative consists in using the artificially reduced version \eqref{eq:ch4_reduced_gcsp_noise} of the noise.

The results are reported in \figref{fig:ch4_gcph_vs_gcsp_harmonic}. The height of the bars labeled with the cosmological parameters is equal to the relative marginalised uncertainty for that particular parameter. Regarding the FoM the height is instead given by the value of the FoM itself. From the plot it can be clearly seen that the constraints coming from $\GCph$ restricted to the $4$ bins in the spectroscopic range (blue bars) are very close to the ones of $\GCsp$ when the shot noise is reduced (yellow bars). This means that in these special conditions the two probes are essentially equivalent. This is expected, since the functional form of the weight for galaxy clustering is always the same, with the photometric function $W_i^{\rm ph}$ differing from the spectroscopic one $W_i^{\rm sp}$ only for the shape of the galaxy distribution and the values of the galaxy bias. The plot \figref{fig:ch4_gcph_vs_gcsp_harmonic} reports also the two probes in the baseline configuration, in which the $10$ bins written in \tabref{tab:ch4_photo_tomo_bins} are used for $\GCph$ (red bars) and the more realistic shot noise \eqref{eq:ch4_gc_shot_noise} is used for $\GCsp$ (green bars). On the one hand, the usage of all bins for $\GCph$ makes a big difference, improving the FoM by a factor of $\sim 30$ and reducing the uncertainties of about one order of magnitude on average. On the other hand, the realistic shot noise of $\GCsp$ significantly affects its performances, reducing the FoM by a factor of $\sim 10$ and making the uncertainties larger.

The conclusion is therefore that the shot noise and the survey volume are what makes the difference between $\GCph$ and $\GCsp$ in terms of constraints, when both are treated in the harmonic domain. In fact, when $\GCph$ is restricted to the same range of $\GCsp$ and the shot noise of the latter is reduced to the same level of the former, the two become equivalent in terms of constraining power.

%------CONTOUR GCphxGCsp-----------------%
\begin{figure*}
\centering
\begin{tabular}{cc}
\includegraphics[width=0.9\textwidth]{Figures/optimistic/contours/phsp/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf} \\
\includegraphics[width=0.9\textwidth]{Figures/optimistic/contours/phsp/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the combination of $\GCph$ and $\GCsp$.}
\label{fig:ch4_contour_w0wa_phsp_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%

% WLxGCsp
%-----------------------------------------%
\subsection{Combining weak lensing and spectroscopic clustering}
In this section the results from the combination of $\WL$ and $\GCsp$ are reported.
\label{sec:ch4_results_wlxsp}

% TABLE FoM WLxGCsp: FULL CL
%-----------------------------------------%
\begin{table*}[]
\centering
\begin{resultstable}{CL*{3}{C}}
\multicolumn{5}{c}{$\WL\times\GCsp$ results: full $C(\ell)$ approach} \\
\midrule
\GCsp \, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Delta \FoM (\%)\\
\midrule
\multirow{3}{*}{4} 
& [\WL] + [\GCsp] & 74.72 & \text{--} & \text{--} \\
& [\WL+\GCsp] & 74.37 & -0.35 & \negative{-0.47\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 103.56 & +28.83 & \positive{+38.59\%}\\
\midrule
\multirow{3}{*}{12} 
& [\WL] + [\GCsp] & 92.90 & \text{--} & \text{--}\\
& [\WL+\GCsp] & 92.77 & -0.13 & \negative{-0.14\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 131.38 & +38.47 & \positive{+41.41\%}\\
\midrule
\multirow{3}{*}{24} 
& [\WL] + [\GCsp] & 111.41 & \text{--}& \text{--}\\
& [\WL+\GCsp] & 111.42 & +0.01 & \positive{+0.0021\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 155.18 & +43.76 & \positive{+39.28\%}\\
\midrule
\multirow{3}{*}{40} 
& [\WL] + [\GCsp] & 141.12 & \text{--} & \text{--}\\
& [\WL+\GCsp] & 141.17 & +0.06 & \positive{+0.042\%}\\
& [\WL+\GCsp+\xc{\WL}{\GCsp}] & 188.45 & +47.34 & \positive{+33.55\%}\\
\end{resultstable}
\caption{Table reporting the $\FoM$ for $\WL$, $\GCsp$ and their cross-correlation, in the full $C(\ell)$ approach.
The $\Delta\FoM$ column contains the variation of the figure of merit with respect to the independent sum $[\WL] + [\GCsp]$ for the given number of bins. The $\Delta\FoM (\%)$ column is calculated by taking $\Delta\FoM$ as a percentage of the FoM of $[\WL] + [\GCsp]$.}
\label{tab:ch4_results_wlsp_fullcl}
\end{table*}
%-----------------------------------------%

% PERC.DIFF ERRORS PLOT WLxGCsp: FULL CL
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/perc_diff_errors/WLGCsp_cov_and_xc_impact.pdf}
\caption{Impact, on 1--$\sigma$ parameter errors and $\FoM$, of cross-covariance and cross-correlation in the full harmonic approach for the combination of $\WL$ and $\GCsp$. The left panel shows the impact of the cross-covariance, quantified with the percentage differences between $[\WL+\GCsp]$ and $[\WL] + [\GCsp]$. In the right panel the impact of the cross-correlation is reported, quantified by percentage differences of $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ with respect to $[\WL]+[\GCsp]$.}
\label{fig:ch4_wlsp_fullcl_percdiff_plot}
\end{figure*}
%-----------------------------------------%

\subsubsection{Cross-covariance impact}
In \tabref{tab:ch4_results_wlsp_fullcl} the results from the combinations of $\WL$ and $\GCsp$ in the full $C(\ell)$ approach are reported. In this case the cross-covariance is even more negligible than in the $\GCph\times\GCsp$ case effect on the figure of merit, always impacting by less than $0.5\%$ on the figure of merit. This effect gets smaller as the number of bins is increased, which is the starting from $-0.47\%$ with $4$ bins up to $+0.0021\%$ and $+0.042\%$ with $24$ and $40$ bins respectively, which are unexpectedly positive. However these contributions are so small to be considered as numerical fluctuations.

The same conclusion is drawn by looking at the effect of the covariance on the marginalised constraints on the cosmological parameters, shown in the left panel of \figref{fig:ch4_wlsp_fullcl_percdiff_plot}. The parameters that are affected the most are $h$ and $\Omb$, with variations of $0.7\%$ and $0.3\%$ respectively. The variations on all the other parameters are always well below $0.2\%$, and in all cases the absolute value of these variations decreases as the number of $\GCsp$ bins increases, confirming the trend observed for the FoM.

The conclusion here is that when combining $\WL$ and $\GCsp$ both treated in the harmonic domain the cross-covariance can be safely neglected. A similar result for another experiment other than \Euclid has been obtained in~\cite{Heymans2020}. Here the authors performed a joint data analysis combining weak lensing measurements from the Kilo-Degree Survey (KiDS-1000) and spectroscopic clustering from the Baryon Acoustic Oscillations Survey (BOSS) and 2-degree Field Lensing Survey (2dFLenS). The $\WL$ was treated with the angular power spectrum formalism as it has been done in this work, as well as $\GCsp$ when computing the cross-covariance between the two probes. The authors estimated the covariance matrix for the data through an analysis of over $\num{20 000}$ fast full-sky mock galaxy catalogues, finding that the off-diagonal (cross-covariance) terms were negligible with respect to the diagonal (auto-covariance) ones.

% ERROR BARPLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/error_plots/wlsp/fullcl_vs_2dx3d/wlsp_fullcl_vs_2dx3d.pdf}
\caption{Comparison between full harmonic and hybrid harmonic-Fourier approaches for the case of $\WL\times\GCsp$.}
\label{fig:ch4_wlsp_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

% FoM Gain PLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/fom_gain/wlsp_fom_gain.pdf}
\caption{Percentage gain on the FoM relative to weak lensing clustering alone ($[\WL]$). In the left panel the computation has been done using the regular $\GCsp$ shot noise \eqref{eq:ch4_gc_shot_noise}, while in the right panel the reduced version \eqref{eq:ch4_reduced_gcsp_noise} has been used.}
\label{fig:ch4_wlsp_fom_gain}
\end{figure*}
%-----------------------------------------%

\subsubsection{Cross-correlation impact}
The $\xc{\WL}{\GCsp}$ has a quite significant impact on the results, as \tabref{tab:ch4_results_wlsp_fullcl} shows. The percentage gain on the figure of merit is always around $+30-40\%$, with a slight dependence on the number of $\GCsp$ bins used. This can be explained by observing (see \figref{fig:ch4_weight_functions_plot}) that $\WL$ weight functions have a broad support, which increases cumulatively with the tomographic index. This suggests that increasing the radial resolution may not help too much in improving the constraints coming from the $\xc{\WL}{\GCsp}$, and this is what happens indeed. It is also worth noting that the FoM percentage gain does not strictly increase with the number of $\GCsp$ bins. In particular it is $+38\%$ at 4 bins and $+33\%$ with $40$ bins, with a maximum of about $+41\%$ at $12$ bins.
This seemingly counterintuitive fact is due to the normalisation of the FoM percentage gain, which is the FoM of $[\WL] + [\GCsp]$. This quantity depends on the number of $\GCsp$ bins too, and it increases slightly faster than the FoM variation of $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ with respect to it. This can be seen from the numbers reported in \tabref{tab:ch4_results_wlsp_fullcl}: the absolute figure-of-merit variation $\Delta\FoM$ saturates as the number of bins is increased, while the FoM of $[\WL] + [\GCsp]$ increases without decelerating. However the effect is quite small, and in fact it cannot be seen with naked eye in \figref{fig:ch4_wlsp_fullcl_vs_2dx3d_error_barplot}.

The marginalised 1--$\sigma$ uncertainties exhibit sensible decreasing when the $\xc{\WL}{\GCsp}$ cross-correlation signal is included, especially $\wz, \wa, \sige$ and $\Omm$, as it can be seen from \figref{fig:ch4_wlsp_fullcl_percdiff_plot}. For these parameters the improvement is always about $12\%$ at least with $4$ $\GCsp$ bins, and about $20\%$ at most when $40$ bins are used. The gain on the baryon density parameter $\Omb$ is more modest, being comprised between $5\%$ and $10\%$. The reduced Hubble constant $h$ and the scalar spectral index $\ns$ have instead by a gain which is always smaller than $5\%$. As it happens for the FoM, also for the uncertainties the gain of the $\rm XC$ seems to decrease when the number of $\GCsp$ bins. Again, the reason of this behaviour is that the normalisation of the percentage differences, which is $[\WL] + [\GCsp]$, exhibits uncertainties that improves faster than the error variation induced by the $\rm XC$. This is true for all parameters except for $h$, which is the parameter affected the least by the $\rm XC$.

When combining $\WL$ and $\GCsp$ in the hybrid approach the cross-correlation has a more significant impact than in the combination $\GCph$ and $\GCsp$. The figure-of-merit of $[\WL+\xc{\WL}{\GCsp}] + [\GCsp(P_k)]$, which is $\sim 183$, is $15\%$ higher than the one of the independent combination $[\WL] + [\GCsp(P_k)]$, which is $\sim 158$.

% WLxGCsp, hybrid vs harmonic: % diff barplot
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=0.75\textwidth]{Figures/optimistic/perc_diff_errors/wlsp_hybrid_vs_harmonic.pdf}
\caption{Percentage difference between FoM and marginalised 1--$\sigma$ errors of the hybrid and harmonic approaches, for the combination of $\WL$ and $\GCsp$ in the baseline optimistic scenario. The percentage differences are normalised to the results of the harmonic approach.}
\label{fig:ch4_wlsp_hybrid_vs_harmonic}
\end{figure*}
%-----------------------------------------%

% WLxGCph vs WLxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=0.6\textwidth]{Figures/optimistic/xcwlph_vs_xcwlsp.pdf}
\caption{Impact, on FoM and marginalised 1--$\sigma$ uncertainties, of $\xc{\WL}{\GCph}$ and $\xc{\WL}{\GCsp}$ in different configurations. The vertical bars represent the percentage differences on the uncertainties normalised to the independent sum of the two probes. For $\xc{\WL}{\GCph}$ the reference is $[\WL] + [\GCph]$, while for $\xc{\WL}{\GCsp}$ is $[\WL] + [\GCsp]$. Note that for the uncertainties the absolute value of the variation has been taken.}
\label{fig:ch4_xcwlph_vs_xcwlsp}
\end{figure*}
%-----------------------------------------%

\subsubsection{Hybrid approach vs harmonic approach}
In contrast to what happens in the case of $\GCph$ and $\GCsp$, when combining $\WL$ and $\GCsp$ the full harmonic approach can reach the FoM of the hybrid one. However, this only happens when $40$ $\GCsp$ bins are used to compute the full harmonic fisher $[\WL+\GCsp+\xc{\WL}{\GCsp}]$, with a FoM of $\sim 188$, which is only $3\%$ higher than the hybrid. Moreover \figref{fig:ch4_wlsp_hybrid_vs_harmonic} shows that the marginalised uncertainties in $\wz, \wa$ of the hybrid approach are smaller than their harmonic counterparts. Nonetheless, as said above, the harmonic FoM is slightly higher than the hybrid one. This is due to the correlation $\mathcal{C}_{\wz\wa}$ between the parameters, which enters the definition \eqref{eq:ch4_fom_def} of the FoM. This correlation is higher for the harmonic approach, and this compensates for the larger uncertainties, with a net result of slightly higher FoM. This effect can also be seen by zooming on the bottom panel of \figref{fig:ch4_contour_w0wa_wlsp_fullcl_vs_2dx3d}. The full harmonic contour (cyan) in $\wz$-$\wa$ plane is slightly narrower than the hybrid contour (red), even if being more elongated, and this has the net result of a smaller ellipse area.

Regarding the marginalised uncertainties, \figref{fig:ch4_wlsp_hybrid_vs_harmonic} shows that even in the $\WL\times\GCsp$ combination the hybrid approach always performs better than the harmonic one. As it happens for the combination of $\GCph$ and $\GCsp$, the best improvement is in constraining $h$, for which the improvement is comprised between $75\%$ and $100\%$. For the other parameters the gap is instead smaller than in the $\GCph\times\GCsp$ case, and it is significantly reduced as the number of $\GCsp$ bins is increased. The parameter most sensitive to the $\GCsp$ binning appears to be the baryon density $\Omb$, for which the difference between the two approaches passes from more than $50\%$ with $4$ bins to less than $10\%$ when using $40$ bins.

As it has been already pointed out in the case of $\GCph\times\GCsp$, from \figref{fig:ch4_wlsp_fom_gain} it can be seen that the shot noise of $\GCsp$ greatly affects the results of the combination of $\WL$ and $\GCsp$ too. When this shot noise is reduced according to the formula \eqref{eq:ch4_reduced_gcsp_noise} all the combinations involving $\GCsp$ systematically gain much more constraining power, as the comparison of the two panels of \figref{fig:ch4_wlsp_fom_gain} shows. In particular in this case the full harmonic approach $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ with the noise reduction becomes competitive with the hybrid approach already with $4$ bins, with a gain of $\sim 300\%$ relative to $\WL$ alone. Increasing the $\GCsp$ binning only improves the results, and as before the probe gaining the most from the noise reduction is $\GCsp$, since the two curves of $[\WL+\GCsp]$ and $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ converges towards each other as the number of bins is increased.

\subsubsection{Comparing $\xc{\WL}{\GCsp}$ with $\xc{\WL}{\GCph}$}
In \citetalias{Blanchard:2019oqi} it has been shown that the cross-correlation between weak lensing and photometric clustering is extremely relevant in improving the constraints on the cosmological parameters. In this work the same result is found: in particular, in the optimistic scenario defined in \secref{sec:ch4_results_settings} the FoM of $[\WL+\GCph+\xc{\WL}{\GCph}]$ is higher than the one of $[\WL] + [\GCph]$ by a factor of $5$, which means that the percentage gain induced by the cross-correlation signal is about $400\%$. The cross-correlation between $\WL$ and $\GCsp$ has instead a smaller impact on the constraints, with the FoM of $[\WL+\GCsp+\xc{\WL}{\GCsp}]$ being at most $\sim 40\%$ higher than the one of $[\WL] + [\GCsp]$. This is what happens when both $\GCph$ and $\GCsp$ are treated in the baseline settings, i.e. when the realistic shot noise \eqref{eq:ch4_gc_shot_noise} is used for $\GCsp$ and $10$ tomographic bins are employed for $\GCph$. In the alternative settings instead the two cross-correlations become practically equivalent. In \figref{fig:ch4_xcwlph_vs_xcwlsp} the absolute value of the percentage differences on marginalised uncertainties and FoM induced by the cross-correlation signals are represented with vertical bars. The bars corresponding to $\xc{\WL}{\GCsp}$ with the spectroscopic shot noise reduced (in yellow) have always almost the same height of those associated to $\xc{\WL}{\GCph}$ when $4$ bins are used for $\GCph$ (in blue). The only exception seems to be the marginalised uncertainty on $h$, but in that case the difference is simply due to the logarithmic scale used for the $y$ axis. At a closer look it is clear that the yellow bar represents a $3\%$ difference, while the blue one corresponds to about $1\%$.

Therefore it can be concluded that the shot noise and the volume of the galaxy catalog are what makes the differences between $\xc{\WL}{\GCph}$ and $\xc{\WL}{\GCsp}$ in terms of constraining power. 

% CONTOUR PLOT WLxGCsp
%-----------------------------------------%
\begin{figure*}
\centering
\begin{tabular}{cc}
\includegraphics[width=0.9\textwidth]{Figures/optimistic/contours/wlsp/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf} \\
\includegraphics[width=0.9\textwidth]{Figures/optimistic/contours/wlsp/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the combination of $\WL$ and $\GCsp$.}
\label{fig:ch4_contour_w0wa_wlsp_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%

% 6x2pt
%-----------------------------------------%

\subsection{Exploiting the \Euclid $\sixtwopt$}
\label{sec:ch4_results_6x2pt}
Here the result for the full $\sixtwopt$ are presented.


\subsubsection{Impact of the cross-covariances with $\GCsp$}

% Cov with GCsp impact 
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/6x2pt/cov_impact_6x2pt.pdf}
\caption{Impact, on FoM and marginalised 1-$\sigma$ errors, of cross covariances between $\GCsp$ and $[\WL+\GCph+\xc{\WL}{\GCph}]$, quantified with percentage differences on the constraints. The reference for the percentage are the constraints of $[\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp]$, where $\GCsp$ is considered as \emph{independent} from the rest.}
\label{fig:ch4_6x2pt_cov_impact}
\end{figure*}
%-----------------------------------------%




\subsubsection{Impact of the $\rm XC$ signals}
The results are shown in \tabref{tab:ch4_results_6x2pt_fullcl}.

%-----------------------------------------%
\begin{table*}
\centering
\begin{resultstable}{CL*{2}{C}}
\multicolumn{4}{c}{$\sixtwopt$ results: full $C(\ell)$ approach} \\
\midrule
\GCsp(C_{\ell})\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM \\
\midrule
\text{--} & \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(P_k) & 1216.16 & \text{--} \\
\midrule
\multirow{6}{*}{4} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1024.65 & \negative{-15.75\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1007.82 & \negative{-17.13\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1017.85 & \negative{-16.31\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1008.39 & \negative{-17.08\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 270.53 & \negative{-77.76\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1018.43 & \negative{-16.26\%} \\
\midrule
\multirow{6}{*}{12} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1069.11 & \negative{-12.09\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1055.66 & \negative{-13.20\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1072.60 & \negative{-11.80\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1056.24 & \negative{-13.15\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 293.85 & \negative{-75.84\%}\\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1073.31 & \negative{-11.75\%}\\
\midrule
\multirow{6}{*}{24}
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1124.17 & \negative{-7.56\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1115.45 & \negative{-8.28\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1148.06 & \negative{-5.60\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1116.16 & \negative{-8.22\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 331.84 & \negative{-72.71\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1148.98 & \negative{-5.52\%} \\
\midrule
\multirow{6}{*}{40} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1196.37 & \negative{-1.63\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1190.81 & \negative{-2.08\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1295.31 & \positive{+6.51\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1191.55 & \negative{-2.02\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 404.45 & \negative{-66.74\%} \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1296.44 & \positive{+6.60\%}\\
\end{resultstable}
\caption{Results for the $\sixtwopt$ in the full harmonic approach. The $\Delta\FoM$ column is referred to the $\FoM$ of the first row, i.e. $\WL+\GCph+\xc{\GCph}{\GCsp}+\GCsp(P_k)$.
}
\label{tab:ch4_results_6x2pt_fullcl}
\end{table*}
%-----------------------------------------%


\subsubsection{Hybrid approach vs harmonic approach}


% ERROR BARPLOT: 6x2pt
%-----------------------------------------%
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/optimistic/error_plots/6x2pt/fullcl_vs_2dx3d/6x2pt_fullcl_vs_2dx3d.pdf}
\caption{Comparison between full harmonic and hybrid harmonic-Fourier approaches for the case of $\sixtwopt$.}
\label{fig:ch4_6x2pt_fullcl_vs_2dx3d_error_barplot}
\end{figure*}
%-----------------------------------------%

% Cov WLxGCph-GCsp impact
%-----------------------------------------%
\begin{table*}
\centering
\begin{resultstable}{CL*{2}{C}}
\multicolumn{4}{c}{Impact of cross-covariance between $3\times 2 \mathrm{pt} (\WL,\GCph)$ and $\GCsp$} \\
\midrule
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM \\
\midrule
\multirow{2}{*}{4} 
& [\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp] & 1024.65 & \text{--} \\
& [\WL+\GCph+\xc{\WL}{\GCph}+\GCsp] & 1007.82 &    \negative{-1.64\%} \\
\midrule
\multirow{2}{*}{12} & [\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp] & 1069.11 &    \text{--} \\
& [\WL+\GCph+\xc{\WL}{\GCph}+\GCsp] & 1055.66 &    \negative{-1.26\%} \\
\midrule
\multirow{2}{*}{24} & [\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp] & 1126.19 &    \text{--} \\
& [\WL+\GCph+\xc{\WL}{\GCph}+\GCsp] & 1117.45 &    \negative{-0.78\%} \\
\midrule
\multirow{2}{*}{40} & [\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp] & 1196.37 &    \text{--} \\
& [\WL+\GCph+\xc{\WL}{\GCph}+\GCsp] & 1190.81 &    \negative{-0.46\%} \\
\end{resultstable}
\caption{Caption}
\label{tab:ch4_cov_impact_wlphxc_sp}
\end{table*}
%-----------------------------------------%

% 6x2pt CL VS 2Dx3D TABLE
%-----------------------------------------%
\begin{table*}
\begin{resultstable}{*{2}{L}*{3}{C}}
\multicolumn{5}{c}{Comparison between hybrid and full harmonic approaches (optimistic scenario)} \\
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Delta \FoM (\%) \\
\midrule
\multirow{3}{*}{4}
& [\WL+\GCph+\xc{\WL}{\GCph}] + [\GCsp(P_k)] & 1216.16 & \text{--} & \text{--} \\
& [\WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] + [\GCsp(P_k)] & 1227.69 & \text{--} & \text{--} \\
& [\WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] & 1018.43 & -209.26 & \negative{-17.05\%} \\
\midrule
\multirow{1}{*}{12}
& [\WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] & 1073.31 & -154.38 & \negative{-12.57\%} \\
\midrule
\multirow{1}{*}{24}
& [\WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] & 1151.13 & -76.56 & \negative{-6.24\%} \\
\midrule
\multirow{1}{*}{40} 
& [\WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}] & 1296.44 & +68.75 & \positive{+5.60\%} \\
\end{resultstable}
\caption{Comparison between the FoM in the full harmonic approach and in the hybrid one, for the $\sixtwopt$ case, in the optimistic scenario. The $\Delta\FoM$ column here contains the difference between the $\FoM$ in full harmonic approach and the $\FoM$ in the hybrid one. The percentage of the $\Delta\FoM(\%)$ column is computed by taking the hyrbid FoM as reference value.}
\label{tab:ch4_6x2pt_hybrid_vs_harmonic}
\end{table*}
%-----------------------------------------%

% CONTOUR PLOT 6x2pt
%-----------------------------------------%
\begin{figure*}
\centering
\begin{tabular}{cc}
\includegraphics[width=\textwidth]{Figures/optimistic/contours/6x2pt/fullcl_vs_2dx3d/contour_w0_wa_4_bins.pdf}\\
\includegraphics[width=\textwidth]{Figures/optimistic/contours/6x2pt/fullcl_vs_2dx3d/contour_w0_wa_40_bins.pdf} \\
\end{tabular}
\caption{Contour plots showing the comparison between the two approaches in the $\sixtwopt$ case.}
\label{fig:ch4_contour_w0wa_6x2pt_fullcl_vs_2dx3d}
\end{figure*}
%-----------------------------------------%



%+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+%
%+-+-+-+-+-+-+-+-APPENDICES+-+-+-+-+-+-+%
%+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+-+%

==> input/tables/optm_results/6x2pt/2dx3d.tex <==
\begin{table}[]
\begin{resultstable}{CL*{9}{C}}
\multicolumn{11}{c}{$\sixtwopt$ results: $\twoDxthreeD$ approach} \\
\midrule
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\text{--} & \WL+\GCph+\xc{\WL}{\GCph} + \GCsp(P_k) & 1216.16 & \text{--} & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0948 \\
\midrule
\multirow{4}{*}{4} 
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} + \GCsp(P_k) & 1216.55 & +0.03\% & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0947 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1227.17 & +0.90\% & 0.0148 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0944 \\
& \WL+\GCph+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 422.42 & -65.27\% & 0.0241 & 0.0131 & 0.0019 & 0.0029 & 0.0045 & 0.0486 & 0.1498 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1227.69 & +0.95\% & 0.0148 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0944 \\
\midrule
\multirow{4}{*}{12} 
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} + \GCsp(P_k) & 1216.72 & +0.05\% & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0947 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1236.52 & +1.67\% & 0.0147 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0941 \\
& \WL+\GCph+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 429.74 & -64.66\% & 0.0239 & 0.0130 & 0.0018 & 0.0029 & 0.0045 & 0.0483 & 0.1490 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1237.17 & +1.73\% & 0.0147 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0254 & 0.0941 \\
\midrule
\multirow{4}{*}{24} 
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} + \GCsp(P_k) & 1216.84 & +0.06\% & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0947 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1243.33 & +2.23\% & 0.0146 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0254 & 0.0937 \\
& \WL+\GCph+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 435.70 & -64.17\% & 0.0237 & 0.0129 & 0.0018 & 0.0029 & 0.0044 & 0.0478 & 0.1474 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1244.14 & +2.30\% & 0.0146 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0253 & 0.0937 \\
\midrule
\multirow{4}{*}{40}
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} + \GCsp(P_k) & 1216.97 & +0.07\% & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0947 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1253.55 & +3.07\% & 0.0145 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0252 & 0.0930 \\
& \WL+\GCph+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 445.24 & -63.39\% & 0.0234 & 0.0127 & 0.0018 & 0.0028 & 0.0044 & 0.0470 & 0.1445 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 1254.40 & +3.14\% & 0.0145 & 0.0059 & 0.0015 & 0.0019 & 0.0022 & 0.0252 & 0.0930 \\
\end{resultstable}
\caption{Results for the $\sixtwopt$ in the hybrid harmonic-Fourier approach. The $\Delta\FoM$ column here is the percentage difference with respect to the first row, which is the sum $\WL+\GCph+\xc{\WL}{\GCph} + \GCsp(P_k)$.}
\label{tab:ch4_results_6x2pt_2dx3d}
\end{table}

==> input/tables/optm_results/6x2pt/fullcl.tex <==
\begin{table*}
\begin{resultstable}{CL*{9}{C}}

\multicolumn{11}{c}{$\sixtwopt$ results: full $C(\ell)$ approach} \\
\midrule
\GCsp(C_{\ell})\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\text{--} & \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(P_k) & 1216.16 & \text{--} & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0948 \\
\midrule
\multirow{6}{*}{4} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1024.65 & -15.75\% & 0.0382 & 0.0061 & 0.0170 & 0.0036 & 0.0023 & 0.0283 & 0.1064 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1007.82 & -17.13\% & 0.0414 & 0.0062 & 0.0183 & 0.0037 & 0.0023 & 0.0283 & 0.1067 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1017.85 & -16.31\% & 0.0404 & 0.0062 & 0.0179 & 0.0036 & 0.0023 & 0.0283 & 0.1063 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1008.39 & -17.08\% & 0.0414 & 0.0062 & 0.0183 & 0.0037 & 0.0023 & 0.0283 & 0.1067 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 270.53 & -77.76\% & 0.0448 & 0.0154 & 0.0183 & 0.0043 & 0.0052 & 0.0654 & 0.2096 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1018.43 & -16.26\% & 0.0404 & 0.0061 & 0.0179 & 0.0036 & 0.0023 & 0.0283 & 0.1062 \\
\midrule
\multirow{6}{*}{12} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1069.11 & -12.09\% & 0.0316 & 0.0061 & 0.0143 & 0.0033 & 0.0023 & 0.0282 & 0.1055 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1055.66 & -13.20\% & 0.0337 & 0.0061 & 0.0151 & 0.0034 & 0.0023 & 0.0283 & 0.1056 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1072.60 & -11.80\% & 0.0325 & 0.0061 & 0.0146 & 0.0033 & 0.0023 & 0.0281 & 0.1048 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1056.24 & -13.15\% & 0.0337 & 0.0061 & 0.0151 & 0.0034 & 0.0023 & 0.0282 & 0.1056 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 293.85 & -75.84\% & 0.0377 & 0.0151 & 0.0149 & 0.0039 & 0.0051 & 0.0636 & 0.2040 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1073.31 & -11.75\% & 0.0325 & 0.0061 & 0.0146 & 0.0033 & 0.0023 & 0.0281 & 0.1048 \\
\midrule
\multirow{6}{*}{24}
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1124.17 & -7.56\% & 0.0266 & 0.0061 & 0.0121 & 0.0030 & 0.0022 & 0.0281 & 0.1041 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1115.45 & -8.28\% & 0.0277 & 0.0061 & 0.0126 & 0.0031 & 0.0022 & 0.0281 & 0.1041 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1148.06 & -5.60\% & 0.0268 & 0.0060 & 0.0122 & 0.0030 & 0.0022 & 0.0277 & 0.1022 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1116.16 & -8.22\% & 0.0277 & 0.0061 & 0.0126 & 0.0031 & 0.0022 & 0.0280 & 0.1040 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 331.84 & -72.71\% & 0.0323 & 0.0143 & 0.0125 & 0.0036 & 0.0049 & 0.0591 & 0.1900 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1148.98 & -5.52\% & 0.0268 & 0.0060 & 0.0122 & 0.0030 & 0.0022 & 0.0276 & 0.1021 \\
\midrule
\multirow{6}{*}{40} 
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(C_{\ell}) & 1196.37 & -1.63\% & 0.0231 & 0.0060 & 0.0106 & 0.0029 & 0.0022 & 0.0276 & 0.1015 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph} & 1190.81 & -2.08\% & 0.0237 & 0.0060 & 0.0108 & 0.0029 & 0.0022 & 0.0276 & 0.1015 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\GCph}{\GCsp} & 1295.31 & +6.51\% & 0.0193 & 0.0059 & 0.0094 & 0.0028 & 0.0021 & 0.0268 & 0.0978 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp} & 1191.55 & -2.02\% & 0.0237 & 0.0060 & 0.0108 & 0.0029 & 0.0022 & 0.0276 & 0.1014 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 404.45 & -66.74\% & 0.0249 & 0.0130 & 0.0097 & 0.0033 & 0.0045 & 0.0521 & 0.1682 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1296.44 & +6.60\% & 0.0193 & 0.0059 & 0.0094 & 0.0028 & 0.0021 & 0.0267 & 0.0977 \\

\end{resultstable}

\caption{Results for the $\sixtwopt$ in the full harmonic approach. The $\Delta\FoM$ column is referred to the $\FoM$ of the first row, i.e. $\WL+\GCph+\xc{\GCph}{\GCsp}+\GCsp(P_k)$.\\
%\textcolor{red}{MC: domanda... perché qui il riferimento è WL+GCph+XC(WL-Ph) e non WL+GCph+XC(WL-Ph)+GCsp(Cl)? Io non ti avevo chiesto il secondo confronto, ricordi? Mi mandasti le tabelle su slack https://euclidgc-swg.slack.com/files/U015DEYSV63/F02117MSUN4/schermata_2021-04-28_alle_19.27.42.pdf}}
}
\label{tab:ch4_results_6x2pt_fullcl}
\end{table*}



==> input/tables/optm_results/fullcl_vs_2dx3d_comparison.tex <==
\begin{table*}[]
\begin{resultstable}{CL*{9}{C}}
\multicolumn{11}{c}{Comparison between $\twoDxthreeD$ and full $C(\ell)$} \\
\midrule
\GCsp(C_{\ell})\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\multirow{3}{*}{\text{--}}
& \GCph+\GCsp(P_k) & 230.27 & \text{--} & 0.0345 & 0.0195 & 0.0024 & 0.0040 & 0.0056 & 0.0628 & 0.1972 \\
& \WL+\GCsp(P_k) & 158.13 & \text{--} & 0.0395 & 0.0228 & 0.0024 & 0.0052 & 0.0083 & 0.0776 & 0.2444 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\GCsp(P_k) & 1216.16 & \text{--} & 0.0149 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0948 \\
\midrule
\multirow{6}{*}{4} 
& \GCph+\xc{\GCph}{\GCsp}+\GCsp(P_k) & 234.54 & \text{--} & 0.0342 & 0.0194 & 0.0024 & 0.0040 & 0.0056 & 0.0625 & 0.1955 \\
& \WL+\xc{\WL}{\GCsp}+\GCsp(P_k) & 182.74 & \text{--} & 0.0369 & 0.0210 & 0.0023 & 0.0050 & 0.0077 & 0.0723 & 0.2303 \\
& \WL+\GCph+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}+\GCsp(P_k) & 1227.69 & \text{--} & 0.0148 & 0.0060 & 0.0015 & 0.0019 & 0.0022 & 0.0255 & 0.0944 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} & 69.63 & -70.31\% & 0.0537 & 0.0361 & 0.0290 & 0.0052 & 0.0082 & 0.1350 & 0.4826 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} & 103.56 & -43.33\% & 0.0878 & 0.0265 & 0.0379 & 0.0085 & 0.0097 & 0.1051 & 0.3376 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1018.43 & -17.05\% & 0.0404 & 0.0061 & 0.0179 & 0.0036 & 0.0023 & 0.0283 & 0.1062 \\
\midrule
\multirow{3}{*}{12} 
& \GCph+\GCsp+\xc{\GCph}{\GCsp} & 79.87 & -65.95\% & 0.0467 & 0.0330 & 0.0237 & 0.0048 & 0.0079 & 0.1251 & 0.4429 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} & 131.38 & -28.11\% & 0.0568 & 0.0258 & 0.0231 & 0.0068 & 0.0093 & 0.1027 & 0.3246 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1073.31 & -12.57\% & 0.0325 & 0.0061 & 0.0146 & 0.0033 & 0.0023 & 0.0281 & 0.1048 \\
\midrule
\multirow{3}{*}{24} 
& \GCph+\GCsp+\xc{\GCph}{\GCsp} & 107.90 & -53.99\% & 0.0389 & 0.0282 & 0.0196 & 0.0043 & 0.0069 & 0.0995 & 0.3453 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} & 155.18 & -15.08\% & 0.0461 & 0.0243 & 0.0179 & 0.0060 & 0.0087 & 0.0964 & 0.3027 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1148.98 & -6.41\% & 0.0268 & 0.0060 & 0.0122 & 0.0030 & 0.0022 & 0.0276 & 0.1021 \\
\midrule
\multirow{3}{*}{40} 
& \GCph+\GCsp+\xc{\GCph}{\GCsp} & 153.71 & -34.47\% & 0.0301 & 0.0240 & 0.0158 & 0.0039 & 0.0060 & 0.0760 & 0.2580 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} & 188.45 & +3.13\% & 0.0392 & 0.0219 & 0.0151 & 0.0055 & 0.0078 & 0.0846 & 0.2634 \\
& \WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp} & 1296.44 & +5.60\% & 0.0193 & 0.0059 & 0.0094 & 0.0028 & 0.0021 & 0.0267 & 0.0977 \\
\end{resultstable}
\caption{Comparison between full harmonic constraints and the corresponding three hybrid ones, represented by the first three rows of block with $4$ bins. The $\Delta\FoM$ column here represents the percentage difference between the $\FoM$ in full harmonic approach and the $\FoM$ in the hybrid one, normalized to the latter. Therefore the difference is reported only for the rows corresponding to the full harmonic fisher matrices.}
\label{tab:ch4_fullcl_vs_2dx3d_comparison}
\end{table*}



==> input/tables/optm_results/phsp/2dx3d.tex <==
\begin{table*}[]
%\caption*{Results from $\twoDxthreeD$ approach.}
%\begin{resultstable*}{CL*{9}{C}}
\multicolumn{11}{c}{$\GCph\times\GCsp$ results: $\twoDxthreeD$ approach} \\
\midrule
\GCsp \, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\text{--} & \GCph & 63.12 & \text{--} & 0.0567 & 0.0377 & 0.0306 & 0.0054 & 0.0085 & 0.1439 & 0.5209 \\
\text{--} & \GCsp(P_k) & 55.14 & \text{--} & 0.0679 & 0.0511 & 0.0032 & 0.0182 & 0.0209 & 0.1456 & 0.4481 \\
\text{--} & \GCph + \GCsp(P_k) & 230.27 & \text{--} & 0.0345 & 0.0195 & 0.0024 & 0.0040 & 0.0056 & 0.0628 & 0.1972 \\
\midrule
4 & \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 234.54 & +1.85\% & 0.0342 & 0.0194 & 0.0024 & 0.0040 & 0.0056 & 0.0625 & 0.1955 \\
12 & \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 237.75 & +3.25\% & 0.0338 & 0.0193 & 0.0024 & 0.0040 & 0.0056 & 0.0620 & 0.1941 \\
24 & \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 242.43 & +5.28\% & 0.0334 & 0.0191 & 0.0024 & 0.0040 & 0.0055 & 0.0610 & 0.1908 \\
40 & \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 250.36 & +8.73\% & 0.0327 & 0.0187 & 0.0024 & 0.0039 & 0.0054 & 0.0594 & 0.1850 \\
%\end{resultstable}
\caption{Marginalized errors (relative to fiducial values) and $\FoM$ for $\GCph$, $\GCsp$ and their cross-correlation, in the hybrid $\mathrm{2D}\times\mathrm{3D}$ approach. The $\Delta\FoM$ column contains the percentage variation of the figure of merit with respect to the independent sum $\GCph + \GCsp (P_k)$ for the given number of bins.}
\label{tab:ch4_results_phsp_2dx3d}
\end{table*}

==> input/tables/optm_results/phsp/fullcl.tex <==
% FULL CL TABLE
\begin{table*}[]
\begin{resultstable}{CL*{9}{C}}
\multicolumn{11}{c}{$\GCph\times\GCsp$ results: full $C(\ell)$ approach} \\
\midrule
\GCsp(C_{\ell})\, \text{bins} & \text{fisher} & \FoM & \Delta\FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\text{--} & \GCph & 63.12 & \text{--} & 0.0567 & 0.0377 & 0.0306 & 0.0054 & 0.0085 & 0.1439 & 0.5209 \\
 \midrule
\multirow{4}{*}{4}
 & \GCsp(C_{\ell}) & 0.33 & \text{--} & 0.8964 & 0.7637 & 0.3041 & 0.0725 & 0.2612 & 2.4018 & 6.4604 \\
 & \GCph + \GCsp(C_{\ell}) & 65.69 & \text{--} & 0.0532 & 0.0366 & 0.0278 & 0.0052 & 0.0085 & 0.1425 & 0.5135 \\
 & \GCph+\GCsp(\mathrm{Cov}) & 63.95 & -2.66\% & 0.0555 & 0.0373 & 0.0297 & 0.0053 & 0.0085 & 0.1434 & 0.5182 \\
 & \GCph+\GCsp+\xc{\GCph}{\GCsp} & 69.63 & +6.00\% & 0.0537 & 0.0361 & 0.0290 & 0.0052 & 0.0082 & 0.1350 & 0.4826 \\
\midrule
\multirow{4}{*}{12}
 & \GCsp(C_{\ell}) & 1.93 & \text{--} & 0.3193 & 0.2719 & 0.1187 & 0.0379 & 0.0992 & 0.8046 & 2.1238 \\
 & \GCph + \GCsp(C_{\ell}) & 72.02 & \text{--} & 0.0480 & 0.0346 & 0.0235 & 0.0050 & 0.0083 & 0.1370 & 0.4892 \\
 & \GCph+\GCsp(\mathrm{Cov}) & 70.48 & -2.15\% & 0.0494 & 0.0350 & 0.0248 & 0.0050 & 0.0083 & 0.1379 & 0.4938 \\
 & \GCph+\GCsp+\xc{\GCph}{\GCsp} & 79.87 & +10.90\% & 0.0467 & 0.0330 & 0.0237 & 0.0048 & 0.0079 & 0.1251 & 0.4429 \\
\midrule
\multirow{4}{*}{24} 
 & \GCsp(C_{\ell}) & 6.70 & \text{--} & 0.1559 & 0.1337 & 0.0672 & 0.0255 & 0.0537 & 0.3471 & 0.8824 \\
 & \GCph + \GCsp(C_{\ell}) & 85.02 & \text{--} & 0.0426 & 0.0315 & 0.0199 & 0.0046 & 0.0077 & 0.1224 & 0.4328 \\
 & \GCph+\GCsp(\mathrm{Cov}) & 83.88 & -1.33\% & 0.0432 & 0.0317 & 0.0207 & 0.0047 & 0.0077 & 0.1229 & 0.4354 \\
 & \GCph+\GCsp+\xc{\GCph}{\GCsp} & 108.35 & +27.45\% & 0.0389 & 0.0281 & 0.0196 & 0.0043 & 0.0069 & 0.0993 & 0.3444 \\
\midrule
\multirow{4}{*}{40}
& \GCsp(C_{\ell}) & 15.73 & \text{--} & 0.1057 & 0.0912 & 0.0496 & 0.0199 & 0.0388 & 0.2080 & 0.4827 \\
& \GCph + \GCsp(C_{\ell}) & 111.22 & \text{--} & 0.0367 & 0.0275 & 0.0172 & 0.0042 & 0.0069 & 0.0992 & 0.3443 \\
& \GCph+\GCsp(\mathrm{Cov}) & 110.39 & -0.75\% & 0.0370 & 0.0275 & 0.0176 & 0.0042 & 0.0069 & 0.0993 & 0.3453 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} & 153.71 & +38.20\% & 0.0301 & 0.0240 & 0.0158 & 0.0039 & 0.0060 & 0.0760 & 0.2580 \\
\end{resultstable}
\caption{Marginalized errors (relative to fiducial values) and $\FoM$ for $\GCph$, $\GCsp$ and their cross-correlation, in the full $C(\ell)$ approach. The $\Delta\FoM$ column contains the percentage variation of the figure of merit with respect to the independent sum $\GCph + \GCsp$ for the given number of bins.}
\label{tab:ch4_results_phsp_fullcl}
\end{table*}


==> input/tables/optm_results/phsp/phsp_2dx3d_approx_check.tex <==
\begin{table*}[htp]
%\begin{resultstable}{LL*{9}{C}}
\GCsp \, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\multirow{4}{*}{4} & \GCph+\xc{\GCph}{\GCsp} & 68.26 & +2.38\% & 0.0545 & 0.0364 & 0.0295 & 0.0053 & 0.0083 & 0.1361 & 0.4879 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) & 66.68 & \text{--} & 0.0581 & 0.0373 & 0.0323 & 0.0054 & 0.0083 & 0.1362 & 0.4890 \\
& \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 234.54 & +2.74\% & 0.0342 & 0.0194 & 0.0024 & 0.0040 & 0.0056 & 0.0625 & 0.1955 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 228.28 & \text{--} & 0.0347 & 0.0197 & 0.0024 & 0.0041 & 0.0056 & 0.0629 & 0.1976 \\
\midrule
\multirow{4}{*}{12} & \GCph+\xc{\GCph}{\GCsp} & 68.48 & -2.54\% & 0.0524 & 0.0355 & 0.0276 & 0.0052 & 0.0082 & 0.1359 & 0.4895 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) & 70.26 & \text{--} & 0.0568 & 0.0360 & 0.0317 & 0.0053 & 0.0080 & 0.1298 & 0.4652 \\
& \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 237.75 & +2.51\% & 0.0338 & 0.0193 & 0.0024 & 0.0040 & 0.0056 & 0.0620 & 0.1941 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 231.94 & \text{--} & 0.0343 & 0.0194 & 0.0024 & 0.0040 & 0.0056 & 0.0621 & 0.1951 \\
\midrule
\multirow{4}{*}{24} & \GCph+\xc{\GCph}{\GCsp} & 75.20 & -13.42\% & 0.0502 & 0.0335 & 0.0269 & 0.0050 & 0.0077 & 0.1245 & 0.4472 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) & 86.85 & \text{--} & 0.0525 & 0.0326 & 0.0303 & 0.0050 & 0.0073 & 0.1085 & 0.3829 \\
& \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 242.43 & -1.01\% & 0.0334 & 0.0191 & 0.0024 & 0.0040 & 0.0055 & 0.0610 & 0.1908 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 244.90 & \text{--} & 0.0333 & 0.0188 & 0.0024 & 0.0039 & 0.0055 & 0.0598 & 0.1867 \\
\midrule
\multirow{4}{*}{40} & \GCph+\xc{\GCph}{\GCsp} & 87.05 & -23.84\% & 0.0478 & 0.0312 & 0.0266 & 0.0048 & 0.0072 & 0.1087 & 0.3872 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) & 114.29 & \text{--} & 0.0361 & 0.0290 & 0.0252 & 0.0046 & 0.0065 & 0.0894 & 0.3120 \\
& \GCph+\xc{\GCph}{\GCsp} + \GCsp(P_k) & 250.36 & -15.18\% & 0.0327 & 0.0187 & 0.0024 & 0.0039 & 0.0054 & 0.0594 & 0.1850 \\
& \GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 295.16 & \text{--} & 0.0294 & 0.0175 & 0.0023 & 0.0038 & 0.0053 & 0.0553 & 0.1666 \\
%\end{resultstable}
\caption{The column $\Delta\FoM$ here contains the percentage difference between the case $\GCph+\mathrm{XC}$ and the one $\GCph+\GCsp+\xc{\GCph}{\GCsp} - \GCsp(C_\ell)$, using the second as the theoretical benchmark reference value.}
\label{tab:ch4_approx_check_phsp_2dx3d}
\end{table*}

==> input/tables/optm_results/wlsp/2dx3d.tex <==
\begin{table}[htp]
\begin{resultstable}{LL*{9}{C}}
\multicolumn{11}{c}{$\WL\times\GCsp$ results: $\twoDxthreeD$ approach} \\
\midrule
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\text{--} & \WL & 45.61 & \text{--}  & 0.4376 & 0.0342 & 0.1940 & 0.0300 & 0.0136 & 0.1368 & 0.4620 \\
\text{--} & \GCsp(P_k) & 55.14 & \text{--}  & 0.0679 & 0.0511 & 0.0032 & 0.0182 & 0.0209 & 0.1456 & 0.4481 \\
\text{--} & \WL + \GCsp(P_k) & 158.13 & \text{--}  & 0.0395 & 0.0228 & 0.0024 & 0.0052 & 0.0083 & 0.0776 & 0.2444 \\
\midrule
4 & \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 182.74 & +15.56\% & 0.0369 & 0.0210 & 0.0023 & 0.0050 & 0.0077 & 0.0723 & 0.2303 \\
12 & \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 182.84 & +15.63\% & 0.0370 & 0.0211 & 0.0023 & 0.0050 & 0.0077 & 0.0725 & 0.2303 \\
24 & \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 183.13 & +15.81\% & 0.0369 & 0.0211 & 0.0023 & 0.0050 & 0.0077 & 0.0725 & 0.2302 \\
40 & \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 183.57 & +16.09\% & 0.0369 & 0.0210 & 0.0023 & 0.0050 & 0.0077 & 0.0724 & 0.2299 \\
\end{resultstable}
\caption{Results for $\WL \times \GCsp$ in the hybrid harmonic-Fourier approach. The column $\Delta\FoM$ here represents the gain with respect $\WL + \GCsp(P_k)$.}
\label{tab:results_wlsp_2dx3d}
\end{table}

==> input/tables/optm_results/wlsp/fullcl.tex <==
\begin{table*}[]
\begin{resultstable}{CL*{9}{C}}
\multicolumn{11}{c}{$\WL\times\GCsp$ results: full $C(\ell)$ approach} \\
\midrule
\GCsp(C_{\ell}) \, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\multirow{3}{*}{4} & \WL + \GCsp(C_{\ell}) & 74.72 & — & 0.0924 & 0.0325 & 0.0383 & 0.0089 & 0.0117 & 0.1343 & 0.4324 \\
 & \WL+\GCsp(\mathrm{Cov}) & 74.37 & -0.47\% & 0.0927 & 0.0325 & 0.0385 & 0.0089 & 0.0117 & 0.1343 & 0.4331 \\
 & \WL+\GCsp+\xc{\WL}{\GCsp} & 103.56 & +38.59\% & 0.0878 & 0.0265 & 0.0379 & 0.0085 & 0.0097 & 0.1051 & 0.3376 \\
\midrule
\multirow{3}{*}{12} & \WL + \GCsp(C_{\ell}) & 92.90 & — & 0.0622 & 0.0313 & 0.0235 & 0.0071 & 0.0111 & 0.1294 & 0.4131 \\
 & \WL+\GCsp(\mathrm{Cov}) & 92.77 & -0.14\% & 0.0622 & 0.0313 & 0.0236 & 0.0071 & 0.0111 & 0.1294 & 0.4133 \\
 & \WL+\GCsp+\xc{\WL}{\GCsp} & 131.38 & +41.41\% & 0.0568 & 0.0258 & 0.0231 & 0.0068 & 0.0093 & 0.1027 & 0.3246 \\
\midrule
\multirow{3}{*}{24} & \WL + \GCsp(C_{\ell}) & 111.41 & — & 0.0508 & 0.0289 & 0.0184 & 0.0062 & 0.0102 & 0.1173 & 0.3728 \\
 & \WL+\GCsp(\mathrm{Cov}) & 111.42 & +0.0021\% & 0.0508 & 0.0289 & 0.0184 & 0.0062 & 0.0102 & 0.1173 & 0.3727 \\
 & \WL+\GCsp+\xc{\WL}{\GCsp} & 155.18 & +39.28\% & 0.0461 & 0.0243 & 0.0179 & 0.0060 & 0.0087 & 0.0964 & 0.3027 \\
\midrule
\multirow{3}{*}{40} & \WL + \GCsp(C_{\ell}) & 141.12 & — & 0.0423 & 0.0251 & 0.0156 & 0.0056 & 0.0088 & 0.0978 & 0.3075 \\
 & \WL+\GCsp(\mathrm{Cov}) & 141.17 & +0.042\% & 0.0423 & 0.0251 & 0.0157 & 0.0056 & 0.0088 & 0.0977 & 0.3074 \\
 & \WL+\GCsp+\xc{\WL}{\GCsp} & 188.45 & +33.55\% & 0.0392 & 0.0219 & 0.0151 & 0.0055 & 0.0078 & 0.0846 & 0.2634 \\
\end{resultstable}
\caption{Marginalized errors (relative to fiducial values) and $\FoM$ for $\WL$, $\GCsp$ and their cross-correlation, in the full $C(\ell)$ approach. The $\Delta\FoM$ column contains the percentage variation of the figure of merit with respect to the independent sum $\WL + \GCsp$ for the given number of bins.\\
\textcolor{red}{[MC: aggiungere tabella dove si vede l'effetto della sola covarianza di GCsp con WL, con GCph, e con XC(GCph,WL) senza aggiungere i corrispondenti segnali di XC GCsp-2D, ma tenendo conto del segnale XC(GCph,WL)...che è quello che chiedeva Martin...]}
}
\label{tab:ch4_results_wlsp_fullcl}
\end{table*}

==> input/tables/optm_results/wlsp/wlsp_2dx3d_approx_check.tex <==
\begin{table}[htp]
\begin{resultstable}{CL*{9}{C}}
\GCsp\, \text{bins} & \text{fisher} & \FoM & \Delta \FoM & \Omb & \Omm & \h & \ns & \sige & \wz & \wa \\
\midrule
\multirow{4}{*}{4} & \WL+\xc{\WL}{\GCsp} & 63.75 & \positive{+0.62\%} & 0.1997 & 0.0289 & 0.0906 & 0.0157 & 0.0113 & 0.1156 & 0.3933 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) & 63.36 & \text{--} & 0.3798 & 0.0280 & 0.1696 & 0.0264 & 0.0115 & 0.1071 & 0.3709 \\
& \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 182.74 & \negative{-1.93\%} & 0.0369 & 0.0210 & 0.0023 & 0.0050 & 0.0077 & 0.0723 & 0.2303 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 186.34 & \text{--} & 0.0365 & 0.0208 & 0.0022 & 0.0050 & 0.0077 & 0.0710 & 0.2254 \\
\midrule
\multirow{4}{*}{12} & \WL+\xc{\WL}{\GCsp} & 64.32 & \positive{+0.29\%} & 0.1803 & 0.0290 & 0.0826 & 0.0147 & 0.0112 & 0.1160 & 0.3931 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) & 64.13 & \text{--} & 0.3466 & 0.0279 & 0.1555 & 0.0245 & 0.0115 & 0.1069 & 0.3696 \\
& \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 182.84 & \negative{-2.76\%} & 0.0370 & 0.0211 & 0.0023 & 0.0050 & 0.0077 & 0.0725 & 0.2303 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 188.03 & \text{--} & 0.0365 & 0.0208 & 0.0022 & 0.0050 & 0.0076 & 0.0709 & 0.2253 \\
\midrule
\multirow{4}{*}{24} & \WL+\xc{\WL}{\GCsp} & 64.62 & \positive{+0.26\%} & 0.1768 & 0.0289 & 0.0811 & 0.0145 & 0.0112 & 0.1158 & 0.3923 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) & 64.45 & \text{--} & 0.3376 & 0.0279 & 0.1516 & 0.0241 & 0.0115 & 0.1066 & 0.3686 \\
& \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 183.13 & \negative{-2.83\%} & 0.0369 & 0.0211 & 0.0023 & 0.0050 & 0.0077 & 0.0725 & 0.2302 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 188.46 & \text{--} & 0.0365 & 0.0208 & 0.0022 & 0.0050 & 0.0076 & 0.0709 & 0.2251 \\
\midrule
\multirow{4}{*}{40} & \WL+\xc{\WL}{\GCsp} & 65.05 & \negative{-0.02\%} & 0.1738 & 0.0288 & 0.0798 & 0.0143 & 0.0112 & 0.1155 & 0.3908 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) & 65.06 & \text{--} & 0.3271 & 0.0278 & 0.1471 & 0.0235 & 0.0114 & 0.1061 & 0.3663 \\
& \WL+\xc{\WL}{\GCsp} + \GCsp(P_k) & 183.57 & \negative{-2.94\%} & 0.0369 & 0.0210 & 0.0023 & 0.0050 & 0.0077 & 0.0724 & 0.2299 \\
& \WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_{\ell}) + \GCsp(P_k) & 189.13 & \text{--} & 0.0364 & 0.0207 & 0.0022 & 0.0050 & 0.0076 & 0.0708 & 0.2246 \\
\end{resultstable} 
\caption{The column $\Delta\FoM$ here contains the percentage difference between the case $\WL+\xc{\WL}{\GCsp}$ and the one $\WL+\GCsp+\xc{\WL}{\GCsp} - \GCsp(C_\ell)$, using the second as the theoretical benchmark reference value.}
\label{tab:my_label}
\end{table}

==> new_commands.tex <==
\def\REF{{\bf REF }}
\def\stef#1{\textcolor{red}{#1}} % SC
\def\stefc#1{\textcolor{red}{{\sf [\textbf{Stef:} #1]}}} % SC

\newcommand{\CAMB}{\texttt{CAMB}\xspace}

% math generic
\newcommand{\de}{\mathrm{d}}
\newcommand{\aeq}{a_{\mathrm{eq}}}
\newcommand{\onesigma}{1\mbox{--}\sigma}
\newcommand{\versor}[1]{\hat{\mathbf{#1}}}

\newcommand{\cl}[3]{C^{#1}_{#2}({#3})}
\newcommand{\pdv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\Omm}{\Omega_{{\rm m},0}}
\newcommand{\Omb}{\Omega_{{\rm b},0}}
\newcommand{\mnu}{\sum m_\nu}
\newcommand{\h}{h}
\newcommand{\ns}{n_{\rm s}}
\newcommand{\wz}{w_0}
\newcommand{\wa}{w_a}
\newcommand{\sige}{\sigma_{8}}

\newcommand{\FoM}{\mathrm{FoM}}
\newcommand{\LCDM}{\Lambda\mathrm{CDM}}
\newcommand{\wzwaCDM}{\wz\wa\mathrm{CDM}}
\newcommand{\Halpha}{\mathrm{H}\alpha}
% nuisance parameters
\newcommand{\aIA}{\mathcal{A}_{\mathrm{IA}}}
\newcommand{\betaIA}{\beta_{\mathrm{IA}}}
\newcommand{\etaIA}{\eta_{\mathrm{IA}}}
\newcommand{\CIA}{C_{\mathrm{IA}}}

% probes
\newcommand{\WL}{\mathrm{WL}}
\newcommand{\GCsp}{\mathrm{GC}_{\rm sp}}
\newcommand{\GCph}{\mathrm{GC}_{\rm ph}}
\newcommand{\xc}[2]{\mathrm{XC}(#1,#2)}
\newcommand{\threetwoptShort}{3 \times 2 \mathrm{pt}}
\newcommand{\sixtwoptShort}{6 \times 2 \mathrm{pt}}
% bold probes
\newcommand{\bWL}{\mathbf{WL}}
\newcommand{\bGCsp}{\mathbf{GC_{sp}}}
\newcommand{\bGCph}{\mathbf{GC_{ph}}}
\newcommand{\bxc}[2]{\mathbf{XC}(#1,#2)}
\newcommand{\bthreetwoptShort}{\mathbf{3 \times 2 pt}}
\newcommand{\bsixtwoptShort}{\mathbf{6 \times 2 pt}}

\newcommand{\threetwoptLong}{\WL+\GCph+\xc{\WL}{\GCph}}
\newcommand{\sixtwoptLong}{\WL+\GCph+\GCsp+\xc{\WL}{\GCph}+\xc{\WL}{\GCsp}+\xc{\GCph}{\GCsp}}

% cl commands
\newcommand{\bcl}[2]{\mathbf{C}^{#1}(#2)}
\newcommand{\hatbcl}[1]{\hat{\mathbf{C}}^{#1}(\ell)}
\newcommand{\sgl}[3]{\Sigma^{#1}_{#2}(#3)}
\newcommand{\bsgl}[2]{\mathbf{\Sigma}^{#1}(#2)}
\newcommand{\cov}[2]{\operatorname{Cov}\left[#1, #2\right]}
\newcommand{\invcov}[2]{\operatorname{Cov}^{-1}\left[#1, #2\right]}

% cl combos
\newcommand{\wlwl}{\mathrm{wlwl}}
\newcommand{\phph}{\mathrm{phph}}
\newcommand{\spsp}{\mathrm{spsp}}
\newcommand{\wlph}{\mathrm{wlph}}
\newcommand{\phwl}{\mathrm{phwl}}
\newcommand{\wlsp}{\mathrm{wlsp}}
\newcommand{\spwl}{\mathrm{spwl}}
\newcommand{\phsp}{\mathrm{phsp}}
\newcommand{\spph}{\mathrm{spph}}

% linalg commands
\newcommand{\mvec}{\operatorname{vec}}
\newcommand{\mvecp}{\operatorname{vecp}}
\newcommand{\iden}{\mathds{1}}
\newcommand{\Bpmat}{B_p}
\newcommand{\Mpmat}{\mathcal{M}_p}
\newcommand{\commutmat}[1]{K_{#1}}

% REFERENCES COMMANDS
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\chpref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}

% FONT COMMANDS
\newcommand{\code}[1]{\texttt{#1}}

% COLOR COMMANDS
\newcommand{\positive}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\negative}[1]{\textcolor{Red}{#1}}

% TABLE COMMANDS
\newcolumntype{L}{>{$}l<{$}} % math-mode version of "l" column type
\newcolumntype{R}{>{$}r<{$}} % math-mode version of "r" column type
\newcolumntype{C}{>{$}c<{$}} % math-mode version of "c" column type

% NEW ENVIRONMENT FOR TABLES
\newenvironment{resultstable}[1]
    {\centering
    \setlength{\tabcolsep}{3.0pt}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{#1}
    \toprule
    }
    {\bottomrule
    \end{tabular}
    \end{adjustbox}
    }
    
% PAPER SPECIFIC NEW COMMANDS
\newenvironment{fullpageequation}
    {
    \begin{strip}
    \begin{center}
    }
    {
    \end{center}
    \end{strip}
    }

\newcommand{\lucap}[1]{\textcolor{blue}{[\textbf{Luca P:} #1]}}
